BANYAN. V. A Systematic All-Sky Survey for New Very Late-Type Low-Mass Stars and Brown Dwarfs in Nearby Young Moving Groups

We present the BANYAN All-Sky Survey (BASS) catalog, consisting of 228 new late-type (M4-L6) candidate members of nearby young moving groups (YMGs) with an expected false-positive rate of ~ 13%. This sample includes 79 new candidate young brown dwarfs and 22 planetary-mass objects. These candidates were identified through the first systematic all-sky survey for late-type low-mass stars and brown dwarfs in YMGs. We cross-matched the 2MASS and ALLWISE catalogs outside of the galactic plane to build a sample of 98 970 potential $\geq$ M5 dwarfs in the solar neighborhood and calculated their proper motions with typical precisions of 5-15 mas yr$^{-1}$. We selected highly probable candidate members of several YMGs from this sample using the Bayesian Analysis for Nearby Young AssociatioNs II tool (BANYAN II). We used the most probable statistical distances inferred from BANYAN II to estimate the spectral type and mass of these candidate YMG members. We used this unique sample to show tentative signs of mass segregation in the AB Doradus moving group and the Tucana-Horologium and Columba associations. The BASS sample has already been successful in identifying several new young brown dwarfs in earlier publications, and will be of great interest in studying the initial mass function of YMGs and for the search of exoplanets by direct imaging; the input sample of potential close-by $\geq$ M5 dwarfs will be useful to study the kinematics of low-mass stars and brown dwarfs and search for new proper motion pairs.

==> bass_table_2_long.tex <==
\onecolumngrid
\LongTables
\begin{deluxetable*}{llcccccccccclcc}
\tablecolumns{15}
\tablecaption{All-Sky Search for > M5 Candidates in Young Moving Groups.\label{tab:bass1}}
\tablehead{\colhead{\href{http://www.ipac.caltech.edu/2mass/}{\emph{2MASS}}} & \colhead{Estim.} & \colhead{} & \multicolumn{3}{c}{\href{http://www.ipac.caltech.edu/2mass/}{\emph{2MASS}}} & \colhead{} & \multicolumn{2}{c}{\href{http://wise2.ipac.caltech.edu/docs/release/allwise/}{\emph{AllWISE}}} & \colhead{} & \colhead{$\mu_\alpha\cos\delta$} & \colhead{$\mu_\delta$}  & \colhead{Member-} & \colhead{Bayesian} & \colhead{Contamination} \\
\cline{4-6}
\cline{8-9}
\colhead{Designation} & \colhead{SpT} & \colhead{} & \colhead{$J$} & \colhead{$H$} & \colhead{$K_S$} & \colhead{} & \colhead{$W1$} & \colhead{$W2$} & \colhead{} & \colhead{(\masyr)} & \colhead{(\masyr)} & \colhead{ship} & \colhead{Prob. (\%)} & \colhead{Prob. (\%)}}
\startdata
\cutinhead{Candidates with a High Probability}
00011217+1535355 & L3.2 & & $15.52$ & $14.51$ & $13.71$ & & $12.97$ & $12.54$ & & $139.6 \pm 7.8$ & $-183.5 \pm 11.8$ & ABDMG  & $79.1$ & $1.6$\\
00040288-6410358 & L2.5 & & $15.79$ & $14.83$ & $14.01$ & & $13.41$ & $12.96$ & & $77.7 \pm 3.0$ & $-56.1 \pm 8.4$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
00041589-8747254 & M5.7 & & $12.90$ & $12.20$ & $11.86$ & & $11.65$ & $11.41$ & & $77.3 \pm 2.0$ & $-29.9 \pm 9.2$ & THA  & $55.4$ & $< 0.1$\\
00065794-6436542 & M6.9 & & $13.39$ & $12.66$ & $12.17$ & & $11.74$ & $11.42$ & & $92.7 \pm 3.1$ & $-71.0 \pm 7.3$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
00111532-3756553 & M5.7 & & $12.15$ & $11.60$ & $11.22$ & & $11.02$ & $10.79$ & & $105.7 \pm 5.0$ & $-77.4 \pm 7.4$ & THA  & $80.2$ & $< 0.1$\\
00182834-6703130 & M9.6 & & $15.46$ & $14.48$ & $13.71$ & & $13.19$ & $12.80$ & & $83.6 \pm 2.9$ & $-65.0 \pm 9.3$ & THA\tablenotemark{a} & $99.8$ & $< 0.1$\\
00191296-6226005 & M9.7 & & $15.64$ & $14.62$ & $13.96$ & & $13.38$ & $12.96$ & & $66.1 \pm 2.9$ & $-50.6 \pm 8.4$ & THA  & $99.5$ & $< 0.1$\\
00212774-6351081 & M4.0 & & $11.02$ & $10.48$ & $10.11$ & & $9.91$ & $9.66$ & & $83.0 \pm 2.9$ & $-57.6 \pm 7.2$ & THA  & $99.8$ & $< 0.1$\\
00235732-5531435 & M4.5 & & $11.11$ & $10.55$ & $10.24$ & & $10.07$ & $9.87$ & & $92.3 \pm 3.4$ & $-67.7 \pm 7.4$ & THA\tablenotemark{a} & $99.5$ & $< 0.1$\\
00305785-6550058\tablenotemark{b} & M2.1 & & $9.82$ & $9.24$ & $8.95$ & & $8.79$ & $8.61$ & & $70.3 \pm 2.9$ & $-51.9 \pm 8.7$ & THA & $99.1$ & $< 0.1$\\
00325584-4405058 & M9.5 & & $14.78$ & $13.86$ & $13.27$ & & $12.84$ & $12.52$ & & $125.9 \pm 4.9$ & $-79.4 \pm 6.9$ & THA  & $82.0$ & $7.0$\\
00344300-4102266 & L2.4 & & $15.71$ & $14.81$ & $14.08$ & & $13.52$ & $13.12$ & & $96.9 \pm 5.1$ & $-51.8 \pm 7.0$ & THA  & $96.1$ & $< 0.1$\\
00354313+0233137 & M4.8 & & $10.52$ & $9.93$ & $9.54$ & & $9.32$ & $9.12$ & & $153.8 \pm 8.7$ & $-185.3 \pm 9.0$ & ABDMG\tablenotemark{a} & $88.2$ & $1.4$\\
00374306-5846229 & M9.2 & & $15.37$ & $14.26$ & $13.59$ & & $13.15$ & $12.77$ & & $81.7 \pm 3.2$ & $-40.0 \pm 6.9$ & THA\tablenotemark{a} & $99.8$ & $< 0.1$\\
00413538-5621127 & M5.3 & & $11.96$ & $11.32$ & $10.86$ & & $10.63$ & $10.37$ & & $110.0 \pm 3.6$ & $-55.9 \pm 6.6$ & THA\tablenotemark{a} & $99.5$ & $< 0.1$\\
00452143+1634446 & L2.4 & & $13.06$ & $12.06$ & $11.37$ & & $10.78$ & $10.40$ & & $367.0 \pm 11.7$ & $-47.7 \pm 9.9$ & ARG  & $94.7$ & $4.5$\\
00514081-5913320 & M4.5 & & $11.28$ & $10.70$ & $10.40$ & & $10.21$ & $9.99$ & & $92.6 \pm 3.1$ & $-48.5 \pm 8.2$ & THA  & $99.8$ & $< 0.1$\\
00525451-6624501 & L0.3 & & $15.67$ & $14.69$ & $13.98$ & & $13.35$ & $12.95$ & & $74.9 \pm 2.4$ & $-10.2 \pm 6.9$ & ABDMG\tablenotemark{a} & $11.8$ & $< 0.1$\\
01033563-5515561 & M3.4 & & $10.16$ & $9.58$ & $9.24$ & & $9.05$ & $8.80$ & & $111.6 \pm 3.6$ & $-43.8 \pm 8.1$ & THA\tablenotemark{a} & $99.3$ & $< 0.1$\\
01075572-6030194 & M5.3 & & $11.84$ & $11.25$ & $10.97$ & & $10.76$ & $10.56$ & & $105.0 \pm 3.4$ & $-33.9 \pm 7.4$ & THA  & $99.6$ & $< 0.1$\\
01134031-5939346 & M3.3 & & $9.95$ & $9.34$ & $9.06$ & & $8.90$ & $8.70$ & & $99.4 \pm 3.7$ & $-25.2 \pm 9.8$ & THA\tablenotemark{a} & $99.3$ & $< 0.1$\\
01174748-3403258 & M9.6 & & $15.18$ & $14.21$ & $13.49$ & & $13.05$ & $12.64$ & & $108.5 \pm 5.5$ & $-58.9 \pm 6.3$ & THA & $98.8$ & $< 0.1$\\
01180670-6258591 & M4.9 & & $11.53$ & $10.96$ & $10.64$ & & $10.44$ & $10.22$ & & $95.4 \pm 3.0$ & $-49.0 \pm 6.7$ & THA  & $99.3$ & $< 0.1$\\
01205114-5200349 & L2.5 & & $15.64$ & $14.66$ & $13.75$ & & $13.23$ & $12.82$ & & $101.9 \pm 4.0$ & $-47.0 \pm 6.8$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
01231125-6921379 & M5.3 & & $12.32$ & $11.71$ & $11.32$ & & $11.07$ & $10.83$ & & $89.9 \pm 2.3$ & $-26.3 \pm 6.7$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
01243060-3355014 & M5.2 & & $10.56$ & $10.01$ & $9.68$ & & $9.48$ & $9.29$ & & $164.2 \pm 5.5$ & $-140.9 \pm 6.5$ & ABDMG  & $88.4$ & $1.5$\\
01265327-5505506\tablenotemark{b} & M4.5 & & $12.04$ & $11.48$ & $11.09$ & & $10.90$ & $10.64$ & & $96.8 \pm 4.5$ & $-37.6 \pm 9.2$ & THA & $99.8$ & $< 0.1$\\
01294256-0823580\tablenotemark{b} & M2.5 & & $10.65$ & $10.09$ & $9.77$ & & $9.55$ & $9.33$ & & $100.7 \pm 8.4$ & $-56.4 \pm 9.0$ & BPMG & $71.6$ & $< 0.1$\\
01320814-6023536 & M4.5 & & $11.42$ & $10.84$ & $10.52$ & & $10.33$ & $10.13$ & & $89.2 \pm 3.0$ & $-23.5 \pm 8.2$ & THA  & $99.8$ & $< 0.1$\\
01344601-5707564 & M5.3 & & $12.07$ & $11.52$ & $11.16$ & & $10.98$ & $10.75$ & & $98.6 \pm 3.4$ & $-29.3 \pm 7.3$ & THA  & $99.8$ & $< 0.1$\\
01372781-4558261 & M4.6 & & $11.11$ & $10.54$ & $10.19$ & & $9.99$ & $9.76$ & & $117.9 \pm 4.3$ & $-40.3 \pm 6.3$ & THA  & $98.6$ & $< 0.1$\\
01393605-6455456 & M5.4 & & $12.58$ & $11.99$ & $11.58$ & & $11.42$ & $11.19$ & & $80.6 \pm 2.6$ & $-6.0 \pm 6.7$ & THA  & $88.9$ & $< 0.1$\\
01415823-4633574 & M9.0 & & $14.83$ & $13.88$ & $13.10$ & & $12.58$ & $12.19$ & & $111.2 \pm 4.3$ & $-45.7 \pm 6.5$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
01443191-4604318 & M5.3 & & $11.88$ & $11.30$ & $10.98$ & & $10.75$ & $10.49$ & & $102.8 \pm 5.0$ & $-42.2 \pm 7.1$ & THA  & $99.6$ & $< 0.1$\\
01484859-5201158 & M4.0 & & $10.87$ & $10.35$ & $9.99$ & & $9.81$ & $9.58$ & & $104.2 \pm 3.7$ & $-28.9 \pm 6.4$ & THA\tablenotemark{a} & $99.8$ & $< 0.1$\\
01504543-5716488 & M5.3 & & $12.16$ & $11.56$ & $11.28$ & & $11.04$ & $10.80$ & & $100.4 \pm 3.3$ & $-27.2 \pm 6.5$ & THA  & $99.9$ & $< 0.1$\\
01531463-6744181 & L2.7 & & $16.41$ & $15.11$ & $14.42$ & & $13.73$ & $13.26$ & & $82.0 \pm 2.7$ & $-21.3 \pm 9.4$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
01532494-6833226 & M3.9 & & $11.07$ & $10.49$ & $10.18$ & & $10.00$ & $9.77$ & & $93.4 \pm 2.6$ & $-16.7 \pm 7.3$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
02004709-5105206 & L5.9 & & $16.41$ & $14.94$ & $13.87$ & & $12.89$ & $12.36$ & & $171.3 \pm 5.4$ & $-75.5 \pm 10.0$ & ABDMG\tablenotemark{a} & $99.1$ & $0.7$\\
02013900-5948345 & M5.3 & & $11.78$ & $11.19$ & $10.87$ & & $10.68$ & $10.48$ & & $118.7 \pm 3.5$ & $-49.4 \pm 7.3$ & THA & $33.1$ & $< 0.1$\\
02025502-7259155 & M3.5 & & $10.71$ & $10.06$ & $9.79$ & & $9.58$ & $9.36$ & & $92.0 \pm 2.2$ & $-2.5 \pm 6.6$ & THA\tablenotemark{a} & $99.6$ & $< 0.1$\\
02103857-3015313 & M9.3 & & $15.07$ & $14.16$ & $13.50$ & & $13.03$ & $12.68$ & & $98.4 \pm 5.7$ & $-45.2 \pm 7.5$ & THA  & $99.7$ & $< 0.1$\\
02153328-5627175 & M5.0 & & $11.93$ & $11.32$ & $10.95$ & & $10.66$ & $10.40$ & & $85.0 \pm 3.3$ & $-8.3 \pm 6.4$ & THA\tablenotemark{a} & $99.3$ & $< 0.1$\\
02180960-6657524 & M3.7 & & $10.82$ & $10.27$ & $9.97$ & & $9.79$ & $9.57$ & & $95.3 \pm 2.7$ & $-6.0 \pm 6.5$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
02192210-3925225 & M4.8 & & $11.38$ & $10.81$ & $10.40$ & & $10.15$ & $9.90$ & & $100.1 \pm 4.6$ & $-45.8 \pm 6.3$ & THA\tablenotemark{a} & $99.2$ & $< 0.1$\\
02212859-6831400 & M7.2 & & $13.97$ & $13.27$ & $12.81$ & & $12.49$ & $12.20$ & & $64.7 \pm 2.1$ & $0.2 \pm 6.7$ & THA  & $90.2$ & $< 0.1$\\
02214262-5947087 & M5.3 & & $11.92$ & $11.35$ & $11.01$ & & $10.81$ & $10.59$ & & $86.4 \pm 3.3$ & $-24.6 \pm 8.1$ & THA  & $99.6$ & $< 0.1$\\
02215494-5412054 & M8.1 & & $13.90$ & $13.22$ & $12.66$ & & $12.34$ & $11.97$ & & $124.1 \pm 4.0$ & $-24.1 \pm 8.2$ & THA  & $98.9$ & $< 0.1$\\
02235464-5815067 & M9.3 & & $15.07$ & $14.00$ & $13.42$ & & $12.84$ & $12.46$ & & $112.8 \pm 3.7$ & $-16.8 \pm 7.4$ & THA  & $99.9$ & $< 0.1$\\
02251947-5837295 & M7.5 & & $13.74$ & $13.06$ & $12.56$ & & $12.26$ & $11.96$ & & $102.2 \pm 3.4$ & $-25.0 \pm 7.3$ & THA  & $99.8$ & $< 0.1$\\
02265658-5327032 & M9.5 & & $15.40$ & $14.35$ & $13.75$ & & $13.24$ & $12.83$ & & $100.0 \pm 3.8$ & $-6.9 \pm 7.5$ & THA  & $99.9$ & $< 0.1$\\
02294869-6906044 & M5.2 & & $11.93$ & $11.37$ & $11.06$ & & $10.88$ & $10.66$ & & $91.6 \pm 2.5$ & $1.0 \pm 8.2$ & THA  & $99.8$ & $< 0.1$\\
02321934-5746117 & M4.0 & & $11.10$ & $10.53$ & $10.23$ & & $10.03$ & $9.84$ & & $85.9 \pm 3.1$ & $-12.2 \pm 6.4$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
02330550-7023148 & M5.3 & & $12.56$ & $11.97$ & $11.67$ & & $11.49$ & $11.26$ & & $54.6 \pm 1.8$ & $2.9 \pm 7.4$ & THA & $15.0$ & $< 0.1$\\
02340093-6442068 & M9.7 & & $15.32$ & $14.44$ & $13.85$ & & $13.27$ & $12.93$ & & $97.7 \pm 3.1$ & $-19.7 \pm 7.8$ & THA  & $99.3$ & $< 0.1$\\
02401209-5305527 & M8.2 & & $14.39$ & $13.65$ & $13.16$ & & $12.75$ & $12.39$ & & $98.7 \pm 3.7$ & $-6.9 \pm 6.6$ & THA  & $99.9$ & $< 0.1$\\
02405344-1724188 & M5.4 & & $12.44$ & $11.85$ & $11.53$ & & $11.33$ & $11.11$ & & $76.9 \pm 6.4$ & $-42.0 \pm 6.1$ & THA  & $96.7$ & $< 0.1$\\
02410564-5511466 & M9.7 & & $15.39$ & $14.33$ & $13.74$ & & $13.21$ & $12.84$ & & $102.7 \pm 3.7$ & $-15.1 \pm 7.4$ & THA  & $99.9$ & $< 0.1$\\
02411151-0326587 & L1.0 & & $15.80$ & $14.81$ & $14.03$ & & $13.65$ & $13.28$ & & $76.3 \pm 8.5$ & $-39.1 \pm 11.9$ & THA & $92.2$ & $< 0.1$\\
02422401-6533400 & M5.7 & & $12.76$ & $12.19$ & $11.82$ & & $11.61$ & $11.38$ & & $53.8 \pm 2.5$ & $-14.8 \pm 10.9$ & THA & $20.3$ & $< 0.1$\\
02435103-5432194 & M7.9 & & $14.04$ & $13.32$ & $12.78$ & & $12.48$ & $12.15$ & & $104.7 \pm 3.7$ & $-9.4 \pm 7.3$ & THA  & $99.9$ & $< 0.1$\\
02441019-3548036 & M9.4 & & $15.34$ & $14.42$ & $13.79$ & & $13.43$ & $13.16$ & & $66.5 \pm 5.4$ & $-19.2 \pm 7.1$ & THA & $87.1$ & $< 0.1$\\
02483062-5259398 & M4.2 & & $11.25$ & $10.68$ & $10.31$ & & $10.07$ & $9.84$ & & $92.4 \pm 3.5$ & $-4.5 \pm 6.4$ & THA  & $99.8$ & $< 0.1$\\
02494277-6812126 & M5.3 & & $12.46$ & $11.87$ & $11.52$ & & $11.31$ & $11.08$ & & $83.6 \pm 2.4$ & $9.1 \pm 6.5$ & THA  & $99.6$ & $< 0.1$\\
02501167-0151295 & M5.7 & & $12.89$ & $12.28$ & $11.91$ & & $11.71$ & $11.45$ & & $68.7 \pm 6.8$ & $-45.2 \pm 7.0$ & THA & $74.1$ & $< 0.1$\\
02523550-7831183 & M4.7 & & $11.67$ & $11.12$ & $10.78$ & & $10.62$ & $10.40$ & & $84.3 \pm 2.3$ & $20.3 \pm 11.8$ & THA  & $97.4$ & $< 0.1$\\
02543476-5108288\tablenotemark{b} & M4.5 & & $12.07$ & $11.49$ & $11.19$ & & $10.98$ & $10.71$ & & $82.6 \pm 5.3$ & $-5.7 \pm 9.4$ & THA & $99.7$ & $< 0.1$\\
02553178-5702522\tablenotemark{b} & M2.7 & & $11.07$ & $10.52$ & $10.22$ & & $10.06$ & $9.84$ & & $69.0 \pm 3.9$ & $-7.4 \pm 8.7$ & THA\tablenotemark{a} & $98.4$ & $< 0.1$\\
02583123-1520536 & L2.4 & & $15.91$ & $14.87$ & $14.19$ & & $13.64$ & $13.21$ & & $69.0 \pm 7.3$ & $-68.6 \pm 7.0$ & THA & $73.6$ & $< 0.1$\\
03014892-5903021 & M6.4 & & $13.52$ & $12.86$ & $12.31$ & & $11.97$ & $11.66$ & & $79.6 \pm 2.9$ & $2.5 \pm 7.3$ & THA\tablenotemark{a} & $99.9$ & $< 0.1$\\
03032042-7312300 & L2.4 & & $16.14$ & $15.10$ & $14.32$ & & $13.80$ & $13.36$ & & $57.5 \pm 2.0$ & $-0.1 \pm 11.4$ & THA & $70.0$ & $< 0.1$\\
03050556-5317182 & M4.1 & & $11.14$ & $10.58$ & $10.26$ & & $10.08$ & $9.86$ & & $79.3 \pm 3.3$ & $-18.6 \pm 6.5$ & THA\tablenotemark{a} & $99.2$ & $< 0.1$\\
03093877-3014352 & M4.8 & & $11.58$ & $11.04$ & $10.70$ & & $10.49$ & $10.27$ & & $88.2 \pm 6.3$ & $-17.7 \pm 8.1$ & THA  & $99.5$ & $< 0.1$\\
03114544-4719501 & M3.5 & & $10.44$ & $9.89$ & $9.57$ & & $9.39$ & $9.19$ & & $85.6 \pm 5.2$ & $-12.9 \pm 6.4$ & THA\tablenotemark{a} & $99.8$ & $< 0.1$\\
03152363-5342539 & M4.2 & & $11.28$ & $10.71$ & $10.36$ & & $10.19$ & $9.98$ & & $80.6 \pm 3.5$ & $-4.0 \pm 7.2$ & THA\tablenotemark{a} & $99.8$ & $< 0.1$\\
03164512-2848521 & L0.0 & & $14.58$ & $13.77$ & $13.11$ & & $12.66$ & $12.32$ & & $101.4 \pm 7.1$ & $-89.7 \pm 7.9$ & ABDMG  & $83.5$ & $4.5$\\
03204919-3313400 & M5.7 & & $12.54$ & $11.91$ & $11.62$ & & $11.39$ & $11.13$ & & $86.0 \pm 6.3$ & $-23.3 \pm 6.1$ & THA  & $99.7$ & $< 0.1$\\
03224622-7940595 & M5.2 & & $12.22$ & $11.63$ & $11.34$ & & $11.15$ & $10.91$ & & $74.0 \pm 1.9$ & $7.8 \pm 6.8$ & THA & $58.9$ & $< 0.1$\\
03231002-4631237 & M9.1 & & $15.39$ & $14.32$ & $13.70$ & & $13.09$ & $12.68$ & & $73.4 \pm 5.2$ & $0.5 \pm 7.4$ & THA\tablenotemark{a} & $99.6$ & $< 0.1$\\
03252938-4312299 & M7.5 & & $14.18$ & $13.43$ & $12.91$ & & $12.61$ & $12.32$ & & $55.3 \pm 6.5$ & $-10.9 \pm 7.3$ & THA  & $79.7$ & $< 0.1$\\
03264225-2102057 & L3.6 & & $16.13$ & $14.79$ & $13.92$ & & $12.96$ & $12.45$ & & $93.1 \pm 8.5$ & $-139.3 \pm 9.8$ & ABDMG\tablenotemark{a} & $96.1$ & $1.2$\\
03283347-6236225 & M5.1 & & $11.89$ & $11.31$ & $11.01$ & & $10.84$ & $10.62$ & & $82.8 \pm 2.7$ & $16.6 \pm 6.5$ & THA  & $99.7$ & $< 0.1$\\
03363144-2619578 & M3.6 & & $10.68$ & $10.13$ & $9.76$ & & $9.56$ & $9.32$ & & $76.5 \pm 6.0$ & $-30.5 \pm 6.0$ & THA  & $99.4$ & $< 0.1$\\
03393521-3525440 & M7.8 & & $10.73$ & $10.02$ & $9.55$ & & $9.13$ & $8.80$ & & $308.4 \pm 14.0$ & $279.5 \pm 13.8$ & ARG  & $84.1$ & $13.8$\\
03420931-2904317 & L2.3 & & $15.92$ & $15.35$ & $14.38$ & & $13.98$ & $13.58$ & & $74.5 \pm 6.7$ & $-16.1 \pm 8.0$ & THA  & $99.2$ & $< 0.1$\\
03421621-6817321 & L3.0 & & $16.85$ & $15.39$ & $14.54$ & & $13.95$ & $13.48$ & & $73.7 \pm 2.3$ & $20.6 \pm 7.8$ & THA\tablenotemark{a} & $99.6$ & $< 0.1$\\
03441258-3716463 & M5.8 & & $13.00$ & $12.41$ & $12.02$ & & $11.80$ & $11.54$ & & $74.5 \pm 5.6$ & $-14.9 \pm 7.2$ & THA  & $99.5$ & $< 0.1$\\
03445673-1145126\tablenotemark{b} & M4.0 & & $12.01$ & $11.42$ & $11.11$ & & $10.88$ & $10.68$ & & $55.2 \pm 8.9$ & $-49.5 \pm 9.0$ & BPMG & $75.2$ & $< 0.1$\\
03552337+1133437 & L3.7 & & $14.05$ & $12.53$ & $11.53$ & & $10.53$ & $9.94$ & & $226.8 \pm 12.2$ & $-623.7 \pm 17.9$ & ABDMG\tablenotemark{a} & $69.5$ & $12.7$\\
03572695-4417305 & M7.8 & & $14.37$ & $13.53$ & $12.91$ & & $12.49$ & $12.10$ & & $75.1 \pm 5.2$ & $-1.0 \pm 6.5$ & THA\tablenotemark{a} & $99.8$ & $< 0.1$\\
04094585-3923319 & M6.4 & & $13.48$ & $12.85$ & $12.45$ & & $12.21$ & $11.94$ & & $65.1 \pm 5.9$ & $-2.2 \pm 8.1$ & THA  & $97.5$ & $< 0.1$\\
04174743-2129191\tablenotemark{b} & M6.9 & & $13.89$ & $13.15$ & $12.67$ & & $12.39$ & $12.21$ & & $82.7 \pm 8.5$ & $0.4 \pm 9.7$ & THA & $60.8$ & $< 0.1$\\
04182880-0533019 & L3.8 & & $16.54$ & $15.52$ & $14.57$ & & $13.90$ & $13.51$ & & $109.9 \pm 12.2$ & $-41.9 \pm 10.5$ & COL & $29.0$ & $7.4$\\
04185879-4507413 & L2.5 & & $16.16$ & $15.05$ & $14.60$ & & $13.86$ & $13.46$ & & $57.6 \pm 5.8$ & $-5.7 \pm 8.4$ & THA  & $87.2$ & $< 0.1$\\
04210718-6306022 & L6.1 & & $15.56$ & $14.28$ & $13.45$ & & $12.58$ & $12.16$ & & $151.6 \pm 3.6$ & $209.7 \pm 7.4$ & BPMG  & $94.6$ & $12.4$\\
04273598-2316586\tablenotemark{b} & M2.5 & & $10.47$ & $9.86$ & $9.58$ & & $9.41$ & $9.19$ & & $59.4 \pm 7.2$ & $-19.6 \pm 7.9$ & COL\tablenotemark{a} & $95.0$ & $10.1$\\
04341693-2526468 & M3.9 & & $11.35$ & $10.77$ & $10.48$ & & $10.30$ & $10.08$ & & $42.8 \pm 5.9$ & $-11.4 \pm 6.8$ & COL\tablenotemark{a} & $90.5$ & $13.7$\\
04362788-4114465 & M6.4 & & $13.10$ & $12.43$ & $12.05$ & & $11.75$ & $11.47$ & & $60.9 \pm 4.2$ & $15.2 \pm 6.2$ & COL  & $95.1$ & $9.6$\\
04380868-4342484 & M5.0 & & $12.31$ & $11.76$ & $11.40$ & & $11.24$ & $11.01$ & & $42.7 \pm 4.5$ & $12.9 \pm 8.4$ & COL  & $87.8$ & $14.6$\\
04400972-5126544 & M9.4 & & $15.69$ & $14.78$ & $14.17$ & & $13.60$ & $13.20$ & & $51.2 \pm 4.3$ & $14.5 \pm 6.8$ & THA  & $80.5$ & $< 0.1$\\
04433761+0002051 & M7.7 & & $12.51$ & $11.80$ & $11.22$ & & $10.83$ & $10.48$ & & $50.1 \pm 7.0$ & $-101.5 \pm 8.6$ & BPMG\tablenotemark{a} & $98.7$ & $7.4$\\
04532647-1751543 & M8.8 & & $15.14$ & $14.06$ & $13.47$ & & $12.95$ & $12.61$ & & $39.1 \pm 6.5$ & $-21.1 \pm 6.2$ & COL\tablenotemark{a} & $95.6$ & $7.8$\\
04533604-2835349 & M3.7 & & $10.17$ & $9.61$ & $9.30$ & & $9.15$ & $8.93$ & & $37.0 \pm 4.9$ & $-6.3 \pm 6.0$ & COL  & $93.9$ & $11.3$\\
05002100+0330501 & L2.3 & & $13.67$ & $12.68$ & $12.06$ & & $11.51$ & $11.24$ & & $24.4 \pm 7.8$ & $-356.5 \pm 12.4$ & ABDMG  & $33.5$ & $2.0$\\
05071673-2352431 & M5.1 & & $12.16$ & $11.61$ & $11.26$ & & $11.09$ & $10.87$ & & $39.2 \pm 5.5$ & $-13.3 \pm 7.7$ & COL  & $94.8$ & $11.2$\\
05120921-1807415 & M5.4 & & $12.68$ & $12.15$ & $11.79$ & & $11.62$ & $11.38$ & & $37.6 \pm 7.3$ & $-16.8 \pm 7.8$ & COL & $88.1$ & $14.2$\\
05123569-3041067 & M4.6 & & $11.90$ & $11.33$ & $10.99$ & & $10.79$ & $10.54$ & & $37.1 \pm 5.0$ & $0.6 \pm 6.1$ & COL  & $95.0$ & $11.5$\\
05130001-1611177 & M4.3 & & $11.64$ & $11.04$ & $10.74$ & & $10.56$ & $10.31$ & & $39.7 \pm 5.9$ & $-19.3 \pm 6.8$ & COL  & $88.8$ & $12.5$\\
05181131-3101529 & M5.0 & & $11.88$ & $11.23$ & $10.90$ & & $10.65$ & $10.40$ & & $46.1 \pm 4.9$ & $4.0 \pm 6.1$ & COL\tablenotemark{a} & $93.6$ & $8.1$\\
05264316-1824315 & M5.3 & & $12.36$ & $11.84$ & $11.45$ & & $11.23$ & $10.96$ & & $29.6 \pm 6.5$ & $-25.1 \pm 6.9$ & COL & $91.4$ & $14.1$\\
05284789-2909077 & M4.5 & & $11.77$ & $11.22$ & $10.89$ & & $10.70$ & $10.45$ & & $31.9 \pm 5.0$ & $-0.3 \pm 6.9$ & COL  & $94.0$ & $12.1$\\
05313142-4323042 & M4.0 & & $10.74$ & $10.13$ & $9.84$ & & $9.67$ & $9.45$ & & $41.5 \pm 4.1$ & $19.2 \pm 7.5$ & COL\tablenotemark{a} & $86.3$ & $11.4$\\
05361998-1920396 & L3.1 & & $15.77$ & $14.69$ & $13.85$ & & $13.26$ & $12.76$ & & $29.7 \pm 6.1$ & $-27.3 \pm 6.6$ & COL\tablenotemark{a} & $97.1$ & $7.4$\\
05400823-3642181 & L2.3 & & $16.08$ & $15.05$ & $14.51$ & & $13.98$ & $13.61$ & & $36.9 \pm 6.0$ & $11.0 \pm 8.5$ & COL & $82.9$ & $12.3$\\
05432117-2204024 & M5.6 & & $11.95$ & $11.37$ & $11.01$ & & $10.76$ & $10.55$ & & $50.9 \pm 5.7$ & $-11.3 \pm 6.2$ & COL & $70.2$ & $13.8$\\
05461532-5547521 & M5.2 & & $11.38$ & $10.81$ & $10.48$ & & $10.32$ & $10.09$ & & $38.3 \pm 2.9$ & $45.6 \pm 6.7$ & CAR  & $93.7$ & $5.2$\\
05490552-4832344 & M4.4 & & $11.31$ & $10.73$ & $10.39$ & & $10.24$ & $10.02$ & & $26.9 \pm 3.8$ & $37.0 \pm 6.7$ & COL  & $78.7$ & $12.4$\\
05504281-5308392 & M3.6 & & $10.22$ & $9.65$ & $9.34$ & & $9.15$ & $8.99$ & & $28.2 \pm 2.9$ & $33.9 \pm 6.6$ & CAR\tablenotemark{a} & $81.6$ & $9.9$\\
06022216+6336391 & M9.7 & & $14.27$ & $13.36$ & $12.68$ & & $12.22$ & $11.95$ & & $-17.0 \pm 2.0$ & $-230.8 \pm 8.4$ & ABDMG  & $30.5$ & $12.9$\\
06272161-5308428\tablenotemark{b} & L5.3 & & $16.39$ & $15.23$ & $14.69$ & & $13.88$ & $13.50$ & & $10.4 \pm 6.6$ & $65.1 \pm 12.3$ & CAR & $65.9$ & $9.6$\\
06420559+4101599 & L6.2 & & $16.16$ & $15.09$ & $14.28$ & & $13.37$ & $12.60$ & & $0.9 \pm 4.7$ & $-375.7 \pm 11.6$ & ABDMG  & $38.4$ & $4.5$\\
06513251-6528322 & M7.6 & & $14.78$ & $14.14$ & $13.67$ & & $13.46$ & $13.16$ & & $5.4 \pm 1.6$ & $35.6 \pm 6.2$ & CAR  & $84.4$ & $5.0$\\
06524851-5741376 & M7.3 & & $13.63$ & $12.97$ & $12.45$ & & $12.17$ & $11.87$ & & $1.1 \pm 2.5$ & $40.5 \pm 6.8$ & CAR  & $97.4$ & $2.8$\\
06561550-5728017 & M5.9 & & $13.08$ & $12.48$ & $12.07$ & & $11.87$ & $11.64$ & & $-4.8 \pm 2.5$ & $37.0 \pm 6.8$ & CAR  & $48.2$ & $9.0$\\
07013784-6411369 & M5.4 & & $12.70$ & $12.13$ & $11.79$ & & $11.58$ & $11.36$ & & $8.7 \pm 1.7$ & $36.3 \pm 6.1$ & CAR & $10.4$ & $8.2$\\
07105337-7431070\tablenotemark{b} & L0.0 & & $14.55$ & $13.79$ & $13.23$ & & $12.90$ & $12.58$ & & $-7.9 \pm 2.3$ & $115.0 \pm 10.1$ & CAR & $67.4$ & $4.0$\\
07485518-6721360 & M3.8 & & $10.87$ & $10.35$ & $10.01$ & & $9.83$ & $9.61$ & & $-16.3 \pm 1.7$ & $59.7 \pm 7.1$ & CAR\tablenotemark{a} & $99.4$ & $1.4$\\
08025781-8330076 & M5.4 & & $10.67$ & $10.04$ & $9.71$ & & $9.48$ & $9.30$ & & $-108.4 \pm 2.6$ & $143.0 \pm 8.2$ & BPMG  & $94.5$ & $8.6$\\
08035086-7344331 & M3.7 & & $11.58$ & $11.02$ & $10.69$ & & $10.52$ & $10.30$ & & $-10.1 \pm 1.1$ & $42.4 \pm 6.9$ & CAR\tablenotemark{a} & $95.4$ & $2.4$\\
08063045-6809212 & M3.8 & & $11.90$ & $11.33$ & $11.05$ & & $10.87$ & $10.64$ & & $-8.2 \pm 1.5$ & $34.2 \pm 6.9$ & CAR\tablenotemark{a} & $82.8$ & $4.6$\\
08144321+2336045\tablenotemark{b} & M4.5 & & $10.94$ & $10.40$ & $10.08$ & & $9.91$ & $9.73$ & & $-53.7 \pm 6.9$ & $-128.5 \pm 8.0$ & TWA & $11.9$ & $7.9$\\
08173829-6817162 & M3.8 & & $10.36$ & $9.81$ & $9.47$ & & $9.20$ & $8.99$ & & $-15.6 \pm 1.6$ & $58.1 \pm 7.1$ & CAR & $35.0$ & $3.1$\\
09532126-1014205 & M7.4 & & $13.47$ & $12.64$ & $12.14$ & & $11.77$ & $11.41$ & & $-72.8 \pm 6.2$ & $-67.7 \pm 6.3$ & CAR\tablenotemark{a} & $65.0$ & $8.3$\\
10212570-2830427 & L4.0 & & $16.91$ & $15.85$ & $14.98$ & & $14.18$ & $13.73$ & & $-54.5 \pm 9.8$ & $-34.7 \pm 12.4$ & TWA  & $88.6$ & $1.4$\\
10284580-2830374 & M4.1 & & $10.95$ & $10.41$ & $10.03$ & & $9.48$ & $8.99$ & & $-68.9 \pm 5.0$ & $-20.3 \pm 6.0$ & TWA  & $95.0$ & $0.9$\\
10513331-1916530 & M9.1 & & $14.69$ & $13.95$ & $13.43$ & & $13.10$ & $12.82$ & & $-93.8 \pm 6.4$ & $-29.6 \pm 6.6$ & TWA  & $42.4$ & $5.5$\\
10554602-8216412 & M5.3 & & $13.47$ & $12.83$ & $12.46$ & & $12.22$ & $11.96$ & & $-44.9 \pm 1.2$ & $31.0 \pm 7.8$ & CAR\tablenotemark{a} & $10.8$ & $11.7$\\
10571669-3512548 & M5.8 & & $13.41$ & $12.78$ & $12.44$ & & $12.18$ & $11.92$ & & $-36.5 \pm 4.6$ & $-5.9 \pm 6.3$ & TWA  & $35.7$ & $10.2$\\
10585054-2346206 & M3.8 & & $10.30$ & $9.71$ & $9.43$ & & $9.21$ & $8.97$ & & $-92.3 \pm 5.3$ & $-15.5 \pm 6.4$ & TWA\tablenotemark{a} & $50.4$ & $4.4$\\
11020983-3430355 & M7.0 & & $13.03$ & $12.36$ & $11.89$ & & $11.45$ & $10.81$ & & $-65.2 \pm 4.7$ & $-15.6 \pm 6.1$ & TWA\tablenotemark{a} & $99.3$ & $0.4$\\
11035165-3711483 & M5.3 & & $12.42$ & $11.84$ & $11.54$ & & $11.34$ & $11.11$ & & $-76.4 \pm 4.7$ & $1.0 \pm 6.3$ & TWA & $84.8$ & $0.9$\\
11035873-4156475 & M5.8 & & $13.54$ & $13.03$ & $12.58$ & & $12.38$ & $12.11$ & & $-30.9 \pm 4.3$ & $-14.3 \pm 7.8$ & TWA & $34.4$ & $13.3$\\
11064461-3715115 & M7.5 & & $14.49$ & $13.85$ & $13.34$ & & $13.09$ & $12.76$ & & $-45.9 \pm 4.6$ & $-4.9 \pm 6.4$ & TWA & $92.9$ & $1.8$\\
11112820-2655027 & M3.8 & & $10.33$ & $9.81$ & $9.45$ & & $9.24$ & $8.97$ & & $-87.4 \pm 5.3$ & $-29.7 \pm 6.0$ & TWA  & $97.8$ & $1.5$\\
11112984-2713320 & M4.9 & & $11.80$ & $11.21$ & $10.90$ & & $10.70$ & $10.50$ & & $-63.1 \pm 5.2$ & $-32.9 \pm 6.1$ & TWA  & $93.3$ & $1.7$\\
11153797-2552192 & M5.3 & & $12.33$ & $11.77$ & $11.46$ & & $11.27$ & $11.07$ & & $-70.5 \pm 6.2$ & $-7.0 \pm 6.2$ & TWA  & $13.2$ & $6.7$\\
11385038-3830011 & M5.4 & & $12.98$ & $12.42$ & $12.10$ & & $11.90$ & $11.71$ & & $-55.3 \pm 4.9$ & $6.6 \pm 6.3$ & TWA & $17.7$ & $2.9$\\
11393382-3040002 & M3.9 & & $9.98$ & $9.41$ & $9.12$ & & $8.82$ & $8.46$ & & $-79.9 \pm 5.7$ & $-30.0 \pm 6.8$ & TWA\tablenotemark{a} & $98.7$ & $1.3$\\
11394506-3729069 & M5.2 & & $12.90$ & $12.32$ & $12.02$ & & $11.84$ & $11.60$ & & $-38.4 \pm 4.6$ & $-19.5 \pm 6.3$ & TWA & $83.4$ & $3.1$\\
11395113-3159214 & M5.7 & & $12.69$ & $12.00$ & $11.50$ & & $11.17$ & $10.82$ & & $-91.8 \pm 6.6$ & $-20.5 \pm 6.7$ & TWA\tablenotemark{a} & $98.4$ & $0.8$\\
11480096-2836488 & L1.9 & & $16.11$ & $15.19$ & $14.56$ & & $14.16$ & $13.85$ & & $-87.4 \pm 9.5$ & $-13.6 \pm 10.4$ & TWA & $45.6$ & $4.6$\\
11510246-3611457 & M5.3 & & $11.21$ & $10.61$ & $10.32$ & & $10.11$ & $9.93$ & & $-150.8 \pm 8.6$ & $-55.1 \pm 7.2$ & TWA  & $62.1$ & $2.9$\\
12035905-3821402 & M5.9 & & $13.77$ & $13.12$ & $12.69$ & & $12.42$ & $12.11$ & & $-51.9 \pm 4.9$ & $-22.8 \pm 6.5$ & TWA\tablenotemark{a} & $99.3$ & $1.0$\\
12073346-3932539 & M5.3 & & $12.99$ & $12.39$ & $11.94$ & & $11.57$ & $11.02$ & & $-56.1 \pm 4.7$ & $-25.8 \pm 6.3$ & TWA\tablenotemark{a} & $99.0$ & $0.4$\\
12074836-3900043 & M9.2 & & $15.49$ & $14.61$ & $14.04$ & & $13.64$ & $13.20$ & & $-66.9 \pm 5.7$ & $-31.2 \pm 6.9$ & TWA & $99.4$ & $0.7$\\
12134001-3723362 & M5.1 & & $12.92$ & $12.31$ & $12.00$ & & $11.80$ & $11.60$ & & $-46.8 \pm 4.8$ & $-9.6 \pm 6.3$ & TWA & $86.0$ & $2.7$\\
12174683-3804157 & M5.2 & & $12.90$ & $12.32$ & $11.96$ & & $11.78$ & $11.57$ & & $-56.7 \pm 5.0$ & $-0.4 \pm 6.3$ & TWA & $20.5$ & $3.3$\\
12175920-3734433 & M3.8 & & $11.57$ & $10.99$ & $10.72$ & & $10.54$ & $10.30$ & & $-54.6 \pm 4.9$ & $-23.8 \pm 6.3$ & TWA\tablenotemark{a} & $98.6$ & $1.0$\\
12214223-4012050\tablenotemark{b} & L3.4 & & $16.47$ & $15.58$ & $15.03$ & & $14.31$ & $14.08$ & & $-92.0 \pm 12.4$ & $-44.6 \pm 20.5$ & TWA & $79.1$ & $1.2$\\
12310489-3801065\tablenotemark{b} & M7.1 & & $14.68$ & $14.09$ & $13.53$ & & $13.37$ & $13.14$ & & $-62.5 \pm 7.5$ & $-6.0 \pm 10.1$ & TWA & $73.8$ & $1.9$\\
12474428-3816464 & M7.6 & & $14.78$ & $14.10$ & $13.57$ & & $13.12$ & $12.53$ & & $-35.8 \pm 4.7$ & $-21.2 \pm 6.5$ & TWA\tablenotemark{a} & $40.2$ & $7.6$\\
12535039-4211215 & M9.0 & & $16.00$ & $15.30$ & $14.74$ & & $14.28$ & $13.93$ & & $-46.1 \pm 6.5$ & $-9.0 \pm 9.5$ & TWA & $50.7$ & $5.4$\\
12563961-2718455\tablenotemark{b} & L3.7 & & $16.42$ & $15.37$ & $14.71$ & & $14.09$ & $13.69$ & & $-67.4 \pm 10.2$ & $-56.5 \pm 12.7$ & TWA & $12.1$ & $14.6$\\
12574941-4111373 & M5.0 & & $13.02$ & $12.46$ & $12.09$ & & $11.88$ & $11.64$ & & $-40.5 \pm 4.4$ & $-22.3 \pm 6.4$ & TWA & $60.0$ & $4.5$\\
13155594-3403418 & M5.4 & & $13.10$ & $12.54$ & $12.22$ & & $12.02$ & $11.82$ & & $-52.9 \pm 5.2$ & $-24.8 \pm 6.4$ & TWA & $10.9$ & $10.2$\\
14252798-3650229 & L3.2 & & $13.75$ & $12.57$ & $11.81$ & & $11.04$ & $10.57$ & & $-273.1 \pm 7.8$ & $-474.0 \pm 12.8$ & ABDMG\tablenotemark{a} & $78.7$ & $1.1$\\
19010688-7115248 & M5.3 & & $12.78$ & $12.23$ & $11.88$ & & $11.70$ & $11.50$ & & $-17.7 \pm 1.5$ & $-80.2 \pm 9.0$ & THA  & $26.1$ & $< 0.1$\\
19075853-8324093 & M5.4 & & $12.92$ & $12.34$ & $11.97$ & & $11.77$ & $11.52$ & & $-21.3 \pm 0.7$ & $-65.4 \pm 8.3$ & THA  & $11.0$ & $< 0.1$\\
19350976-6200473 & L1.7 & & $16.25$ & $15.29$ & $14.72$ & & $14.04$ & $13.68$ & & $-5.8 \pm 3.1$ & $-69.7 \pm 11.4$ & THA & $13.4$ & $0.1$\\
19395435-5216468 & L1.3 & & $14.66$ & $13.86$ & $13.27$ & & $12.89$ & $12.59$ & & $77.1 \pm 3.7$ & $-135.7 \pm 7.6$ & BPMG  & $57.9$ & $11.8$\\
19444417-4359015 & M4.9 & & $10.66$ & $10.14$ & $9.71$ & & $9.51$ & $9.30$ & & $47.4 \pm 3.9$ & $-148.9 \pm 7.3$ & BPMG\tablenotemark{a} & $86.4$ & $7.7$\\
19514573-6641061 & M5.2 & & $12.42$ & $11.85$ & $11.49$ & & $11.33$ & $11.09$ & & $-4.4 \pm 1.8$ & $-81.3 \pm 10.9$ & THA  & $59.9$ & $< 0.1$\\
19564700-7542270 & L1.8 & & $16.15$ & $15.04$ & $14.23$ & & $13.70$ & $13.27$ & & $9.7 \pm 1.4$ & $-76.9 \pm 10.7$ & THA\tablenotemark{a} & $77.5$ & $< 0.1$\\
20004841-7523070 & M7.0 & & $12.73$ & $11.97$ & $11.51$ & & $11.13$ & $10.81$ & & $59.0 \pm 1.8$ & $-117.6 \pm 8.4$ & BPMG\tablenotemark{a} & $97.8$ & $13.1$\\
20092431-6330508 & M4.3 & & $11.42$ & $10.86$ & $10.56$ & & $10.38$ & $10.15$ & & $12.3 \pm 2.1$ & $-101.9 \pm 7.5$ & THA\tablenotemark{a} & $79.9$ & $< 0.1$\\
20113196-5048112 & L2.5 & & $16.42$ & $15.26$ & $14.58$ & & $14.02$ & $13.60$ & & $19.1 \pm 4.6$ & $-86.4 \pm 9.3$ & THA  & $28.1$ & $< 0.1$\\
20224803-5645567 & M4.6 & & $11.76$ & $11.24$ & $10.83$ & & $10.65$ & $10.40$ & & $4.8 \pm 2.5$ & $-89.7 \pm 7.6$ & THA\tablenotemark{a} & $66.1$ & $< 0.1$\\
20282203-5637024 & M6.6 & & $13.84$ & $13.24$ & $12.71$ & & $12.49$ & $12.19$ & & $24.3 \pm 3.0$ & $-75.3 \pm 7.6$ & THA & $30.0$ & $< 0.1$\\
20291446-5456116 & M4.2 & & $11.23$ & $10.64$ & $10.36$ & & $10.18$ & $9.96$ & & $8.6 \pm 3.0$ & $-109.6 \pm 7.7$ & THA\tablenotemark{a} & $38.5$ & $< 0.1$\\
20330186-4903105 & M5.2 & & $10.11$ & $9.52$ & $9.19$ & & $8.99$ & $8.77$ & & $115.1 \pm 4.4$ & $-208.0 \pm 8.0$ & BPMG  & $91.3$ & $5.5$\\
20334473-5635338\tablenotemark{b} & M9.8 & & $15.72$ & $15.14$ & $14.24$ & & $13.82$ & $13.41$ & & $16.0 \pm 6.1$ & $-73.1 \pm 12.5$ & THA & $49.8$ & $< 0.1$\\
20334670-3733443 & M4.6 & & $10.85$ & $10.30$ & $9.96$ & & $9.76$ & $9.51$ & & $74.3 \pm 4.4$ & $-102.9 \pm 7.0$ & BPMG  & $89.1$ & $13.8$\\
20423672-5425263 & M3.5 & & $10.75$ & $10.16$ & $9.86$ & & $9.71$ & $9.48$ & & $18.1 \pm 3.0$ & $-94.6 \pm 8.3$ & THA\tablenotemark{a} & $83.1$ & $< 0.1$\\
20430452-5547114 & M5.3 & & $12.30$ & $11.71$ & $11.41$ & & $11.22$ & $11.00$ & & $9.3 \pm 2.9$ & $-88.4 \pm 7.5$ & THA  & $68.6$ & $< 0.1$\\
20452795-7717561 & M5.7 & & $13.14$ & $12.56$ & $12.14$ & & $11.88$ & $11.65$ & & $23.3 \pm 1.1$ & $-71.8 \pm 8.3$ & THA  & $80.0$ & $< 0.1$\\
20484222-5127435 & M9.4 & & $15.38$ & $14.51$ & $13.88$ & & $13.41$ & $13.11$ & & $44.1 \pm 3.6$ & $-92.8 \pm 7.4$ & THA  & $25.6$ & $< 0.1$\\
21083826-4244540 & M3.3 & & $10.14$ & $9.57$ & $9.24$ & & $9.08$ & $8.86$ & & $35.8 \pm 3.9$ & $-99.2 \pm 6.7$ & THA\tablenotemark{a} & $46.4$ & $< 0.1$\\
21102873-5540391 & M9.2 & & $15.44$ & $14.60$ & $13.93$ & & $13.51$ & $13.22$ & & $25.6 \pm 3.2$ & $-70.3 \pm 8.1$ & THA & $60.8$ & $< 0.1$\\
21121598-8128452\tablenotemark{b} & M2.4 & & $10.67$ & $10.08$ & $9.70$ & & $9.55$ & $9.34$ & & $48.7 \pm 1.1$ & $-101.7 \pm 10.2$ & THA & $40.4$ & $< 0.1$\\
21143529-6124082 & M5.7 & & $12.91$ & $12.34$ & $11.92$ & & $11.68$ & $11.42$ & & $20.1 \pm 2.3$ & $-76.6 \pm 7.2$ & THA  & $85.4$ & $< 0.1$\\
21192028-8145446 & M4.1 & & $11.14$ & $10.56$ & $10.21$ & & $10.05$ & $9.82$ & & $48.4 \pm 1.4$ & $-106.0 \pm 9.3$ & THA\tablenotemark{a} & $35.7$ & $< 0.1$\\
21265040-8140293 & L1.9 & & $15.54$ & $14.40$ & $13.55$ & & $12.93$ & $12.47$ & & $46.7 \pm 1.3$ & $-107.8 \pm 10.4$ & THA\tablenotemark{a} & $64.1$ & $< 0.1$\\
21490499-6413039 & M3.4 & & $10.35$ & $9.80$ & $9.47$ & & $9.29$ & $9.08$ & & $41.3 \pm 2.1$ & $-101.2 \pm 8.5$ & THA\tablenotemark{a} & $97.8$ & $< 0.1$\\
21503682-7023414\tablenotemark{b} & M4.3 & & $12.20$ & $11.65$ & $11.30$ & & $11.13$ & $10.91$ & & $19.1 \pm 1.5$ & $-71.0 \pm 7.4$ & THA & $39.9$ & $< 0.1$\\
21544859-7459134 & M8.0 & & $14.29$ & $13.57$ & $13.08$ & & $12.72$ & $12.39$ & & $54.3 \pm 1.7$ & $-89.8 \pm 9.5$ & THA  & $98.2$ & $< 0.1$\\
22025794-5605087 & M8.0 & & $14.36$ & $13.62$ & $13.16$ & & $12.84$ & $12.57$ & & $53.3 \pm 3.1$ & $-78.7 \pm 7.1$ & THA & $95.5$ & $< 0.1$\\
22060961-0723353 & M5.3 & & $10.67$ & $10.06$ & $9.76$ & & $9.55$ & $9.35$ & & $172.2 \pm 9.6$ & $-216.8 \pm 7.5$ & ABDMG  & $90.4$ & $1.1$\\
22064498-4217208 & L3.2 & & $15.56$ & $14.45$ & $13.61$ & & $12.86$ & $12.40$ & & $132.6 \pm 4.8$ & $-187.7 \pm 9.3$ & ABDMG\tablenotemark{a} & $96.0$ & $1.3$\\
22244102-7724036 & M4.2 & & $11.42$ & $10.81$ & $10.53$ & & $10.33$ & $10.12$ & & $56.8 \pm 1.6$ & $-74.9 \pm 12.8$ & THA\tablenotemark{a} & $98.2$ & $< 0.1$\\
22283837-3648372 & M5.3 & & $11.77$ & $11.18$ & $10.90$ & & $10.69$ & $10.51$ & & $84.5 \pm 4.9$ & $-125.0 \pm 7.1$ & ABDMG  & $28.9$ & $13.7$\\
22320782-8308108 & M9.4 & & $15.80$ & $14.98$ & $14.17$ & & $13.72$ & $13.33$ & & $53.7 \pm 1.5$ & $-43.8 \pm 8.0$ & THA  & $41.3$ & $< 0.1$\\
22351658-3844154 & M9.3 & & $15.18$ & $14.27$ & $13.63$ & & $13.03$ & $12.62$ & & $58.1 \pm 4.8$ & $-88.8 \pm 7.7$ & THA  & $90.8$ & $< 0.1$\\
22353560-5906306 & M8.1 & & $14.28$ & $13.59$ & $13.17$ & & $12.71$ & $12.38$ & & $68.2 \pm 3.2$ & $-90.5 \pm 7.5$ & THA  & $99.1$ & $< 0.1$\\
22400144+0532162 & M5.3 & & $11.72$ & $11.09$ & $10.75$ & & $10.52$ & $10.30$ & & $112.6 \pm 9.2$ & $-134.2 \pm 10.2$ & ABDMG  & $71.8$ & $4.4$\\
22443167+2043433 & L5.9 & & $16.48$ & $15.00$ & $14.02$ & & $12.79$ & $12.13$ & & $236.6 \pm 7.7$ & $-234.8 \pm 8.3$ & ABDMG  & $98.1$ & $0.6$\\
22444835-6650032 & M3.8 & & $11.03$ & $10.41$ & $10.14$ & & $9.93$ & $9.69$ & & $65.2 \pm 2.2$ & $-71.4 \pm 8.4$ & THA\tablenotemark{a} & $99.5$ & $< 0.1$\\
22511530-6811216 & M5.3 & & $12.10$ & $11.59$ & $11.24$ & & $11.03$ & $10.79$ & & $58.4 \pm 2.0$ & $-74.2 \pm 8.4$ & THA  & $99.6$ & $< 0.1$\\
22583200+1014589 & M4.9 & & $10.39$ & $9.80$ & $9.50$ & & $9.29$ & $9.08$ & & $163.1 \pm 9.3$ & $-182.9 \pm 8.2$ & ABDMG  & $92.3$ & $1.2$\\
23051517-3550073 & M4.9 & & $11.80$ & $11.17$ & $10.81$ & & $10.59$ & $10.40$ & & $59.0 \pm 4.4$ & $-64.2 \pm 6.7$ & THA\tablenotemark{a} & $16.3$ & $< 0.1$\\
23130558-6127077 & M3.7 & & $10.93$ & $10.37$ & $10.05$ & & $9.86$ & $9.65$ & & $55.0 \pm 2.6$ & $-73.6 \pm 8.4$ & THA\tablenotemark{a} & $98.0$ & $< 0.1$\\
23155665-4747315 & L2.3 & & $16.08$ & $15.08$ & $14.45$ & & $13.93$ & $13.60$ & & $58.4 \pm 5.2$ & $-53.3 \pm 8.9$ & THA  & $20.5$ & $< 0.1$\\
23221690-6833004 & M3.7 & & $10.93$ & $10.38$ & $10.03$ & & $9.80$ & $9.62$ & & $72.8 \pm 2.3$ & $-55.2 \pm 9.2$ & THA\tablenotemark{a} & $99.2$ & $< 0.1$\\
23225240-6151114 & M4.9 & & $11.53$ & $10.96$ & $10.65$ & & $10.48$ & $10.25$ & & $87.7 \pm 2.9$ & $-77.7 \pm 6.8$ & THA  & $99.5$ & $< 0.1$\\
23225299-6151275 & L0.8 & & $15.55$ & $14.53$ & $13.86$ & & $13.22$ & $12.81$ & & $82.7 \pm 3.0$ & $-74.0 \pm 7.1$ & THA  & $99.9$ & $< 0.1$\\
23233072-2807141 & M4.9 & & $11.41$ & $10.83$ & $10.51$ & & $10.32$ & $10.13$ & & $113.2 \pm 5.9$ & $-110.7 \pm 6.3$ & ABDMG  & $47.4$ & $9.9$\\
23321028-6926537 & M5.3 & & $12.01$ & $11.45$ & $11.14$ & & $10.94$ & $10.71$ & & $88.8 \pm 2.7$ & $-67.8 \pm 8.2$ & THA  & $99.4$ & $< 0.1$\\
23360735-3541489\tablenotemark{b} & M8.9 & & $14.65$ & $13.81$ & $13.39$ & & $13.00$ & $12.65$ & & $69.6 \pm 8.2$ & $-80.7 \pm 9.9$ & THA & $39.2$ & $< 0.1$\\
23392527+3507165 & L3.0 & & $15.36$ & $14.35$ & $13.59$ & & $13.08$ & $12.76$ & & $174.0 \pm 6.4$ & $-33.9 \pm 6.9$ & BPMG & $16.5$ & $13.6$\\
23424333-6224564 & M4.6 & & $11.30$ & $10.76$ & $10.41$ & & $10.25$ & $10.02$ & & $85.3 \pm 2.9$ & $-70.5 \pm 8.4$ & THA  & $99.7$ & $< 0.1$\\
23433470-3646021 & L5.1 & & $16.57$ & $15.01$ & $14.19$ & & $13.14$ & $12.61$ & & $97.1 \pm 6.0$ & $-109.4 \pm 10.1$ & BPMG\tablenotemark{a} & $42.6$ & $5.6$\\
23520507-1100435 & M6.0 & & $12.84$ & $12.17$ & $11.74$ & & $11.46$ & $11.15$ & & $97.2 \pm 6.8$ & $-128.8 \pm 6.5$ & ABDMG & $49.8$ & $6.5$\\
23523223-3413068 & M5.3 & & $11.31$ & $10.72$ & $10.42$ & & $10.23$ & $10.02$ & & $139.5 \pm 6.7$ & $-133.6 \pm 7.8$ & ABDMG  & $79.9$ & $2.7$\\
\cutinhead{Candidates with a Modest Probability}
00160844-0043021 & L4.0 & & $16.33$ & $15.23$ & $14.54$ & & $13.84$ & $13.39$ & & $138.3 \pm 9.9$ & $-33.7 \pm 14.2$ & BPMG & $18.8$ & $36.4$\\
00192626+4614078 & M5.9 & & $12.60$ & $11.94$ & $11.50$ & & $11.28$ & $11.02$ & & $119.6 \pm 6.1$ & $-82.5 \pm 6.9$ & ABDMG  & $53.3$ & $17.5$\\
00274534-0806046 & M5.3 & & $11.57$ & $10.97$ & $10.61$ & & $10.41$ & $10.18$ & & $111.5 \pm 7.0$ & $-59.9 \pm 6.7$ & BPMG & $45.6$ & $35.1$\\
00390342+1330170 & M5.1 & & $10.94$ & $10.37$ & $10.06$ & & $9.84$ & $9.65$ & & $109.8 \pm 6.8$ & $-96.5 \pm 7.0$ & BPMG & $57.9$ & $15.3$\\
00464841+0715177 & M8.2 & & $13.89$ & $13.18$ & $12.55$ & & $12.09$ & $11.64$ & & $97.0 \pm 9.2$ & $-60.3 \pm 7.3$ & BPMG\tablenotemark{a} & $78.5$ & $28.4$\\
00581143-5653326 & L6.1 & & $16.78$ & $15.55$ & $14.55$ & & $13.76$ & $13.24$ & & $197.4 \pm 6.2$ & $46.0 \pm 12.2$ & ARG  & $80.4$ & $32.9$\\
01033203+1935361 & L6.2 & & $16.29$ & $14.90$ & $14.15$ & & $13.18$ & $12.70$ & & $303.0 \pm 13.4$ & $16.6 \pm 7.2$ & ARG  & $31.7$ & $16.9$\\
01525534-6329301 & M4.7 & & $10.17$ & $9.60$ & $9.26$ & & $9.06$ & $8.84$ & & $130.0 \pm 3.5$ & $7.0 \pm 6.4$ & BPMG  & $71.4$ & $22.1$\\
02534448-7959133 & M5.4 & & $11.34$ & $10.74$ & $10.38$ & & $10.18$ & $9.97$ & & $81.7 \pm 2.2$ & $90.3 \pm 9.3$ & BPMG  & $71.8$ & $24.9$\\
03390160-2434059 & M3.7 & & $10.90$ & $10.34$ & $9.97$ & & $9.72$ & $9.52$ & & $56.3 \pm 5.7$ & $-12.7 \pm 6.0$ & COL & $60.5$ & $32.9$\\
03473987-4114014 & M5.3 & & $13.13$ & $12.52$ & $12.23$ & & $12.04$ & $11.81$ & & $39.1 \pm 4.5$ & $1.7 \pm 6.5$ & COL  & $38.0$ & $45.4$\\
03510460-5701469 & M5.1 & & $12.83$ & $12.27$ & $11.94$ & & $11.76$ & $11.58$ & & $43.3 \pm 3.3$ & $14.3 \pm 7.3$ & COL & $17.6$ & $47.4$\\
03550477-1032415\tablenotemark{b} & M4.6 & & $13.08$ & $12.46$ & $11.98$ & & $11.71$ & $11.43$ & & $46.4 \pm 7.2$ & $-26.5 \pm 6.5$ & BPMG & $35.1$ & $40.7$\\
03582255-4116060 & L6.0 & & $15.85$ & $14.61$ & $13.84$ & & $12.91$ & $12.47$ & & $66.6 \pm 5.7$ & $102.3 \pm 8.3$ & BPMG & $44.7$ & $19.8$\\
04050182-3409330 & M5.6 & & $13.31$ & $12.74$ & $12.42$ & & $12.21$ & $11.97$ & & $40.7 \pm 5.0$ & $0.0 \pm 6.2$ & COL & $60.2$ & $29.4$\\
04075737-6310253 & M5.3 & & $12.49$ & $11.92$ & $11.59$ & & $11.43$ & $11.22$ & & $44.3 \pm 1.9$ & $16.2 \pm 6.7$ & THA & $14.2$ & $36.5$\\
04135144-4010093 & L2.5 & & $16.69$ & $15.56$ & $14.80$ & & $14.39$ & $14.03$ & & $45.9 \pm 7.3$ & $3.5 \pm 12.6$ & COL  & $82.5$ & $20.1$\\
04190316-1904217 & M5.6 & & $13.31$ & $12.70$ & $12.35$ & & $12.08$ & $11.91$ & & $28.6 \pm 6.5$ & $-23.9 \pm 7.0$ & COL & $13.2$ & $43.7$\\
04353042-6449570 & M8.4 & & $15.27$ & $14.51$ & $13.93$ & & $13.58$ & $13.21$ & & $39.2 \pm 1.9$ & $36.0 \pm 6.2$ & CAR  & $29.9$ & $25.5$\\
04503398-5216075\tablenotemark{b} & M2.9 & & $11.42$ & $10.84$ & $10.52$ & & $10.36$ & $10.15$ & & $43.6 \pm 4.7$ & $13.5 \pm 8.7$ & THA\tablenotemark{a} & $43.7$ & $22.4$\\
05012406-0010452 & L3.9 & & $14.98$ & $13.71$ & $12.96$ & & $12.05$ & $11.52$ & & $187.1 \pm 7.5$ & $-159.0 \pm 8.4$ & COL & $16.6$ & $21.6$\\
05020502-5706426 & M5.2 & & $13.06$ & $12.51$ & $12.20$ & & $12.00$ & $11.77$ & & $23.8 \pm 3.0$ & $23.0 \pm 6.7$ & COL & $16.8$ & $43.9$\\
05074031-1151582 & M5.3 & & $12.73$ & $12.12$ & $11.78$ & & $11.56$ & $11.31$ & & $41.2 \pm 6.2$ & $-17.8 \pm 6.2$ & COL & $47.5$ & $19.8$\\
05120636-2949540 & L6.2 & & $15.46$ & $14.16$ & $13.28$ & & $12.39$ & $11.92$ & & $-5.0 \pm 5.1$ & $84.5 \pm 6.6$ & BPMG & $42.8$ & $40.9$\\
05134660-1345346 & M5.2 & & $12.60$ & $12.01$ & $11.70$ & & $11.51$ & $11.31$ & & $30.8 \pm 6.0$ & $-19.7 \pm 7.7$ & COL & $72.9$ & $19.8$\\
05135141-4703059 & M6.7 & & $13.85$ & $13.27$ & $12.85$ & & $12.62$ & $12.37$ & & $37.9 \pm 3.8$ & $8.3 \pm 6.7$ & COL & $22.2$ & $25.3$\\
05350641-1706329 & M3.7 & & $10.18$ & $9.57$ & $9.30$ & & $9.11$ & $8.90$ & & $27.3 \pm 5.7$ & $-27.7 \pm 6.1$ & COL\tablenotemark{a} & $90.8$ & $15.7$\\
05504794-3020065 & M9.4 & & $15.39$ & $14.53$ & $14.03$ & & $13.68$ & $13.27$ & & $32.1 \pm 5.6$ & $12.0 \pm 7.6$ & COL & $40.7$ & $22.9$\\
05553750-4133488 & L0.4 & & $15.56$ & $14.66$ & $14.06$ & & $13.58$ & $13.21$ & & $29.4 \pm 4.7$ & $9.8 \pm 8.2$ & COL & $64.8$ & $17.9$\\
06100088-4727412\tablenotemark{b} & M8.4 & & $14.39$ & $13.77$ & $13.20$ & & $12.92$ & $12.67$ & & $20.6 \pm 6.0$ & $40.2 \pm 9.5$ & COL & $42.4$ & $21.8$\\
08095903+4434216 & L6.2 & & $16.44$ & $15.18$ & $14.42$ & & $13.36$ & $12.82$ & & $-178.3 \pm 7.0$ & $-204.9 \pm 10.9$ & ARG  & $35.8$ & $35.0$\\
09455843-3253299\tablenotemark{b} & M4.2 & & $9.20$ & $8.60$ & $8.28$ & & $8.09$ & $7.91$ & & $-295.3 \pm 6.2$ & $133.0 \pm 7.9$ & ARG & $71.5$ & $16.8$\\
10582800-1046304\tablenotemark{b} & M2.7 & & $9.51$ & $8.97$ & $8.64$ & & $8.46$ & $8.28$ & & $-185.1 \pm 8.3$ & $-73.7 \pm 7.7$ & TWA\tablenotemark{a} & $10.7$ & $37.8$\\
10584787-1548172 & L2.3 & & $14.15$ & $13.23$ & $12.53$ & & $12.08$ & $11.78$ & & $-260.9 \pm 7.8$ & $30.9 \pm 5.8$ & ARG  & $34.8$ & $36.8$\\
13262009-2729370 & L6.2 & & $15.85$ & $14.74$ & $13.85$ & & $12.87$ & $12.35$ & & $-366.5 \pm 17.0$ & $-19.2 \pm 6.5$ & ARG  & $38.2$ & $25.4$\\
17571539+7042011 & M7.2 & & $11.45$ & $10.84$ & $10.40$ & & $10.15$ & $9.89$ & & $12.0 \pm 1.3$ & $312.6 \pm 10.1$ & ARG  & $13.6$ & $31.1$\\
19112321-5105175 & M7.0 & & $12.83$ & $12.24$ & $11.78$ & & $11.58$ & $11.33$ & & $9.1 \pm 3.6$ & $-130.6 \pm 8.1$ & BPMG & $13.4$ & $30.9$\\
19541276-5711271 & M5.4 & & $11.81$ & $11.22$ & $10.93$ & & $10.70$ & $10.47$ & & $76.0 \pm 3.0$ & $-90.7 \pm 6.7$ & BPMG  & $24.1$ & $31.5$\\
20111744-2917584 & M5.3 & & $10.94$ & $10.31$ & $10.02$ & & $9.81$ & $9.63$ & & $102.9 \pm 5.2$ & $-81.9 \pm 6.0$ & ARG  & $67.9$ & $36.0$\\
20391000-5136094 & M4.1 & & $11.11$ & $10.54$ & $10.22$ & & $10.02$ & $9.83$ & & $47.3 \pm 3.2$ & $-131.6 \pm 7.1$ & ABDMG\tablenotemark{a} & $20.4$ & $24.0$\\
20405616-8245093 & M3.6 & & $9.52$ & $8.94$ & $8.64$ & & $8.45$ & $8.26$ & & $89.9 \pm 2.4$ & $-124.3 \pm 8.6$ & ARG\tablenotemark{a} & $93.9$ & $15.7$\\
20414283-3506442\tablenotemark{b} & M9.0 & & $14.89$ & $13.99$ & $13.40$ & & $12.86$ & $12.57$ & & $42.3 \pm 7.5$ & $-128.5 \pm 9.4$ & ABDMG & $15.3$ & $33.9$\\
21420580-3101162 & L1.1 & & $15.84$ & $14.77$ & $13.97$ & & $13.44$ & $13.16$ & & $57.8 \pm 5.5$ & $-114.0 \pm 7.7$ & ABDMG\tablenotemark{a} & $13.3$ & $39.1$\\
21471744-0444406 & M4.7 & & $9.42$ & $8.84$ & $8.50$ & & $8.30$ & $8.13$ & & $247.7 \pm 8.2$ & $-2.6 \pm 6.9$ & ARG & $71.2$ & $17.5$\\
21543454-1055308\tablenotemark{b} & L7.8 & & $16.44$ & $15.07$ & $14.20$ & & $13.37$ & $12.92$ & & $175.4 \pm 11.5$ & $8.8 \pm 11.6$ & ARG & $38.1$ & $34.8$\\
22030693-2538256 & M3.5 & & $10.58$ & $10.03$ & $9.69$ & & $9.49$ & $9.30$ & & $70.6 \pm 6.1$ & $-112.0 \pm 7.4$ & ABDMG\tablenotemark{a} & $14.6$ & $32.3$\\
22500814-5640571 & L2.9 & & $15.62$ & $14.55$ & $13.92$ & & $13.36$ & $13.01$ & & $183.2 \pm 5.1$ & $-55.4 \pm 7.1$ & ARG  & $53.7$ & $36.2$\\
23225384+7847386 & M5.2 & & $10.42$ & $9.84$ & $9.52$ & & $9.32$ & $9.10$ & & $213.6 \pm 6.1$ & $62.1 \pm 9.3$ & ARG & $22.7$ & $23.7$\\
23255604-0259508 & L2.3 & & $15.96$ & $14.94$ & $14.11$ & & $13.71$ & $13.41$ & & $85.5 \pm 9.6$ & $-108.2 \pm 7.0$ & ABDMG  & $32.1$ & $18.9$\\
23270843+3858234 & M5.2 & & $11.74$ & $11.10$ & $10.76$ & & $10.53$ & $10.31$ & & $96.6 \pm 4.8$ & $-88.9 \pm 6.7$ & ABDMG\tablenotemark{a} & $25.1$ & $25.5$\\
23290437+0329113 & M4.8 & & $11.11$ & $10.55$ & $10.19$ & & $10.00$ & $9.79$ & & $92.7 \pm 8.2$ & $-67.8 \pm 7.1$ & BPMG  & $29.4$ & $38.6$\\
23353085-1908389 & M4.8 & & $11.51$ & $10.97$ & $10.62$ & & $10.43$ & $10.22$ & & $97.7 \pm 5.7$ & $-106.5 \pm 6.9$ & ABDMG  & $35.7$ & $15.7$\\
23355015-3401477 & M5.4 & & $11.64$ & $11.06$ & $10.76$ & & $10.51$ & $10.27$ & & $112.9 \pm 5.8$ & $-52.7 \pm 7.2$ & BPMG  & $34.4$ & $40.4$\\
\enddata
\tablenotetext{a}{The binary hypothesis is more probable than the single hypothesis (see \hyperref[sec:filters]{Section~\ref*{sec:filters}}).}
\tablenotetext{b}{Object from the \href{http://irsa.ipac.caltech.edu/Missions/wise.html}{\emph{WISE}} catalog rather than \href{http://wise2.ipac.caltech.edu/docs/release/allwise/}{\emph{AllWISE}}.}
\end{deluxetable*}
\twocolumngrid

==> bass_table_5_long.tex <==
\onecolumngrid
\LongTables
\begin{deluxetable*}{lllcccccc}
\tablecolumns{9}
\tablecaption{The Complete \href{http://www.astro.umontreal.ca/\textasciitilde gagne/BASS.php}{\emph{BASS}} Catalog.\label{tab:allbass}}
\tablehead{\colhead{\href{http://www.ipac.caltech.edu/2mass/}{\emph{2MASS}}} & \colhead{Spectral} & \colhead{Probable} & \colhead{Bayesian} & \colhead{Contamination} & \colhead{Estimated Mass} & \colhead{Statistical} & \colhead{Statistical}\\
\colhead{Designation} & \colhead{Type\tablenotemark{a}} & \colhead{Membership} & \colhead{Prob. (\%)} & \colhead{Prob. (\%)} & \colhead{Range (\Mjup)} & \colhead{Distance (pc)} & \colhead{RV (\kms)}}
\startdata
\cutinhead{Candidates with a High Probability}
00011217+1535355 & L4: & ABDMG & $77.8$ & $1.8$ & $17.5^{+0.8}_{-1.1}$ & $27.3 \pm 1.6$ & $-6.5 \pm 2.0$\\
00040288-6410358 & L1$\gamma$ & THA & $> 99.9$ & $< 0.1$ & $12.8 \pm 0.3$ & $45.0 \pm 2.4$ & $6.5 \pm 2.5$\\
00041589-8747254 & (M5.7) & THA & $55.4$ & $< 0.1$ & $60.9^{+8.8}_{-7.1}$ & $51.8 \pm 3.6$ & $11.3 \pm 2.2$\\
00065794-6436542 & M9: & THA & $> 99.9$ & $< 0.1$ & $20.5^{+1.1}_{-13.9}$ & $41.4 \pm 2.4$ & $6.2 \pm 2.4$\\
00111532-3756553 & (M5.7) & THA & $80.2$ & $< 0.1$ & $60.6^{+8.6}_{-6.7}$ & $38.2^{+2.0}_{-2.4}$ & $1.5 \pm 2.2$\\
00182834-6703130 & (M9.6) & THA & $99.8$ & $< 0.1$ & $13.3 \pm 0.3$ & $43.8^{+2.8}_{-2.4}$ & $6.9 \pm 2.5$\\
00191296-6226005 & (M9.7) & THA & $99.5$ & $< 0.1$ & $13.3^{+0.3}_{-0.4}$ & $46.6^{+2.4}_{-2.8}$ & $6.7 \pm 2.5$\\
00192626+4614078 & M8 & ABDMG & $92.1$ & $4.1$ & $87.1^{+8.5}_{-8.6}$ & $37.8 \pm 3.2$ & $-19.5 \pm 3.0$\\
00212774-6351081 & M5.5 & THA & $99.8$ & $< 0.1$ & $158.3^{+19.9}_{-18.5}$ & $44.2^{+2.8}_{-2.4}$ & $6.8 \pm 2.4$\\
00235732-5531435 & M4.1 & THA & $99.8$ & $< 0.1$ & $133.1^{+17.4}_{-14.6}$ & $41.4 \pm 2.4$ & $5.3 \pm 0.7$\\
00305785-6550058 & (M3.3) & THA & $99.1$ & $< 0.1$ & $392.6^{+49.2}_{-44.1}$ & $47.0^{+2.8}_{-3.2}$ & $7.4 \pm 2.5$\\
00325584-4405058 & L0$\gamma$ & BPMG & $97.7$ & $0.2$ & $12.2 \pm 0.3$ & $26.4 \pm 3.3$ & $11.2 \pm 1.7$\\
00344300-4102266 & (L2.4) & THA & $96.1$ & $< 0.1$ & $12.8 \pm 0.3$ & $42.2 \pm 2.4$ & $2.6 \pm 2.2$\\
00354313+0233137 & M5+M6 & ABDMG & $88.4$ & $1.5$ & $191.9^{+13.9}_{-11.8}$ & $26.9 \pm 1.6$ & $1.3 \pm 2.0$\\
00374306-5846229 & L0$\gamma$ & THA & $99.9$ & $< 0.1$ & $13.9^{+0.4}_{-0.3}$ & $46.6 \pm 2.8$ & $6.8 \pm 2.4$\\
00390342+1330170 & (M5.1) & BPMG & $91.9$ & $11.3$ & $88.2^{+5.7}_{-5.4}$ & $29.7^{+2.4}_{-2.8}$ & $0.1 \pm 1.7$\\
00413538-5621127 & M6.5+M9 & THA & $> 99.9$ & $< 0.1$ & $78.6^{+10.2}_{-9.6}$ & $39.8^{+2.0}_{-2.4}$ & $2.8 \pm 1.9$\\
00452143+1634446 & L2$\beta$ & ARG & $98.0$ & $0.1$ & $14.7^{+0.3}_{-0.1}$ & $17.5 \pm 0.6$ & $3.3 \pm 0.2$\\
00514081-5913320 & M4.4 & THA & $99.9$ & $< 0.1$ & $128.9^{+16.9}_{-14.5}$ & $43.4^{+2.4}_{-2.8}$ & $6.3 \pm 1.3$\\
00525451-6624501 & (L0.3) & ABDMG & $11.8$ & $< 0.1$ & $31.0^{+2.0}_{-2.4}$ & $55.0 \pm 4.8$ & $23.8 \pm 1.8$\\
01033203+1935361 & L6$\beta$ & ARG & $78.2$ & $0.2$ & $10.4 \pm 0.4$ & $21.3 \pm 3.4$ & $8.6 \pm 2.2$\\
01033563-5515561 & M5.5 & THA & $99.9$ & $< 0.1$ & $320.6^{+40.2}_{-37.4}$ & $47.2 \pm 3.1$ & $5.2 \pm 1.6$\\
01075572-6030194 & (M5.3) & THA & $99.6$ & $< 0.1$ & $85.7^{+11.1}_{-8.9}$ & $42.2 \pm 2.4$ & $8.2 \pm 2.4$\\
01134031-5939346 & M5.0 & THA & $99.7$ & $< 0.1$ & $207.8^{+2.6}_{-1.3}$ & $43.0 \pm 3.2$ & $11.9 \pm 6.7$\\
01174748-3403258 & L1$\beta$ & THA & $99.6$ & $< 0.1$ & $13.5 \pm 0.3$ & $39.0 \pm 2.0$ & $4.7 \pm 2.1$\\
01180670-6258591 & M5.1 & THA & $> 99.9$ & $< 0.1$ & $105.1^{+13.7}_{-11.7}$ & $42.2^{+2.4}_{-2.8}$ & $9.3 \pm 1.3$\\
01205114-5200349 & (L2.5) & THA & $99.9$ & $< 0.1$ & $12.8 \pm 0.3$ & $41.0 \pm 2.4$ & $7.6 \pm 2.2$\\
01231125-6921379 & M8 & THA & $> 99.9$ & $< 0.1$ & $65.2^{+9.6}_{-8.6}$ & $42.2 \pm 4.8$ & $10.9 \pm 3.0$\\
01243060-3355014 & M4.5 & ABDMG & $> 99.9$ & $0.1$ & $167.6^{+14.6}_{-13.4}$ & $25.3 \pm 0.8$ & $18.3 \pm 0.5$\\
01265327-5505506 & (M5.3) & THA & $99.8$ & $< 0.1$ & $77.2^{+10.5}_{-8.8}$ & $42.6^{+2.4}_{-2.8}$ & $8.2 \pm 2.4$\\
01294256-0823580 & M5 & BPMG & $66.2$ & $< 0.1$ & $122.9^{+8.4}_{-8.8}$ & $32.5 \pm 3.2$ & $9.2 \pm 1.7$\\
01320814-6023536 & (M4.5) & THA & $99.8$ & $< 0.1$ & $126.0^{+16.3}_{-14.1}$ & $45.4 \pm 2.8$ & $9.2 \pm 2.4$\\
01344601-5707564 & M4.9 & THA & $99.8$ & $< 0.1$ & $76.2^{+10.5}_{-8.8}$ & $43.4^{+2.8}_{-3.2}$ & $11.1 \pm 6.3$\\
01372781-4558261 & M5.0 & THA & $97.8$ & $< 0.1$ & $126.5^{+16.6}_{-14.9}$ & $39.4^{+2.0}_{-2.4}$ & $13.5 \pm 1.4$\\
01393605-6455456 & (M5.4) & THA & $88.9$ & $< 0.1$ & $65.5^{+9.5}_{-7.4}$ & $48.6^{+3.2}_{-2.8}$ & $10.6 \pm 2.4$\\
01415823-4633574 & L0$\gamma$ & THA & $99.5$ & $< 0.1$ & $14.5^{+0.4}_{-0.7}$ & $41.0 \pm 2.8$ & $12.0 \pm 15.0$\\
01443191-4604318 & M5.5 & THA & $99.1$ & $< 0.1$ & $80.9^{+10.7}_{-9.1}$ & $41.0 \pm 2.4$ & $8.1 \pm 2.2$\\
01484859-5201158 & (M4.0) & THA & $99.8$ & $< 0.1$ & $158.8^{+20.2}_{-18.0}$ & $41.8 \pm 2.4$ & $8.6 \pm 2.2$\\
01504543-5716488 & M5.5 & THA & $> 99.9$ & $< 0.1$ & $71.2^{+10.3}_{-8.1}$ & $43.0^{+2.4}_{-2.8}$ & $9.3 \pm 1.7$\\
01531463-6744181 & L2: & THA & $99.9$ & $< 0.1$ & $12.2 \pm 0.4$ & $46.6 \pm 2.8$ & $10.2 \pm 2.4$\\
01532494-6833226 & M5.1 & THA & $> 99.9$ & $< 0.1$ & $159.0^{+20.3}_{-18.0}$ & $45.4 \pm 2.8$ & $9.8 \pm 1.4$\\
02004709-5105206 & (L5.9) & ABDMG & $99.1$ & $0.7$ & $12.5^{+0.1}_{-0.4}$ & $22.5 \pm 1.6$ & $23.8 \pm 1.8$\\
02013900-5948345 & (M5.3) & THA & $33.1$ & $< 0.1$ & $71.2^{+10.2}_{-8.1}$ & $36.2 \pm 2.4$ & $9.6 \pm 2.2$\\
02025502-7259155 & (M3.5) & THA & $99.6$ & $< 0.1$ & $193.7^{+13.4}_{-11.0}$ & $46.6^{+3.2}_{-2.8}$ & $11.2 \pm 2.1$\\
02103857-3015313 & (M9.3) & THA & $99.7$ & $< 0.1$ & $13.8^{+0.4}_{-0.3}$ & $41.4^{+2.0}_{-2.4}$ & $7.6 \pm 2.1$\\
02153328-5627175 & M5.4 & THA & $99.8$ & $< 0.1$ & $93.1^{+12.0}_{-10.9}$ & $45.0 \pm 3.2$ & $11.3 \pm 5.7$\\
02180960-6657524 & M4.5 & THA & $> 99.9$ & $< 0.1$ & $180.2^{+21.6}_{-18.7}$ & $45.0 \pm 2.8$ & $11.0 \pm 1.2$\\
02192210-3925225 & M4.9 & THA & $> 99.9$ & $< 0.1$ & $112.0^{+13.1}_{-14.8}$ & $40.6 \pm 2.4$ & $10.6 \pm 0.7$\\
02212859-6831400 & M8: & ABDMG & $40.8$ & $< 0.1$ & $44.0^{+4.9}_{-4.7}$ & $39.4 \pm 5.6$ & $25.5 \pm 2.0$\\
02214262-5947087 & (M5.3) & THA & $99.6$ & $< 0.1$ & $87.5^{+11.3}_{-9.5}$ & $44.2 \pm 2.8$ & $10.9 \pm 2.2$\\
02215494-5412054 & M8$\beta$ & THA & $99.8$ & $< 0.1$ & $20.0^{+3.8}_{-4.7}$ & $38.2^{+2.4}_{-2.0}$ & $10.2 \pm 2.2$\\
02235464-5815067 & L0$\gamma$ & THA & $> 99.9$ & $< 0.1$ & $13.8^{+0.3}_{-0.4}$ & $39.4^{+2.0}_{-2.4}$ & $10.6 \pm 2.2$\\
02251947-5837295 & M9 & THA & $99.9$ & $< 0.1$ & $25.5^{+5.4}_{-4.0}$ & $41.4 \pm 2.4$ & $10.7 \pm 2.2$\\
02265658-5327032 & (M9.5) & THA & $99.9$ & $< 0.1$ & $13.5 \pm 0.3$ & $43.4 \pm 2.4$ & $10.3 \pm 2.2$\\
02294869-6906044 & M4.6 & THA & $> 99.9$ & $< 0.1$ & $90.6^{+11.7}_{-9.9}$ & $46.2 \pm 3.2$ & $13.0 \pm 1.2$\\
02321934-5746117 & M4.4 & THA & $> 99.9$ & $< 0.1$ & $156.6^{+20.1}_{-17.3}$ & $45.8 \pm 2.8$ & $11.2 \pm 0.7$\\
02330550-7023148 & (M5.3) & THA & $15.0$ & $< 0.1$ & $75.9^{+10.5}_{-8.5}$ & $54.2 \pm 3.6$ & $12.6 \pm 2.2$\\
02340093-6442068 & L0$\gamma$ & THA & $99.8$ & $< 0.1$ & $13.5 \pm 0.3$ & $43.8^{+2.4}_{-2.8}$ & $10.6 \pm 2.2$\\
02401209-5305527 & M9.5 & THA & $99.9$ & $< 0.1$ & $20.2^{+4.7}_{-2.9}$ & $43.8 \pm 2.4$ & $10.9 \pm 2.2$\\
02405344-1724188 & (M5.4) & THA & $96.7$ & $< 0.1$ & $66.9^{+9.6}_{-7.2}$ & $47.0 \pm 2.8$ & $7.8 \pm 2.0$\\
02410564-5511466 & (M9.7) & THA & $99.9$ & $< 0.1$ & $13.5 \pm 0.3$ & $41.8 \pm 2.4$ & $11.2 \pm 2.2$\\
02411151-0326587 & L0$\gamma$ & THA & $98.3$ & $< 0.1$ & $13.1^{+0.4}_{-0.3}$ & $46.7 \pm 5.7$ & $5.7 \pm 2.7$\\
02422401-6533400 & (M5.7) & THA & $20.3$ & $< 0.1$ & $61.1^{+8.8}_{-7.1}$ & $50.6 \pm 3.6$ & $11.7 \pm 2.5$\\
02435103-5432194 & M9 & THA & $99.9$ & $< 0.1$ & $20.3^{+3.6}_{-5.3}$ & $41.8 \pm 2.4$ & $11.2 \pm 2.2$\\
02441019-3548036 & (M9.4) & THA & $87.1$ & $< 0.1$ & $14.0 \pm 0.3$ & $49.0 \pm 2.8$ & $9.7 \pm 2.1$\\
02483062-5259398 & (M4.2) & THA & $99.8$ & $< 0.1$ & $138.1^{+18.4}_{-16.6}$ & $44.2 \pm 2.8$ & $11.3 \pm 2.2$\\
02494277-6812126 & (M5.3) & THA & $99.6$ & $< 0.1$ & $67.7^{+9.8}_{-7.7}$ & $47.4 \pm 3.2$ & $12.1 \pm 2.1$\\
02501167-0151295 & (M7.0) & BPMG & $88.3$ & $1.2$ & $26.3^{+3.5}_{-4.3}$ & $33.1 \pm 4.9$ & $13.1 \pm 2.0$\\
02523550-7831183 & M4.4 & THA & $98.6$ & $< 0.1$ & $119.3^{+15.3}_{-13.7}$ & $49.4^{+3.6}_{-4.0}$ & $12.8 \pm 1.3$\\
02543476-5108288 & (M5.3) & THA & $99.7$ & $< 0.1$ & $81.9^{+10.9}_{-9.1}$ & $45.4^{+3.2}_{-2.8}$ & $11.7 \pm 2.2$\\
02553178-5702522 & (M3.8) & THA & $98.4$ & $< 0.1$ & $167.5^{+21.3}_{-18.7}$ & $47.8 \pm 3.2$ & $12.1 \pm 2.4$\\
02583123-1520536 & (L2.4) & THA & $73.6$ & $< 0.1$ & $12.8 \pm 0.3$ & $45.0 \pm 2.8$ & $10.5 \pm 2.0$\\
03014892-5903021 & M9 & THA & $99.9$ & $< 0.1$ & $31.9^{+10.0}_{-9.8}$ & $47.4^{+2.8}_{-3.2}$ & $12.3 \pm 2.2$\\
03032042-7312300 & L2$\gamma$ & THA & $78.2$ & $< 0.1$ & $12.9 \pm 0.3$ & $52.2^{+3.6}_{-3.2}$ & $11.9 \pm 2.4$\\
03050556-5317182 & M5.4 & THA & $99.9$ & $< 0.1$ & $150.8^{+19.5}_{-17.1}$ & $45.4 \pm 3.2$ & $12.1 \pm 2.2$\\
03093877-3014352 & M4.7 & THA & $99.9$ & $< 0.1$ & $112.4^{+14.4}_{-13.0}$ & $45.4 \pm 3.2$ & $12.5 \pm 2.3$\\
03114544-4719501 & M4.3 & THA & $> 99.9$ & $< 0.1$ & $199.4^{+9.6}_{-7.0}$ & $44.6 \pm 2.8$ & $11.3 \pm 0.5$\\
03152363-5342539 & M5.2 & THA & $99.9$ & $< 0.1$ & $141.8^{+18.7}_{-16.2}$ & $46.2^{+2.8}_{-3.2}$ & $12.7 \pm 2.2$\\
03164512-2848521 & L0 & ABDMG & $77.2$ & $4.9$ & $28.8^{+2.2}_{-2.4}$ & $31.7 \pm 2.4$ & $24.3 \pm 2.0$\\
03204919-3313400 & (M5.7) & THA & $99.7$ & $< 0.1$ & $59.6^{+8.5}_{-6.7}$ & $44.6 \pm 2.8$ & $12.3 \pm 2.1$\\
03224622-7940595 & (M5.2) & THA & $58.9$ & $< 0.1$ & $88.3^{+11.4}_{-9.6}$ & $51.4 \pm 3.6$ & $10.2 \pm 2.1$\\
03231002-4631237 & L0$\gamma$ & THA & $99.7$ & $< 0.1$ & $14.0^{+0.3}_{-0.4}$ & $48.6 \pm 3.2$ & $12.6 \pm 2.2$\\
03252938-4312299 & M9 & THA & $78.9$ & $< 0.1$ & $23.9^{+7.1}_{-5.2}$ & $49.8 \pm 3.2$ & $13.0 \pm 2.2$\\
03264225-2102057 & L4 & ABDMG & $98.9$ & $1.3$ & $13.8^{+0.6}_{-0.7}$ & $26.1^{+1.6}_{-2.0}$ & $23.1 \pm 2.0$\\
03283347-6236225 & (M5.1) & THA & $99.7$ & $< 0.1$ & $93.5^{+12.1}_{-10.3}$ & $46.2 \pm 3.2$ & $13.0 \pm 2.1$\\
03363144-2619578 & M5.7 & THA & $99.9$ & $< 0.1$ & $186.3^{+19.0}_{-15.7}$ & $43.5 \pm 3.8$ & $12.7 \pm 2.1$\\
03420931-2904317 & (L2.3) & THA & $99.2$ & $< 0.1$ & $12.8 \pm 0.3$ & $48.6^{+3.6}_{-3.2}$ & $12.7 \pm 2.1$\\
03421621-6817321 & L2: & THA & $99.7$ & $< 0.1$ & $11.8^{+0.6}_{-0.4}$ & $49.0^{+3.2}_{-3.6}$ & $13.0 \pm 2.1$\\
03441258-3716463 & (M5.8) & THA & $99.5$ & $< 0.1$ & $46.9^{+7.4}_{-6.0}$ & $47.0 \pm 3.2$ & $13.7 \pm 2.1$\\
03445673-1145126 & (M6.0) & BPMG & $75.2$ & $< 0.1$ & $46.4^{+4.0}_{-4.2}$ & $31.3^{+4.0}_{-4.4}$ & $16.9 \pm 2.0$\\
03552337+1133437 & L5$\gamma$ & ABDMG & $99.7$ & $1.1$ & $13.2 \pm 0.1$ & $9.1 \pm 0.1$ & $11.9 \pm 0.2$\\
03572695-4417305 & M9$\beta$+L1.5$\beta$ & THA & $99.9$ & $< 0.1$ & $17.1^{+1.1}_{-1.8}$ & $47.4 \pm 2.8$ & $14.2 \pm 2.0$\\
04094585-3923319 & (M6.4) & THA & $97.5$ & $< 0.1$ & $36.2^{+9.2}_{-6.4}$ & $49.4 \pm 3.6$ & $14.5 \pm 2.1$\\
04174743-2129191 & M8 & THA & $57.7$ & $< 0.1$ & $30.3^{+7.5}_{-5.2}$ & $49.0 \pm 3.6$ & $13.3 \pm 2.2$\\
04182880-0533019 & (L3.8) & COL & $29.0$ & $7.4$ & $9.6^{+0.6}_{-1.5}$ & $34.6^{+3.2}_{-2.8}$ & $18.4 \pm 2.0$\\
04185879-4507413 & (L2.5) & THA & $87.2$ & $< 0.1$ & $12.8^{+0.4}_{-0.3}$ & $50.6^{+3.6}_{-4.0}$ & $15.1 \pm 2.1$\\
04210718-6306022 & L5$\gamma$ & ARG & $97.7$ & $13.5$ & $10.3^{+0.7}_{-0.3}$ & $16.1^{+1.6}_{-1.2}$ & $9.7 \pm 2.2$\\
04273598-2316586 & (M3.7) & COL & $95.0$ & $10.1$ & $199.8^{+11.4}_{-7.0}$ & $46.2^{+5.2}_{-5.6}$ & $21.3 \pm 1.7$\\
04341693-2526468 & (M3.9) & COL & $90.5$ & $13.7$ & $178.5^{+22.0}_{-19.2}$ & $57.0^{+7.2}_{-6.4}$ & $21.5 \pm 1.7$\\
04362788-4114465 & M8$\gamma$ & COL & $97.6$ & $9.7$ & $41.1^{+9.2}_{-6.7}$ & $43.8 \pm 4.8$ & $22.0 \pm 1.4$\\
04380868-4342484 & (M5.0) & COL & $87.8$ & $14.6$ & $95.2^{+13.8}_{-14.6}$ & $56.6^{+9.2}_{-8.0}$ & $21.8 \pm 1.5$\\
04400972-5126544 & (M9.4) & THA & $80.5$ & $< 0.1$ & $13.6 \pm 0.3$ & $52.6 \pm 3.6$ & $15.6 \pm 2.1$\\
04433761+0002051 & M9$\gamma$ & BPMG & $99.8$ & $3.3$ & $18.2^{+2.4}_{-2.5}$ & $20.5^{+2.8}_{-3.2}$ & $17.1 \pm 3.0$\\
04532647-1751543 & L3: & COL & $95.8$ & $8.5$ & $17.7^{+2.4}_{-4.3}$ & $54.2 \pm 4.4$ & $21.5 \pm 1.7$\\
04533604-2835349 & (M4.0) & COL & $87.6$ & $7.4$ & $202.6^{+10.2}_{-5.0}$ & $52.6^{+11.2}_{-12.0}$ & $22.5 \pm 6.7$\\
05002100+0330501 & L4 & ABDMG & $62.8$ & $0.6$ & $23.9^{+7.7}_{-1.7}$ & $14.9 \pm 0.8$ & $15.9 \pm 0.2$\\
05012406-0010452 & L3$\gamma$ & CAR & $97.7$ & $< 0.1$ & $10.0^{+1.0}_{-0.8}$ & $14.7 \pm 2.8$ & $18.9 \pm 1.4$\\
05071673-2352431 & (M5.1) & COL & $94.8$ & $11.2$ & $91.1^{+12.7}_{-12.8}$ & $51.4^{+7.6}_{-6.4}$ & $22.7 \pm 1.5$\\
05120921-1807415 & (M5.4) & COL & $88.1$ & $14.2$ & $68.0^{+10.2}_{-9.3}$ & $53.8^{+7.2}_{-6.0}$ & $22.4 \pm 1.7$\\
05123569-3041067 & (M4.6) & COL & $95.0$ & $11.5$ & $114.8^{+16.2}_{-17.0}$ & $52.6^{+8.0}_{-7.2}$ & $22.9 \pm 1.5$\\
05130001-1611177 & (M4.3) & COL & $88.8$ & $12.5$ & $137.2^{+18.8}_{-18.1}$ & $53.0^{+6.4}_{-5.6}$ & $22.2 \pm 1.7$\\
05181131-3101529 & M6.5 & COL & $93.7$ & $8.0$ & $95.6^{+13.4}_{-13.7}$ & $44.6^{+5.6}_{-6.4}$ & $23.2 \pm 1.4$\\
05264316-1824315 & (M5.3) & COL & $91.4$ & $14.1$ & $77.5 \pm 11.3$ & $49.8^{+7.2}_{-6.4}$ & $22.7 \pm 1.5$\\
05284789-2909077 & (M4.5) & COL & $94.0$ & $12.1$ & $121.9^{+17.7}_{-19.1}$ & $52.2^{+9.2}_{-7.6}$ & $23.4 \pm 1.4$\\
05313142-4323042 & (M4.0) & COL & $86.3$ & $11.4$ & $178.1^{+23.6}_{-20.1}$ & $43.0^{+8.0}_{-6.8}$ & $23.2 \pm 1.4$\\
05361998-1920396 & L2$\gamma$ & COL & $96.6$ & $0.7$ & $12.6^{+1.0}_{-0.8}$ & $39.0 \pm 14.0$ & $22.8 \pm 1.8$\\
05400823-3642181 & (L2.3) & COL & $82.9$ & $12.3$ & $12.5^{+0.7}_{-0.4}$ & $48.6^{+10.0}_{-7.6}$ & $23.6 \pm 1.4$\\
05432117-2204024 & (M5.6) & COL & $70.2$ & $13.8$ & $62.8^{+9.3}_{-8.5}$ & $35.4^{+4.4}_{-4.0}$ & $23.6 \pm 1.4$\\
05461532-5547521 & (M5.2) & CAR & $93.7$ & $5.2$ & $91.1^{+11.8}_{-10.5}$ & $35.8^{+3.2}_{-2.8}$ & $22.1 \pm 1.0$\\
05490552-4832344 & (M4.4) & COL & $78.7$ & $12.4$ & $129.4^{+19.1}_{-20.5}$ & $43.8^{+7.6}_{-6.8}$ & $23.1 \pm 1.3$\\
05504281-5308392 & (M3.6) & CAR & $81.6$ & $9.9$ & $202.8^{+8.4}_{-4.9}$ & $42.6^{+4.4}_{-3.6}$ & $22.4 \pm 1.0$\\
06022216+6336391 & L1: & ABDMG & $26.1$ & $14.1$ & $28.4^{+1.8}_{-2.1}$ & $26.9 \pm 1.6$ & $-12.0 \pm 1.5$\\
06272161-5308428 & (L4.0) & CAR & $65.9$ & $9.6$ & $10.3^{+1.1}_{-0.8}$ & $32.5 \pm 4.4$ & $23.4 \pm 1.1$\\
06420559+4101599 & L/Tp & ABDMG & $38.4$ & $4.5$ & $11.4 \pm 0.1$ & $16.9 \pm 0.8$ & $0.6 \pm 1.7$\\
06513251-6528322 & (M7.6) & CAR & $84.4$ & $5.0$ & $25.2^{+6.6}_{-3.9}$ & $66.2^{+6.4}_{-5.6}$ & $20.6 \pm 1.0$\\
06524851-5741376 & M8$\beta$ & CAR & $87.9$ & $< 0.1$ & $20.3^{+4.9}_{-3.1}$ & $32.0 \pm 3.3$ & $21.5 \pm 0.8$\\
06561550-5728017 & (M5.9) & CAR & $48.2$ & $9.0$ & $50.3^{+7.8}_{-7.1}$ & $50.6^{+6.0}_{-5.6}$ & $22.4 \pm 1.1$\\
07013784-6411369 & (M5.4) & CAR & $10.4$ & $8.2$ & $72.3^{+10.6}_{-10.0}$ & $55.8^{+6.8}_{-6.0}$ & $20.4 \pm 1.0$\\
07105337-7431070 & (M9.7) & CAR & $67.4$ & $4.0$ & $13.6^{+0.4}_{-0.3}$ & $34.2 \pm 3.6$ & $19.3 \pm 1.0$\\
07485518-6721360 & (M3.8) & CAR & $99.4$ & $1.4$ & $185.5^{+19.9}_{-16.3}$ & $48.2^{+5.6}_{-4.8}$ & $20.4 \pm 1.0$\\
08025781-8330076 & (M5.4) & BPMG & $94.5$ & $8.6$ & $63.8 \pm 5.0$ & $20.5^{+2.4}_{-2.0}$ & $11.9 \pm 2.2$\\
08035086-7344331 & (M3.7) & CAR & $95.4$ & $2.4$ & $196.8^{+13.5}_{-9.1}$ & $74.2^{+9.2}_{-7.6}$ & $19.0 \pm 1.1$\\
08063045-6809212 & (M3.8) & CAR & $82.8$ & $4.6$ & $181.8^{+21.5}_{-18.0}$ & $75.4^{+9.2}_{-8.4}$ & $19.8 \pm 1.1$\\
08144321+2336045 & (M5.3) & TWA & $11.9$ & $7.9$ & $36.9^{+7.7}_{-6.0}$ & $27.7 \pm 2.4$ & $11.7 \pm 1.3$\\
08173829-6817162 & (M3.8) & CAR & $35.0$ & $3.1$ & $206.8^{+4.0}_{-2.0}$ & $53.0^{+6.4}_{-5.2}$ & $20.0 \pm 1.0$\\
09532126-1014205 & L0 & CAR & $63.7$ & $8.3$ & $18.9^{+1.3}_{-1.7}$ & $37.8 \pm 2.0$ & $17.6 \pm 1.0$\\
10212570-2830427 & (L4.0) & TWA & $88.6$ & $1.4$ & $7.5^{+0.6}_{-0.3}$ & $42.6 \pm 5.6$ & $13.7 \pm 1.7$\\
10284580-2830374 & M5 & TWA & $96.3$ & $1.1$ & $105.7^{+11.1}_{-13.1}$ & $45.4 \pm 5.2$ & $14.0 \pm 1.4$\\
10513331-1916530 & (M9.1) & TWA & $42.4$ & $5.5$ & $12.1^{+0.8}_{-0.4}$ & $44.2 \pm 3.6$ & $11.7 \pm 1.4$\\
10554602-8216412 & (M5.3) & CAR & $10.8$ & $11.7$ & $72.3^{+10.3}_{-8.8}$ & $76.6 \pm 5.2$ & $17.2 \pm 1.5$\\
10571669-3512548 & (M5.8) & TWA & $35.7$ & $10.2$ & $20.9^{+1.0}_{-1.5}$ & $61.0 \pm 6.8$ & $13.4 \pm 1.5$\\
10584787-1548172 & L3 & ARG & $93.1$ & $0.3$ & $12.4 \pm 0.1$ & $17.3 \pm 0.3$ & $6.8 \pm 1.1$\\
10585054-2346206 & (M3.8) & TWA & $50.4$ & $4.4$ & $133.8^{+15.7}_{-15.3}$ & $42.2 \pm 4.8$ & $11.4 \pm 1.4$\\
11020983-3430355 & M8.5$\gamma$ & TWA & $99.8$ & $0.1$ & $26.2^{+1.7}_{-8.5}$ & $56.4 \pm 1.6$ & $12.7 \pm 1.5$\\
11035165-3711483 & (M5.3) & TWA & $84.8$ & $0.9$ & $31.6^{+5.4}_{-8.5}$ & $50.6^{+6.4}_{-6.0}$ & $12.7 \pm 1.4$\\
11035873-4156475 & (M5.8) & TWA & $34.4$ & $13.3$ & $21.6^{+1.1}_{-1.7}$ & $68.6^{+8.4}_{-7.6}$ & $13.1 \pm 1.5$\\
11064461-3715115 & (M7.5) & TWA & $92.9$ & $1.8$ & $15.3 \pm 0.6$ & $62.6^{+6.8}_{-6.4}$ & $13.0 \pm 1.5$\\
11112820-2655027 & (M3.8) & TWA & $97.8$ & $1.5$ & $136.1^{+15.5}_{-15.2}$ & $43.4 \pm 4.8$ & $11.7 \pm 1.4$\\
11112984-2713320 & (M4.9) & TWA & $93.3$ & $1.7$ & $48.9^{+10.9}_{-9.8}$ & $47.0 \pm 5.6$ & $12.3 \pm 1.4$\\
11153797-2552192 & (M5.3) & TWA & $13.2$ & $6.7$ & $33.1^{+6.1}_{-7.7}$ & $49.8^{+5.6}_{-5.2}$ & $11.2 \pm 1.5$\\
11385038-3830011 & (M5.4) & TWA & $17.7$ & $2.9$ & $28.1^{+3.6}_{-9.6}$ & $63.4^{+8.0}_{-7.2}$ & $11.9 \pm 1.5$\\
11393382-3040002 & M4.7 & TWA & $99.0$ & $1.3$ & $196.8^{+13.7}_{-8.9}$ & $48.2^{+5.2}_{-5.6}$ & $10.7 \pm 1.5$\\
11394506-3729069 & (M5.2) & TWA & $83.4$ & $3.1$ & $36.6^{+7.5}_{-6.6}$ & $67.8^{+8.0}_{-7.6}$ & $11.9 \pm 1.5$\\
11395113-3159214 & M8$\gamma$ & TWA & $99.8$ & $< 0.1$ & $16.1^{+0.6}_{-0.7}$ & $28.5 \pm 3.5$ & $11.2 \pm 2.0$\\
11480096-2836488 & (L1.9) & TWA & $45.6$ & $4.6$ & $9.0^{+0.7}_{-0.6}$ & $50.2^{+5.6}_{-5.2}$ & $10.2 \pm 1.8$\\
11510246-3611457 & (M5.3) & TWA & $62.1$ & $2.9$ & $34.9 \pm 7.0$ & $30.1^{+3.6}_{-3.2}$ & $10.2 \pm 1.5$\\
12035905-3821402 & (M5.9) & TWA & $99.3$ & $1.0$ & $20.0^{+0.8}_{-1.0}$ & $67.0^{+7.2}_{-6.8}$ & $10.5 \pm 1.7$\\
12073346-3932539 & M8 & TWA & $99.6$ & $< 0.1$ & $22.1^{+0.4}_{-1.3}$ & $52.3 \pm 1.1$ & $10.9 \pm 1.5$\\
12074836-3900043 & L1$\gamma$ & TWA & $99.7$ & $< 0.1$ & $12.0^{+0.7}_{-0.6}$ & $59.4 \pm 5.2$ & $9.9 \pm 1.7$\\
12134001-3723362 & (M5.1) & TWA & $86.0$ & $2.7$ & $38.9^{+7.9}_{-6.6}$ & $70.2^{+8.0}_{-7.6}$ & $10.6 \pm 1.7$\\
12174683-3804157 & (M5.2) & TWA & $20.5$ & $3.3$ & $35.5^{+7.1}_{-7.0}$ & $65.8 \pm 8.0$ & $10.3 \pm 1.7$\\
12175920-3734433 & (M3.8) & TWA & $98.6$ & $1.0$ & $102.3^{+11.4}_{-13.0}$ & $65.0^{+7.2}_{-6.8}$ & $9.9 \pm 1.7$\\
12214223-4012050 & (L2.5) & TWA & $79.1$ & $1.2$ & $8.2^{+0.6}_{-0.7}$ & $53.0^{+6.4}_{-8.4}$ & $9.2 \pm 2.1$\\
12310489-3801065 & (M7.4) & TWA & $73.8$ & $1.9$ & $14.9^{+0.6}_{-0.4}$ & $67.0^{+6.4}_{-7.6}$ & $9.9 \pm 2.0$\\
12474428-3816464 & M9$\gamma$ & TWA & $47.1$ & $< 0.1$ & $16.7 \pm 0.6$ & $75.0^{+6.4}_{-7.2}$ & $9.5 \pm 1.8$\\
12535039-4211215 & (M9.0) & TWA & $50.7$ & $5.4$ & $12.1^{+0.7}_{-0.6}$ & $81.0^{+7.6}_{-7.2}$ & $9.6 \pm 2.0$\\
12563961-2718455 & (L2.7) & TWA & $12.1$ & $14.6$ & $8.3 \pm 0.6$ & $49.0^{+5.2}_{-5.6}$ & $7.8 \pm 2.2$\\
12574941-4111373 & (M5.0) & TWA & $60.0$ & $4.5$ & $42.9^{+9.3}_{-7.4}$ & $77.8^{+8.8}_{-8.4}$ & $9.0 \pm 1.8$\\
13155594-3403418 & (M5.4) & TWA & $10.9$ & $10.2$ & $25.6^{+2.2}_{-5.4}$ & $65.0^{+6.8}_{-6.4}$ & $7.5 \pm 2.0$\\
14252798-3650229 & L5 & ABDMG & $99.6$ & $0.1$ & $18.2^{+0.3}_{-0.1}$ & $11.6 \pm 0.1$ & $5.4 \pm 0.3$\\
17571539+7042011 & M7.5 & ARG & $91.0$ & $0.2$ & $41.8^{+3.2}_{-5.0}$ & $19.1 \pm 0.4$ & $-12.4 \pm 0.6$\\
19010688-7115248 & (M5.3) & THA & $26.1$ & $< 0.1$ & $69.5^{+10.0}_{-7.9}$ & $57.0^{+4.4}_{-4.0}$ & $4.4 \pm 2.2$\\
19075853-8324093 & (M5.4) & THA & $11.0$ & $< 0.1$ & $67.1^{+9.8}_{-7.8}$ & $58.2 \pm 4.4$ & $7.9 \pm 2.1$\\
19350976-6200473 & (L1.7) & THA & $13.4$ & $0.1$ & $13.2 \pm 0.3$ & $60.6 \pm 4.4$ & $1.6 \pm 2.5$\\
19395435-5216468 & (L1.3) & BPMG & $57.9$ & $11.8$ & $12.6^{+0.3}_{-0.1}$ & $28.9^{+2.8}_{-2.4}$ & $-3.0 \pm 2.1$\\
19444417-4359015 & (M4.9) & BPMG & $86.4$ & $7.7$ & $100.0^{+5.3}_{-6.0}$ & $28.1 \pm 2.4$ & $-2.9 \pm 2.0$\\
19514573-6641061 & (M5.2) & THA & $59.9$ & $< 0.1$ & $86.8^{+11.3}_{-9.6}$ & $55.4 \pm 4.0$ & $2.9 \pm 2.4$\\
19564700-7542270 & L0$\gamma$ & THA & $85.2$ & $< 0.1$ & $13.3 \pm 0.3$ & $57.0 \pm 4.0$ & $6.5 \pm 2.4$\\
20004841-7523070 & M9 & BPMG & $98.2$ & $3.1$ & $33.7^{+2.8}_{-2.6}$ & $31.3^{+2.4}_{-2.8}$ & $11.8 \pm 1.0$\\
20092431-6330508 & (M4.3) & THA & $79.9$ & $< 0.1$ & $138.1^{+18.3}_{-15.6}$ & $49.0 \pm 3.2$ & $2.0 \pm 2.1$\\
20113196-5048112 & (L2.5) & THA & $28.1$ & $< 0.1$ & $12.6^{+0.4}_{-0.3}$ & $53.0 \pm 3.6$ & $-1.9 \pm 2.2$\\
20224803-5645567 & M5.5 & THA & $59.2$ & $< 0.1$ & $122.5^{+15.9}_{-14.6}$ & $52.2^{+3.2}_{-3.6}$ & $-1.1 \pm 2.2$\\
20282203-5637024 & (M6.6) & THA & $30.0$ & $< 0.1$ & $34.4^{+9.3}_{-6.7}$ & $55.8 \pm 3.6$ & $0.4 \pm 2.2$\\
20291446-5456116 & M4.3 & THA & $71.4$ & $< 0.1$ & $145.6^{+19.1}_{-16.3}$ & $46.2 \pm 3.2$ & $-1.4 \pm 1.2$\\
20330186-4903105 & (M5.6) & BPMG & $99.1$ & $0.1$ & $67.3^{+12.7}_{-15.6}$ & $16.3 \pm 5.0$ & $-0.5 \pm 3.5$\\
20334473-5635338 & (M9.6) & THA & $49.8$ & $< 0.1$ & $13.5^{+0.4}_{-0.3}$ & $55.4 \pm 3.6$ & $0.2 \pm 2.7$\\
20423672-5425263 & M4.0 & THA & $94.8$ & $< 0.1$ & $196.5^{+11.8}_{-9.1}$ & $49.8^{+3.2}_{-3.6}$ & $-1.4 \pm 1.7$\\
20430452-5547114 & (M5.3) & THA & $68.6$ & $< 0.1$ & $83.2^{+11.0}_{-8.9}$ & $51.0 \pm 3.2$ & $-1.3 \pm 2.2$\\
20452795-7717561 & (M5.7) & THA & $80.0$ & $< 0.1$ & $56.3^{+7.9}_{-6.8}$ & $55.8^{+4.0}_{-3.6}$ & $7.5 \pm 2.2$\\
20484222-5127435 & (M9.4) & THA & $25.6$ & $< 0.1$ & $13.9 \pm 0.3$ & $49.0 \pm 2.8$ & $-0.6 \pm 2.2$\\
21083826-4244540 & M4.4 & THA & $84.4$ & $< 0.1$ & $207.9^{+2.4}_{-1.1}$ & $45.8^{+2.8}_{-3.2}$ & $-4.9 \pm 1.9$\\
21102873-5540391 & (M9.2) & THA & $60.8$ & $< 0.1$ & $14.2 \pm 0.3$ & $54.2 \pm 3.2$ & $-0.2 \pm 2.2$\\
21121598-8128452 & (M3.6) & THA & $40.4$ & $< 0.1$ & $191.3^{+15.3}_{-12.5}$ & $45.0 \pm 3.2$ & $8.9 \pm 2.2$\\
21143529-6124082 & (M5.7) & THA & $85.4$ & $< 0.1$ & $59.6^{+8.6}_{-7.1}$ & $52.6 \pm 3.2$ & $1.2 \pm 2.2$\\
21192028-8145446 & (M4.1) & THA & $35.7$ & $< 0.1$ & $145.3^{+19.0}_{-16.6}$ & $43.8^{+3.2}_{-2.8}$ & $8.6 \pm 2.1$\\
21265040-8140293 & L3$\gamma$ & THA & $85.1$ & $< 0.1$ & $13.3 \pm 0.3$ & $43.4 \pm 2.8$ & $8.1 \pm 2.2$\\
21490499-6413039 & M4.5 & THA & $99.7$ & $< 0.1$ & $205.5^{+5.3}_{-2.9}$ & $46.6^{+3.2}_{-3.6}$ & $0.4 \pm 5.1$\\
21503682-7023414 & (M5.1) & THA & $39.9$ & $< 0.1$ & $94.7^{+12.4}_{-10.6}$ & $53.8 \pm 3.6$ & $3.9 \pm 2.2$\\
21544859-7459134 & (M8.0) & THA & $98.2$ & $< 0.1$ & $20.3^{+3.8}_{-5.3}$ & $47.0^{+3.2}_{-2.8}$ & $6.8 \pm 2.2$\\
22025794-5605087 & (M8.0) & THA & $95.5$ & $< 0.1$ & $22.1^{+4.7}_{-3.9}$ & $48.6 \pm 2.8$ & $1.3 \pm 2.4$\\
22060961-0723353 & M5.5 & ABDMG & $82.1$ & $1.4$ & $142.4^{+13.0}_{-11.6}$ & $23.3 \pm 1.2$ & $-7.8 \pm 2.0$\\
22064498-4217208 & L2 & ABDMG & $95.2$ & $1.6$ & $18.8 \pm 0.8$ & $27.7 \pm 1.6$ & $7.6 \pm 1.8$\\
22244102-7724036 & M4.2 & THA & $99.2$ & $< 0.1$ & $145.1^{+19.0}_{-16.4}$ & $49.8^{+3.2}_{-3.6}$ & $8.5 \pm 1.4$\\
22283837-3648372 & (M5.3) & ABDMG & $28.9$ & $13.7$ & $154.2^{+14.1}_{-12.8}$ & $41.4^{+2.8}_{-2.4}$ & $6.5 \pm 2.0$\\
22320782-8308108 & (M9.4) & THA & $41.3$ & $< 0.1$ & $13.6 \pm 0.3$ & $55.8 \pm 3.2$ & $11.0 \pm 2.2$\\
22351658-3844154 & (M9.3) & THA & $90.8$ & $< 0.1$ & $13.6 \pm 0.3$ & $42.2 \pm 2.4$ & $-3.0 \pm 2.2$\\
22353560-5906306 & (M8.1) & THA & $99.1$ & $< 0.1$ & $20.6^{+4.3}_{-3.3}$ & $44.2^{+2.8}_{-2.4}$ & $2.9 \pm 2.4$\\
22400144+0532162 & (M6.3) & BPMG & $79.0$ & $0.1$ & $38.4^{+3.5}_{-3.3}$ & $23.6 \pm 2.7$ & $-6.5 \pm 2.1$\\
22443167+2043433 & L6$\gamma$ & ABDMG & $99.8$ & $0.6$ & $11.5^{+0.1}_{-1.0}$ & $16.1 \pm 0.8$ & $-15.8 \pm 1.5$\\
22444835-6650032 & M4.8 & THA & $99.7$ & $< 0.1$ & $175.3^{+21.9}_{-19.7}$ & $47.4^{+3.2}_{-2.8}$ & $0.7 \pm 1.7$\\
22511530-6811216 & (M5.3) & THA & $99.6$ & $< 0.1$ & $83.7^{+11.0}_{-9.2}$ & $47.4^{+2.8}_{-3.2}$ & $5.4 \pm 2.4$\\
22583200+1014589 & (M5.1) & ABDMG & $98.3$ & $0.1$ & $167.6^{+15.1}_{-13.9}$ & $23.1 \pm 1.4$ & $-11.2 \pm 2.1$\\
23051517-3550073 & (M4.9) & THA & $16.3$ & $< 0.1$ & $101.6^{+13.2}_{-11.7}$ & $45.4 \pm 2.8$ & $-3.3 \pm 2.1$\\
23130558-6127077 & M4.5 & THA & $99.8$ & $< 0.1$ & $178.5^{+21.7}_{-19.1}$ & $46.6^{+3.2}_{-2.8}$ & $2.9 \pm 2.3$\\
23155665-4747315 & (L2.3) & THA & $20.5$ & $< 0.1$ & $12.6^{+0.4}_{-0.1}$ & $47.8^{+3.2}_{-2.8}$ & $0.6 \pm 2.4$\\
23221690-6833004 & (M3.7) & THA & $99.2$ & $< 0.1$ & $184.2^{+19.4}_{-17.1}$ & $48.2^{+3.2}_{-2.8}$ & $6.9 \pm 2.5$\\
23225240-6151114 & M5 & THA & $98.7$ & $< 0.1$ & $104.4^{+13.7}_{-11.1}$ & $42.2 \pm 2.4$ & $5.0 \pm 2.4$\\
23225299-6151275 & L2$\gamma$ & THA & $> 99.9$ & $< 0.1$ & $13.1 \pm 0.3$ & $43.0^{+2.0}_{-2.4}$ & $5.0 \pm 2.4$\\
23225384+7847386 & M5 & CAR & $29.7$ & $1.0$ & $71.3^{+14.5}_{-17.4}$ & $19.1 \pm 5.5$ & $-17.0 \pm 1.3$\\
23233072-2807141 & (M4.9) & ABDMG & $47.4$ & $9.9$ & $187.0^{+15.7}_{-13.8}$ & $40.2 \pm 2.4$ & $7.2 \pm 2.0$\\
23321028-6926537 & (M5.3) & THA & $99.4$ & $< 0.1$ & $79.1^{+10.7}_{-8.5}$ & $43.4^{+2.8}_{-2.4}$ & $7.1 \pm 2.4$\\
23360735-3541489 & (M8.9) & THA & $39.2$ & $< 0.1$ & $14.6^{+0.3}_{-0.4}$ & $43.0 \pm 2.4$ & $-0.5 \pm 2.4$\\
23392527+3507165 & L3.5 & BPMG & $10.6$ & $10.7$ & $11.0^{+0.4}_{-0.3}$ & $25.3 \pm 2.0$ & $-4.6 \pm 1.8$\\
23424333-6224564 & M4.3 & THA & $99.6$ & $< 0.1$ & $127.6^{+16.7}_{-14.6}$ & $43.8^{+3.2}_{-2.8}$ & $5.1 \pm 4.6$\\
23433470-3646021 & (L5.1) & BPMG & $42.6$ & $5.6$ & $10.0^{+0.3}_{-0.4}$ & $26.5^{+2.0}_{-2.4}$ & $7.5 \pm 1.5$\\
23520507-1100435 & M7 & ABDMG & $42.0$ & $7.9$ & $80.1^{+7.2}_{-7.4}$ & $39.4^{+2.0}_{-2.4}$ & $2.9 \pm 2.0$\\
23523223-3413068 & (M5.3) & ABDMG & $79.9$ & $2.7$ & $141.0^{+13.1}_{-11.8}$ & $31.3 \pm 2.0$ & $11.7 \pm 2.0$\\
\cutinhead{Candidates with a Modest Probability}
00160844-0043021 & L5.5 & BPMG & $19.1$ & $36.1$ & $9.6 \pm 0.3$ & $30.9^{+2.8}_{-3.2}$ & $3.3 \pm 1.8$\\
00274534-0806046 & (M5.3) & BPMG & $45.6$ & $35.1$ & $66.9 \pm 4.2$ & $32.1 \pm 2.8$ & $4.4 \pm 1.5$\\
00464841+0715177 & M9 & BPMG & $77.0$ & $26.9$ & $15.0^{+0.1}_{-0.3}$ & $33.8^{+2.8}_{-3.2}$ & $3.2 \pm 1.7$\\
00581143-5653326 & (L6.1) & ARG & $80.4$ & $32.9$ & $10.3^{+0.7}_{-0.3}$ & $25.3^{+2.8}_{-2.4}$ & $2.6 \pm 2.0$\\
01525534-6329301 & (M4.7) & BPMG & $71.4$ & $22.1$ & $107.6^{+6.8}_{-7.8}$ & $23.7 \pm 2.4$ & $14.7 \pm 1.7$\\
02534448-7959133 & M5.5 & BPMG & $50.1$ & $30.9$ & $66.9 \pm 4.9$ & $28.9^{+2.8}_{-3.2}$ & $12.0 \pm 2.1$\\
03390160-2434059 & M5.9 & COL & $77.8$ & $31.9$ & $204.7^{+6.6}_{-3.5}$ & $59.4^{+5.6}_{-6.0}$ & $18.6 \pm 1.8$\\
03473987-4114014 & (M5.3) & COL & $38.0$ & $45.4$ & $77.2^{+11.0}_{-10.5}$ & $71.0^{+8.8}_{-8.0}$ & $19.7 \pm 1.7$\\
03510460-5701469 & (M5.1) & COL & $17.6$ & $47.4$ & $88.3^{+12.0}_{-11.7}$ & $68.6^{+8.8}_{-8.0}$ & $19.1 \pm 1.7$\\
03550477-1032415 & M8.5 & BPMG & $39.5$ & $38.5$ & $26.4^{+3.5}_{-4.2}$ & $35.0^{+4.4}_{-4.8}$ & $17.7 \pm 1.8$\\
03582255-4116060 & L5 & BPMG & $36.8$ & $21.9$ & $9.3 \pm 0.1$ & $18.9^{+2.8}_{-2.4}$ & $17.6 \pm 1.7$\\
04050182-3409330 & (M5.6) & COL & $60.2$ & $29.4$ & $62.3^{+9.1}_{-8.1}$ & $67.0^{+7.6}_{-7.2}$ & $20.6 \pm 1.8$\\
04075737-6310253 & (M5.3) & THA & $14.2$ & $36.5$ & $79.1^{+10.7}_{-8.9}$ & $54.2 \pm 4.0$ & $14.9 \pm 2.0$\\
04135144-4010093 & (L2.5) & COL & $82.5$ & $20.1$ & $12.4^{+0.7}_{-0.4}$ & $57.8^{+8.4}_{-7.6}$ & $21.1 \pm 2.0$\\
04190316-1904217 & (M5.6) & COL & $13.2$ & $43.7$ & $61.4^{+9.1}_{-7.9}$ & $64.6^{+7.6}_{-6.4}$ & $20.0 \pm 2.0$\\
04353042-6449570 & (M8.4) & CAR & $29.9$ & $25.5$ & $19.8^{+4.7}_{-2.6}$ & $63.0 \pm 4.4$ & $19.7 \pm 1.0$\\
04503398-5216075 & (M4.0) & THA & $43.7$ & $22.4$ & $157.6^{+20.3}_{-18.3}$ & $53.0^{+4.0}_{-4.4}$ & $15.8 \pm 2.1$\\
05020502-5706426 & (M5.2) & COL & $16.8$ & $43.9$ & $82.6^{+11.7}_{-11.6}$ & $73.0^{+10.4}_{-9.2}$ & $20.8 \pm 1.5$\\
05074031-1151582 & (M5.3) & COL & $47.5$ & $19.8$ & $76.9^{+10.7}_{-10.0}$ & $57.8^{+6.4}_{-5.6}$ & $21.4 \pm 1.8$\\
05120636-2949540 & L4: & BPMG & $33.8$ & $43.0$ & $9.2 \pm 0.1$ & $13.3^{+2.0}_{-2.4}$ & $19.8 \pm 1.5$\\
05134660-1345346 & (M5.2) & COL & $72.9$ & $19.8$ & $85.5^{+11.6}_{-11.1}$ & $59.8^{+7.6}_{-6.4}$ & $21.8 \pm 1.8$\\
05135141-4703059 & (M6.7) & COL & $22.2$ & $25.3$ & $37.0^{+9.2}_{-7.0}$ & $59.8^{+9.2}_{-8.4}$ & $22.5 \pm 1.4$\\
05350641-1706329 & (M3.7) & COL & $90.8$ & $15.7$ & $206.1^{+5.2}_{-2.5}$ & $49.4^{+6.8}_{-5.6}$ & $22.8 \pm 1.5$\\
05504794-3020065 & (M9.4) & COL & $40.7$ & $22.9$ & $14.2 \pm 0.4$ & $55.4^{+7.6}_{-8.0}$ & $23.9 \pm 1.5$\\
05553750-4133488 & (L0.4) & COL & $64.8$ & $17.9$ & $13.9 \pm 0.4$ & $53.0^{+7.2}_{-7.6}$ & $23.5 \pm 1.4$\\
06100088-4727412 & (M8.4) & COL & $42.4$ & $21.8$ & $20.5^{+4.2}_{-4.3}$ & $48.2^{+5.2}_{-6.8}$ & $23.5 \pm 1.4$\\
08095903+4434216 & L6 & ARG & $30.7$ & $35.4$ & $6.5^{+0.1}_{-0.3}$ & $16.1 \pm 1.6$ & $15.1 \pm 1.5$\\
09455843-3253299 & M4.5 & ARG & $89.2$ & $15.6$ & $113.7^{+11.7}_{-12.0}$ & $13.7^{+1.6}_{-1.2}$ & $11.4 \pm 1.3$\\
10582800-1046304 & M4 & TWA & $4.3$ & $46.8$ & $99.6^{+10.7}_{-12.5}$ & $24.9 \pm 2.4$ & $10.0 \pm 1.3$\\
13262009-2729370 & L5 & ARG & $23.3$ & $27.3$ & $6.5^{+0.1}_{-0.3}$ & $12.9^{+0.8}_{-1.2}$ & $-7.6 \pm 1.5$\\
19112321-5105175 & (M7.0) & BPMG & $13.4$ & $30.9$ & $29.4^{+2.8}_{-2.9}$ & $33.8^{+3.2}_{-2.8}$ & $-0.1 \pm 2.2$\\
19541276-5711271 & (M5.4) & BPMG & $24.1$ & $31.5$ & $63.8 \pm 4.0$ & $35.4^{+3.2}_{-2.8}$ & $-2.5 \pm 2.1$\\
20111744-2917584 & M5.5 & ARG & $49.3$ & $41.0$ & $95.6^{+10.9}_{-11.4}$ & $26.9^{+3.2}_{-3.6}$ & $-18.6 \pm 1.7$\\
20334670-3733443 & M5 & BPMG & $80.0$ & $16.6$ & $113.6^{+6.6}_{-7.0}$ & $33.8 \pm 2.8$ & $-4.6 \pm 1.8$\\
20391000-5136094 & (M4.1) & ABDMG & $20.4$ & $24.0$ & $207.3^{+3.2}_{-1.5}$ & $44.2 \pm 2.8$ & $7.6 \pm 1.8$\\
20405616-8245093 & (M3.6) & ARG & $93.9$ & $15.7$ & $207.2^{+3.5}_{-1.7}$ & $32.5^{+3.6}_{-3.2}$ & $-1.8 \pm 2.0$\\
20414283-3506442 & L2: & ABDMG & $14.4$ & $26.0$ & $33.8^{+2.0}_{-2.2}$ & $45.0 \pm 2.8$ & $-0.4 \pm 2.2$\\
21420580-3101162 & L3 & ABDMG & $12.6$ & $41.4$ & $26.6^{+1.1}_{-1.8}$ & $49.4 \pm 3.2$ & $1.1 \pm 2.1$\\
21471744-0444406 & (M4.7) & ARG & $71.2$ & $17.5$ & $128.9^{+14.4}_{-14.9}$ & $16.5 \pm 2.0$ & $-14.1 \pm 1.3$\\
21543454-1055308 & L4$\beta$ & ARG & $58.6$ & $34.2$ & $10.3^{+0.7}_{-0.3}$ & $22.5 \pm 2.4$ & $-13.1 \pm 1.5$\\
22030693-2538256 & (M3.5) & ABDMG & $14.6$ & $32.3$ & $403.8^{+25.7}_{-20.7}$ & $47.8^{+3.2}_{-2.8}$ & $0.1 \pm 2.1$\\
22500814-5640571 & (L2.9) & ARG & $53.7$ & $36.2$ & $12.0 \pm 0.3$ & $28.5^{+2.8}_{-2.4}$ & $-3.9 \pm 1.5$\\
23255604-0259508 & L3 & ABDMG & $29.8$ & $19.4$ & $24.5^{+2.2}_{-2.6}$ & $45.4^{+3.2}_{-2.8}$ & $-2.7 \pm 2.2$\\
23270843+3858234 & (M5.2) & ABDMG & $25.1$ & $25.5$ & $159.7^{+15.1}_{-14.5}$ & $40.2 \pm 3.2$ & $-17.2 \pm 1.5$\\
23290437+0329113 & (M4.8) & BPMG & $29.4$ & $38.6$ & $106.2^{+6.3}_{-7.2}$ & $36.2^{+3.6}_{-3.2}$ & $-2.6 \pm 1.7$\\
23353085-1908389 & (M4.8) & ABDMG & $35.7$ & $15.7$ & $191.9^{+14.2}_{-11.8}$ & $43.8 \pm 2.8$ & $4.6 \pm 2.0$\\
23355015-3401477 & (M5.4) & BPMG & $34.4$ & $40.4$ & $63.5 \pm 4.3$ & $32.5^{+3.2}_{-2.8}$ & $4.8 \pm 1.5$\\
\enddata
\tablenotetext{a}{Spectral types in parentheses were estimated from \href{http://www.ipac.caltech.edu/2mass/}{\emph{2MASS}}--\href{http://wise2.ipac.caltech.edu/docs/release/allwise/}{\emph{AllWISE}} colors (see \hyperref[sec:filters]{Section~\ref*{sec:spt}}).}
\tablenotetext{b}{The binary hypothesis is more probable than the single hypothesis (see \hyperref[sec:filters]{Section~\ref*{sec:filters}}).}
\end{deluxetable*}
\twocolumngrid

==> bass_table_B2_long.tex <==
\onecolumngrid
\LongTables
\begin{deluxetable*}{lllcccccc}
\tablecolumns{9}
\tablecaption{The Complete \href{http://www.astro.umontreal.ca/\textasciitilde gagne/LP-BASS.php}{\emph{LP-BASS}} Catalog.\label{tab:allbass_ann}}
\tablehead{\colhead{\href{http://www.ipac.caltech.edu/2mass/}{\emph{2MASS}}} & \colhead{Spectral} & \colhead{Probable} & \colhead{Bayesian} & \colhead{Contamination} & \colhead{Estimated Mass} & \colhead{Statistical} & \colhead{Statistical}\\
\colhead{Designation} & \colhead{Type\tablenotemark{a}} & \colhead{Membership} & \colhead{Prob. (\%)} & \colhead{Prob. (\%)} & \colhead{Range (\Mjup)} & \colhead{Distance (pc)} & \colhead{RV (\kms)}}
\startdata
\cutinhead{Candidates with a High Probability}
00081980-2559449 & (M5.8) & ABDMG & $60.1$ & $5.3$ & $87.1^{+8.2}_{-7.8}$ & $36.2^{+2.4}_{-2.0}$ & $10.0 \pm 2.0$\\
00091768+0603461 & (M5.2) & ABDMG & $36.6$ & $2.4$ & $156.3^{+14.4}_{-12.8}$ & $25.3 \pm 1.6$ & $-2.0 \pm 2.0$\\
00165057-7122387 & (M5.7) & THA & $36.6$ & $< 0.1$ & $57.7^{+8.1}_{-6.3}$ & $47.4 \pm 3.2$ & $-3.4 \pm 3.0$\\
00165242-7640540 & (M5.3) & THA & $31.8$ & $< 0.1$ & $85.0^{+11.1}_{-8.9}$ & $45.4^{+3.2}_{-2.8}$ & $6.4 \pm 2.4$\\
00200551-5359372 & (M6.2) & THA & $98.9$ & $< 0.1$ & $36.2^{+9.3}_{-6.7}$ & $39.8^{+2.4}_{-2.0}$ & $5.3 \pm 2.4$\\
00303013-1450333 & L7 & ARG & $24.1$ & $2.6$ & $10.4^{+0.6}_{-0.4}$ & $26.7 \pm 3.2$ & $4.3 \pm 2.0$\\
00381489-6403529 & (M8.6) & THA & $99.7$ & $< 0.1$ & $15.3^{+0.7}_{-6.1}$ & $44.2 \pm 2.4$ & $7.5 \pm 2.4$\\
00425349-6117384 & M4.2 & THA & $99.9$ & $< 0.1$ & $123.0^{+15.6}_{-13.1}$ & $42.6 \pm 2.4$ & $6.9 \pm 1.0$\\
00455663+3347109 & M4.5+M5.5 & ARG & $89.7$ & $0.1$ & $86.4^{+8.4}_{-7.7}$ & $18.1 \pm 1.3$ & $4.3 \pm 1.4$\\
00474453+4159428 & (M3.7) & BPMG & $49.0$ & $14.4$ & $169.0^{+10.5}_{-11.0}$ & $30.5 \pm 2.8$ & $-3.2 \pm 2.2$\\
00485254-6526330 & (M3.3) & THA & $84.9$ & $< 0.1$ & $207.2^{+3.3}_{-1.7}$ & $50.2 \pm 3.2$ & $8.5 \pm 2.5$\\
00514561-6227073 & (M5.7) & THA & $99.8$ & $< 0.1$ & $54.7^{+7.7}_{-6.1}$ & $43.4^{+2.8}_{-2.4}$ & $7.6 \pm 2.4$\\
00530909+0511387 & (M5.1) & ABDMG & $24.9$ & $4.8$ & $168.7^{+16.0}_{-15.7}$ & $32.1 \pm 2.8$ & $1.8 \pm 2.4$\\
00551459+4511019 & (M5.3) & ABDMG & $19.3$ & $3.3$ & $141.1^{+13.9}_{-13.5}$ & $35.8 \pm 3.3$ & $-14.4 \pm 2.2$\\
00575326-1028004 & (M5.3) & ABDMG & $15.6$ & $12.3$ & $122.3^{+12.4}_{-11.3}$ & $38.6 \pm 2.4$ & $8.5 \pm 2.0$\\
00583298-0547135 & (M5.7) & BPMG & $10.8$ & $< 0.1$ & $54.2^{+3.9}_{-4.6}$ & $36.6 \pm 4.0$ & $5.5 \pm 1.8$\\
00584253-0651239 & L0 & BPMG & $88.6$ & $0.3$ & $-1047.2 \pm NaN$ & $29.6 \pm 3.5$ & $6.7 \pm 2.0$\\
01000219-6156270 & M6 & THA & $99.1$ & $< 0.1$ & $48.3^{+7.4}_{-5.9}$ & $41.4 \pm 2.4$ & $7.8 \pm 2.4$\\
01075893-3255427 & (M5.2) & THA & $52.1$ & $< 0.1$ & $90.6^{+11.6}_{-9.2}$ & $41.8 \pm 2.4$ & $1.9 \pm 2.1$\\
01121205+0541262 & (M5.3) & ABDMG & $24.1$ & $4.7$ & $134.3^{+13.1}_{-12.1}$ & $30.9 \pm 2.4$ & $3.2 \pm 2.2$\\
01144953-7813430 & (M5.0) & THA & $52.2$ & $< 0.1$ & $96.3^{+12.7}_{-10.6}$ & $51.8^{+3.6}_{-3.2}$ & $12.4 \pm 2.1$\\
01190749-4943305 & (M5.7) & THA & $77.2$ & $< 0.1$ & $52.5^{+7.5}_{-5.7}$ & $37.4^{+2.4}_{-2.0}$ & $6.7 \pm 2.2$\\
01225371-4952175 & (M5.3) & THA & $82.8$ & $< 0.1$ & $75.5^{+10.3}_{-7.9}$ & $35.8 \pm 2.0$ & $7.4 \pm 2.2$\\
01253196-6646023 & M4.2 & THA & $99.7$ & $< 0.1$ & $172.1^{+21.9}_{-19.2}$ & $46.2 \pm 3.2$ & $7.1 \pm 5.1$\\
01275875-6032243 & M4.2 & THA & $> 99.9$ & $< 0.1$ & $147.8^{+19.2}_{-16.0}$ & $43.8 \pm 2.8$ & $9.1 \pm 2.5$\\
01283025-4921094 & M4.1 & THA & $99.3$ & $< 0.1$ & $189.5^{+16.6}_{-13.8}$ & $43.0 \pm 2.8$ & $6.5 \pm 5.7$\\
01321248-0910029 & (M6.3) & THA & $20.8$ & $< 0.1$ & $36.3^{+8.8}_{-6.0}$ & $45.8^{+3.2}_{-2.8}$ & $0.6 \pm 2.1$\\
01375150+0727458 & (M6.8) & ABDMG & $53.7$ & $8.1$ & $66.0^{+6.3}_{-5.9}$ & $39.0 \pm 2.8$ & $4.6 \pm 2.2$\\
01375879-5645447 & M3.9 & THA & $99.9$ & $< 0.1$ & $198.6^{+10.0}_{-7.7}$ & $43.4^{+2.4}_{-2.8}$ & $8.5 \pm 0.6$\\
01422579-6504120 & (M5.4) & THA & $99.7$ & $< 0.1$ & $68.1^{+9.8}_{-7.1}$ & $46.2 \pm 2.8$ & $10.2 \pm 2.2$\\
01534955+4427284 & (M5.3) & ARG & $98.5$ & $0.1$ & $86.8^{+8.2}_{-7.2}$ & $20.2 \pm 1.2$ & $7.4 \pm 1.8$\\
02001992-6614017 & M4.3 & THA & $> 99.9$ & $< 0.1$ & $182.4^{+21.2}_{-17.8}$ & $43.8 \pm 2.8$ & $11.8 \pm 1.1$\\
02015072-0726581 & (M3.9) & THA & $87.0$ & $< 0.1$ & $163.2^{+20.9}_{-18.1}$ & $43.8^{+3.2}_{-2.8}$ & $3.6 \pm 2.1$\\
02025788-3136262 & M4.0 & COL & $40.7$ & $< 0.1$ & $150.9^{+19.8}_{-18.1}$ & $57.0^{+4.8}_{-5.2}$ & $12.4 \pm 1.5$\\
02030658-5545420 & M4.5 & THA & $99.9$ & $< 0.1$ & $133.5^{+17.4}_{-14.5}$ & $45.0 \pm 2.8$ & $9.7 \pm 2.2$\\
02071861-2513254 & (M5.3) & THA & $90.1$ & $< 0.1$ & $80.5^{+10.7}_{-8.5}$ & $39.0 \pm 2.4$ & $7.8 \pm 2.0$\\
02091868-2717161 & (M5.1) & THA & $60.4$ & $< 0.1$ & $94.0^{+12.1}_{-9.9}$ & $36.6^{+2.4}_{-2.0}$ & $8.6 \pm 2.0$\\
02115630-0142153 & (M4.1) & ABDMG & $53.7$ & $13.2$ & $206.8^{+3.9}_{-2.0}$ & $42.2 \pm 3.2$ & $11.2 \pm 2.2$\\
02123372-6049185 & M6.5 & THA & $94.8$ & $< 0.1$ & $35.4^{+8.6}_{-6.1}$ & $43.4^{+2.8}_{-3.2}$ & $13.1 \pm 0.2$\\
02190228+2352550 & M3.6 & ARG & $72.2$ & $0.3$ & $134.5^{+13.0}_{-10.6}$ & $20.6 \pm 0.8$ & $15.7 \pm 0.7$\\
02210522-0750071 & (M5.7) & THA & $29.3$ & $< 0.1$ & $53.6^{+7.7}_{-6.1}$ & $48.6^{+3.6}_{-3.2}$ & $4.3 \pm 2.5$\\
02273458-1606328 & (M5.7) & ABDMG & $38.1$ & $9.3$ & $106.0^{+10.7}_{-10.3}$ & $35.4^{+2.8}_{-2.4}$ & $17.6 \pm 2.1$\\
02282694+0218331 & (M5.8) & BPMG & $67.2$ & $< 0.1$ & $50.1^{+3.3}_{-4.0}$ & $35.0^{+4.0}_{-3.6}$ & $12.0 \pm 2.0$\\
02284949-1121137 & (M5.7) & THA & $52.0$ & $< 0.1$ & $60.0^{+8.6}_{-6.8}$ & $48.6 \pm 3.2$ & $5.0 \pm 2.2$\\
02294569-5541496 & M4.8 & THA & $> 99.9$ & $< 0.1$ & $143.8^{+18.8}_{-16.3}$ & $43.4 \pm 2.8$ & $11.5 \pm 1.0$\\
02300966-1325202 & (M5.2) & THA & $86.0$ & $< 0.1$ & $92.1^{+12.0}_{-10.2}$ & $42.6^{+2.4}_{-2.8}$ & $5.5 \pm 2.1$\\
02333091-3846191 & (M6.1) & ABDMG & $60.3$ & $< 0.1$ & $76.6^{+7.2}_{-7.1}$ & $39.0 \pm 3.2$ & $24.1 \pm 2.0$\\
02341866-5128462 & M4.3 & THA & $> 99.9$ & $< 0.1$ & $186.6^{+18.7}_{-15.7}$ & $43.0^{+2.4}_{-2.8}$ & $10.9 \pm 0.9$\\
02351494+0247534 & (M5.3) & BPMG & $77.6$ & $0.1$ & $76.2^{+2.9}_{-3.3}$ & $17.8 \pm 1.0$ & $8.9 \pm 2.2$\\
02354496+3429215 & (M5.3) & BPMG & $33.6$ & $13.9$ & $68.7 \pm 4.5$ & $25.3 \pm 2.4$ & $6.0 \pm 2.2$\\
02383255-7528065 & M4.1 & THA & $98.9$ & $< 0.1$ & $121.6^{+15.6}_{-13.5}$ & $50.2 \pm 3.2$ & $12.3 \pm 0.6$\\
02391762-2649188 & (M3.3) & THA & $99.3$ & $< 0.1$ & $369.2^{+45.8}_{-41.9}$ & $41.0 \pm 2.4$ & $9.2 \pm 2.1$\\
02404759-4253377 & (M5.7) & THA & $99.4$ & $< 0.1$ & $60.7^{+8.6}_{-6.7}$ & $39.4 \pm 2.4$ & $10.6 \pm 2.1$\\
02412721-3049149 & M4.7 & BPMG & $88.3$ & $7.8$ & $68.3 \pm 5.2$ & $27.3^{+3.2}_{-2.8}$ & $18.2 \pm 1.1$\\
02420204-5359147 & M4.6 & THA & $> 99.9$ & $< 0.1$ & $165.5^{+21.2}_{-18.5}$ & $42.2 \pm 2.8$ & $11.5 \pm 2.3$\\
02444769-1148259 & (M4.8) & THA & $97.8$ & $< 0.1$ & $112.0^{+14.2}_{-12.7}$ & $45.4^{+3.2}_{-2.8}$ & $7.4 \pm 2.2$\\
02552243-2044490 & (M6.8) & BPMG & $85.0$ & $< 0.1$ & $30.9 \pm 3.5$ & $22.5^{+2.8}_{-2.4}$ & $16.3 \pm 1.7$\\
02591904-5122341 & M5.4 & THA & $> 99.9$ & $< 0.1$ & $103.7^{+13.5}_{-11.8}$ & $45.4^{+3.2}_{-2.8}$ & $11.0 \pm 2.3$\\
03022816-3257020 & (M4.0) & THA & $13.7$ & $< 0.1$ & $150.1^{+19.5}_{-16.6}$ & $48.2 \pm 3.2$ & $12.1 \pm 2.0$\\
03025156-1911496 & (M3.5) & THA & $99.3$ & $< 0.1$ & $194.4^{+13.0}_{-10.5}$ & $44.6 \pm 2.8$ & $10.0 \pm 2.0$\\
03060278-1243526 & (M5.6) & ABDMG & $13.5$ & $7.5$ & $115.9^{+11.8}_{-10.9}$ & $28.9 \pm 2.0$ & $19.4 \pm 2.0$\\
03104941-3616471 & M4.3 & THA & $> 99.9$ & $< 0.1$ & $188.7^{+17.3}_{-14.4}$ & $44.2 \pm 2.8$ & $13.8 \pm 1.6$\\
03114240-1537183 & (M5.7) & ABDMG & $26.7$ & $4.9$ & $94.7^{+9.3}_{-8.6}$ & $25.3 \pm 1.6$ & $20.7 \pm 2.1$\\
03114241-3239449 & (M9.8) & THA & $93.2$ & $< 0.1$ & $13.8 \pm 0.3$ & $46.6 \pm 2.8$ & $10.6 \pm 2.2$\\
03123239-0040081 & (M5.8) & BPMG & $30.1$ & $< 0.1$ & $52.1^{+3.9}_{-4.7}$ & $39.4^{+4.4}_{-4.8}$ & $14.1 \pm 2.0$\\
03132588-2447246 & (M7.6) & BPMG & $85.2$ & $< 0.1$ & $19.3^{+3.1}_{-2.4}$ & $22.9^{+2.4}_{-2.0}$ & $17.0 \pm 1.7$\\
03134187-2932470 & (M6.3) & BPMG & $62.1$ & $< 0.1$ & $35.4^{+4.0}_{-3.8}$ & $19.7 \pm 2.4$ & $17.6 \pm 1.8$\\
03171968-7722171 & (M5.1) & ABDMG & $70.2$ & $12.3$ & $161.2^{+16.2}_{-16.3}$ & $26.5 \pm 2.8$ & $25.6 \pm 1.4$\\
03181842-6433220 & (L2.0) & THA & $89.8$ & $< 0.1$ & $12.0^{+0.1}_{-0.3}$ & $46.6 \pm 3.2$ & $12.6 \pm 2.4$\\
03333313-3215181 & (M6.1) & THA & $66.6$ & $< 0.1$ & $39.0^{+9.3}_{-6.0}$ & $45.8 \pm 3.2$ & $13.7 \pm 2.1$\\
03341065-2130343 & M6 & BPMG & $22.9$ & $12.0$ & $20.5^{+3.6}_{-2.1}$ & $18.1^{+1.6}_{-2.0}$ & $19.0 \pm 0.8$\\
03355693-1030568 & (M5.3) & ABDMG & $76.6$ & $2.6$ & $137.5^{+13.0}_{-11.3}$ & $26.9 \pm 1.6$ & $20.0 \pm 2.0$\\
03370362-3709236 & (M5.7) & THA & $48.9$ & $< 0.1$ & $56.0^{+7.8}_{-6.1}$ & $47.8 \pm 3.2$ & $14.2 \pm 2.0$\\
03391444+0217026 & (M5.8) & COL & $16.1$ & $< 0.1$ & $51.4^{+7.8}_{-6.7}$ & $47.8^{+4.4}_{-5.2}$ & $14.5 \pm 2.7$\\
03404953-1016298 & (M4.2) & COL & $91.5$ & $< 0.1$ & $145.3^{+19.1}_{-16.9}$ & $38.6^{+3.2}_{-2.8}$ & $16.8 \pm 1.5$\\
03455498-0929169 & (M5.3) & THA & $39.8$ & $< 0.1$ & $74.9^{+10.5}_{-8.4}$ & $57.0^{+4.0}_{-3.6}$ & $10.2 \pm 2.0$\\
03464992-2243173 & (M7.9) & THA & $38.1$ & $< 0.1$ & $24.8^{+5.3}_{-2.5}$ & $52.6 \pm 3.2$ & $11.3 \pm 2.1$\\
03492272-2112537 & (M7.3) & ABDMG & $19.4$ & $< 0.1$ & $53.3^{+5.3}_{-5.2}$ & $39.8^{+3.6}_{-4.0}$ & $24.3 \pm 2.4$\\
03514874-4736213 & (M5.2) & COL & $83.5$ & $< 0.1$ & $85.0^{+11.7}_{-11.4}$ & $45.0^{+5.2}_{-6.0}$ & $20.1 \pm 1.5$\\
03561624-3915219 & M5.0 & THA & $99.9$ & $< 0.1$ & $200.2^{+9.5}_{-6.6}$ & $45.8 \pm 3.2$ & $16.7 \pm 0.7$\\
04011423-1304570 & (M5.0) & COL & $90.5$ & $< 0.1$ & $96.1^{+13.0}_{-12.3}$ & $42.6^{+4.0}_{-4.8}$ & $18.9 \pm 2.0$\\
04013874-3127472 & (M4.9) & COL & $94.8$ & $< 0.1$ & $99.2 \pm 13.7$ & $50.6^{+6.0}_{-6.4}$ & $20.6 \pm 1.8$\\
04032484+0824508 & (M5.0) & BPMG & $96.7$ & $14.1$ & $86.1^{+7.4}_{-7.8}$ & $25.7^{+3.2}_{-3.6}$ & $14.2 \pm 2.2$\\
04054799-1515399 & M8 & THA & $70.1$ & $< 0.1$ & $40.1^{+9.2}_{-6.3}$ & $54.6 \pm 4.0$ & $12.4 \pm 2.2$\\
04055753-3704468 & (M5.3) & THA & $90.6$ & $< 0.1$ & $71.6^{+10.2}_{-8.4}$ & $42.2^{+3.2}_{-2.8}$ & $14.9 \pm 2.1$\\
04100670-7316244 & (M5.2) & THA & $89.0$ & $< 0.1$ & $89.4^{+11.6}_{-9.8}$ & $49.4 \pm 3.6$ & $12.1 \pm 2.0$\\
04111790-0556489 & M9 & COL & $20.6$ & $8.1$ & $15.2^{+0.7}_{-6.3}$ & $53.0 \pm 4.8$ & $20.1 \pm 5.0$\\
04131526-1256319 & (M5.2) & COL & $87.3$ & $14.0$ & $86.8^{+11.6}_{-10.7}$ & $47.0^{+4.8}_{-5.2}$ & $19.6 \pm 2.0$\\
04133609-4413325 & M3.9 & THA & $99.6$ & $< 0.1$ & $193.6^{+14.2}_{-11.1}$ & $49.4 \pm 3.6$ & $16.4 \pm 1.4$\\
04143504-1001030 & (M5.8) & COL & $67.0$ & $6.2$ & $51.0^{+7.7}_{-6.4}$ & $25.3^{+2.4}_{-2.0}$ & $19.4 \pm 1.5$\\
04194254-2238345 & (M5.4) & THA & $46.5$ & $< 0.1$ & $67.3^{+9.6}_{-7.8}$ & $48.6^{+3.6}_{-4.0}$ & $13.4 \pm 2.1$\\
04231498-1533245 & (M8.1) & BPMG & $93.3$ & $1.2$ & $15.0^{+0.3}_{-0.1}$ & $22.4 \pm 1.0$ & $19.3 \pm 1.5$\\
04413536-3111054 & (M5.9) & COL & $94.9$ & $9.4$ & $49.9^{+7.8}_{-7.2}$ & $45.8^{+5.6}_{-5.2}$ & $22.2 \pm 1.5$\\
04425799-2651074 & (M5.4) & COL & $35.2$ & $15.0$ & $68.3^{+10.0}_{-9.1}$ & $51.0^{+6.0}_{-5.6}$ & $22.1 \pm 1.7$\\
04475779-5035200 & M4.0 & COL & $72.0$ & $10.0$ & $196.1^{+15.1}_{-9.6}$ & $54.2^{+7.2}_{-8.0}$ & $18.6 \pm 0.9$\\
04581330-3754491 & (M5.0) & COL & $94.6$ & $10.5$ & $92.9^{+13.2}_{-13.9}$ & $51.4^{+8.0}_{-7.2}$ & $22.7 \pm 1.4$\\
04584239-3002061 & (M7.3) & COL & $17.8$ & $12.7$ & $28.8^{+6.0}_{-3.9}$ & $40.6^{+4.8}_{-3.6}$ & $23.1 \pm 1.4$\\
04584686-4343421 & (M5.4) & COL & $90.5$ & $12.9$ & $71.2^{+10.9}_{-10.7}$ & $53.8^{+8.0}_{-7.2}$ & $22.4 \pm 1.5$\\
05010082-4337102 & (M4.5) & COL & $55.9$ & $14.1$ & $118.8^{+17.4}_{-18.8}$ & $47.8^{+8.4}_{-7.2}$ & $22.4 \pm 1.4$\\
05012725-5708012 & (M5.8) & CAR & $80.4$ & $< 0.1$ & $51.0^{+7.7}_{-6.3}$ & $36.6 \pm 3.2$ & $20.8 \pm 1.0$\\
05014639-2512183 & (M7.7) & COL & $81.5$ & $14.1$ & $22.7^{+5.4}_{-4.5}$ & $56.6^{+6.4}_{-5.2}$ & $22.8 \pm 1.5$\\
05035585-2328109 & (M5.8) & COL & $93.1$ & $10.3$ & $56.3^{+8.4}_{-7.9}$ & $51.0^{+7.2}_{-6.0}$ & $22.5 \pm 1.7$\\
05071519-2907205 & (M5.4) & COL & $64.2$ & $14.3$ & $70.3^{+10.6}_{-10.3}$ & $53.8^{+7.6}_{-6.8}$ & $22.7 \pm 1.7$\\
05073494-4200301 & (M6.8) & COL & $74.5$ & $9.0$ & $34.3^{+7.9}_{-6.3}$ & $37.0^{+5.2}_{-4.8}$ & $22.9 \pm 1.4$\\
05104958-1843548 & (L2.6) & COL & $25.2$ & $10.0$ & $11.7^{+0.3}_{-0.1}$ & $26.5 \pm 2.4$ & $23.2 \pm 1.3$\\
05113330-5551371 & (M5.2) & CAR & $68.8$ & $14.3$ & $86.9^{+11.6}_{-10.5}$ & $43.8^{+4.0}_{-4.8}$ & $21.0 \pm 1.1$\\
05121347+0131539 & (M4.9) & ABDMG & $80.3$ & $2.8$ & $178.9^{+16.0}_{-14.8}$ & $24.1 \pm 1.6$ & $19.7 \pm 1.8$\\
05170387-8055573 & (M5.7) & CAR & $50.7$ & $12.6$ & $56.1^{+8.1}_{-7.1}$ & $64.2^{+7.2}_{-6.0}$ & $17.6 \pm 1.1$\\
05195412-0723359 & M4+M4.5 & COL & $89.7$ & $7.2$ & $102.4^{+13.7}_{-12.1}$ & $33.8 \pm 2.8$ & $22.1 \pm 1.4$\\
05300976-4444561 & (M5.5) & COL & $82.9$ & $12.5$ & $67.3 \pm 10.3$ & $47.4^{+7.6}_{-6.8}$ & $23.1 \pm 1.4$\\
05315184-1611425 & (M3.8) & COL & $90.6$ & $11.9$ & $184.2^{+20.8}_{-16.9}$ & $45.0^{+5.6}_{-4.8}$ & $22.9 \pm 1.4$\\
05320932-4607036 & (M5.7) & CAR & $66.4$ & $14.3$ & $58.9^{+8.4}_{-7.0}$ & $35.4^{+3.2}_{-2.8}$ & $22.7 \pm 1.0$\\
06075808-6115107 & (M5.2) & ARG & $81.1$ & $13.2$ & $102.7^{+10.3}_{-10.2}$ & $18.5 \pm 1.6$ & $11.0 \pm 2.2$\\
06101564-5805143 & (L2.1) & CAR & $86.7$ & $4.0$ & $12.0^{+0.8}_{-0.3}$ & $43.0^{+4.8}_{-4.4}$ & $22.0 \pm 1.1$\\
06234738-5351131 & (M4.1) & CAR & $44.3$ & $6.9$ & $153.8^{+20.9}_{-20.5}$ & $33.3^{+4.4}_{-3.6}$ & $22.1 \pm 0.8$\\
06240437-5948063 & (M7.3) & CAR & $57.7$ & $9.1$ & $28.8^{+5.6}_{-3.5}$ & $53.8^{+5.6}_{-4.4}$ & $21.4 \pm 1.1$\\
06313103-8811365 & M5 & ARG & $28.1$ & $4.8$ & $55.2^{+5.6}_{-5.4}$ & $12.1^{+0.8}_{-1.2}$ & $2.2 \pm 1.8$\\
07024648-7540494 & (M5.8) & CAR & $24.4$ & $9.8$ & $56.0^{+8.4}_{-7.8}$ & $74.2^{+8.8}_{-10.0}$ & $19.3 \pm 1.4$\\
07135309-6545115 & (M6.0) & CAR & $91.5$ & $3.8$ & $43.6^{+8.1}_{-6.4}$ & $67.8^{+6.0}_{-7.6}$ & $20.8 \pm 1.3$\\
07140394+3702459 & M8 & ARG & $74.9$ & $0.6$ & $20.6^{+2.5}_{-1.7}$ & $12.5 \pm 0.7$ & $17.5 \pm 1.7$\\
07355465+3333459 & M4.5 & ABDMG & $26.2$ & $2.0$ & $146.9^{+13.9}_{-13.0}$ & $32.4 \pm 2.5$ & $3.2 \pm 2.4$\\
07380664-8121403 & (M5.3) & CAR & $91.9$ & $3.8$ & $74.3^{+10.7}_{-10.0}$ & $68.2^{+8.0}_{-7.2}$ & $18.0 \pm 1.3$\\
07435603-6744184 & (M4.9) & CAR & $17.0$ & $7.5$ & $103.9^{+14.4}_{-14.1}$ & $68.6^{+8.8}_{-7.6}$ & $20.4 \pm 1.1$\\
07525265-7916367 & (M6.8) & CAR & $50.0$ & $7.1$ & $36.9^{+9.2}_{-6.7}$ & $72.6^{+8.0}_{-9.2}$ & $18.3 \pm 1.4$\\
07550342-6717478 & (M4.7) & CAR & $98.3$ & $2.0$ & $113.4^{+15.5}_{-15.2}$ & $64.2^{+8.4}_{-7.2}$ & $20.1 \pm 1.1$\\
08122535-6852061 & (M4.7) & CAR & $90.3$ & $5.3$ & $110.2^{+14.9}_{-15.1}$ & $77.4^{+10.0}_{-8.8}$ & $19.7 \pm 1.3$\\
09285061-8610165 & (M4.4) & CAR & $10.8$ & $9.8$ & $131.1^{+18.0}_{-17.6}$ & $31.7^{+3.6}_{-4.0}$ & $17.7 \pm 1.8$\\
09395647-2946286 & (M5.1) & TWA & $15.4$ & $8.2$ & $39.0^{+8.2}_{-7.0}$ & $42.6^{+5.6}_{-6.0}$ & $15.9 \pm 1.5$\\
09400251-2229251 & (M3.9) & CAR & $69.5$ & $3.5$ & $159.8^{+20.6}_{-17.8}$ & $47.8^{+3.6}_{-3.2}$ & $20.3 \pm 1.1$\\
09515130-8215394 & (M4.9) & ARG & $18.1$ & $12.2$ & $115.8^{+12.1}_{-12.5}$ & $68.2^{+7.6}_{-7.2}$ & $1.9 \pm 2.1$\\
09533862-7929598 & (M3.7) & CAR & $79.4$ & $3.2$ & $183.4^{+20.8}_{-17.3}$ & $63.0^{+5.6}_{-6.0}$ & $17.9 \pm 1.4$\\
10023100-2814280 & M4+M6 & CAR & $93.7$ & $1.8$ & $208.0^{+2.2}_{-1.0}$ & $43.0^{+2.8}_{-3.2}$ & $19.7 \pm 1.0$\\
10134260-2759586 & M5 & CAR & $43.5$ & $3.5$ & $77.9^{+10.6}_{-8.9}$ & $46.6^{+3.2}_{-3.6}$ & $18.6 \pm 1.0$\\
10144705-3728151 & (M5.6) & TWA & $55.0$ & $2.9$ & $23.4^{+1.8}_{-2.8}$ & $49.8^{+6.8}_{-6.4}$ & $14.9 \pm 1.5$\\
10190109-2646336 & (M5.3) & TWA & $94.0$ & $1.6$ & $30.8^{+5.0}_{-8.9}$ & $40.2^{+4.8}_{-4.4}$ & $14.5 \pm 1.4$\\
10282500-3959230 & (M5.3) & CAR & $19.3$ & $6.2$ & $79.7^{+10.7}_{-8.6}$ & $26.1 \pm 1.6$ & $19.1 \pm 0.8$\\
10292874-3823394 & (M5.7) & TWA & $17.2$ & $4.2$ & $21.8^{+1.3}_{-1.8}$ & $53.4^{+6.4}_{-6.8}$ & $14.8 \pm 1.5$\\
10380178-2154225 & (M5.4) & TWA & $46.1$ & $5.0$ & $26.3^{+2.6}_{-8.2}$ & $36.6 \pm 4.0$ & $12.4 \pm 1.3$\\
10394605-3510139 & (M5.2) & TWA & $91.3$ & $1.8$ & $37.0^{+7.7}_{-6.7}$ & $55.4 \pm 6.8$ & $14.0 \pm 1.5$\\
10443052-3730554 & (M5.5) & TWA & $12.4$ & $7.3$ & $24.8^{+2.2}_{-4.2}$ & $58.6^{+6.8}_{-7.2}$ & $14.4 \pm 1.7$\\
10451718-2607249 & M8 & ABDMG & $18.2$ & $12.0$ & $46.9^{+4.5}_{-4.0}$ & $24.9 \pm 1.6$ & $17.3 \pm 1.5$\\
10455263-2819303 & (M5.7) & TWA & $56.0$ & $4.8$ & $22.5^{+1.4}_{-2.0}$ & $52.2^{+6.0}_{-5.6}$ & $13.3 \pm 1.5$\\
10492026-2440101 & (M5.6) & TWA & $30.3$ & $5.0$ & $23.8^{+1.8}_{-2.8}$ & $43.4 \pm 5.2$ & $13.0 \pm 1.5$\\
10542303-1507082 & (M5.2) & TWA & $51.4$ & $12.0$ & $37.7^{+7.7}_{-6.4}$ & $30.5^{+3.6}_{-3.2}$ & $12.1 \pm 1.3$\\
10563080-3028137 & (M4.7) & TWA & $12.1$ & $3.8$ & $55.7^{+8.6}_{-8.8}$ & $47.4^{+6.0}_{-5.6}$ & $12.7 \pm 1.5$\\
11023986-2507113 & (M4.3) & TWA & $81.1$ & $2.6$ & $70.3^{+11.1}_{-9.2}$ & $46.2 \pm 5.2$ & $11.9 \pm 1.5$\\
11034950-3409445 & (M9.4) & TWA & $35.7$ & $3.6$ & $11.4^{+0.8}_{-0.7}$ & $66.2^{+6.8}_{-7.2}$ & $12.7 \pm 1.7$\\
11062620-4019330 & (M5.4) & TWA & $39.8$ & $1.5$ & $26.4^{+2.9}_{-8.9}$ & $49.0^{+6.0}_{-6.4}$ & $13.0 \pm 1.5$\\
11150259-3759251 & (M8.4) & TWA & $94.8$ & $1.3$ & $13.1^{+0.6}_{-0.4}$ & $68.2^{+6.0}_{-5.6}$ & $12.6 \pm 1.5$\\
11152992-2954436 & (M5.2) & TWA & $83.8$ & $2.5$ & $37.0^{+7.7}_{-6.4}$ & $54.2^{+6.4}_{-6.0}$ & $12.4 \pm 1.5$\\
11160937-3601063 & (M5.6) & TWA & $99.0$ & $0.8$ & $23.1^{+1.5}_{-2.2}$ & $56.6 \pm 6.4$ & $12.3 \pm 1.7$\\
11191302-4342401 & (M5.2) & TWA & $87.2$ & $2.9$ & $35.4^{+7.1}_{-7.0}$ & $70.6^{+8.8}_{-8.4}$ & $13.0 \pm 1.5$\\
11204706-2738056 & (M4.5) & TWA & $31.4$ & $7.5$ & $60.7^{+9.1}_{-8.5}$ & $53.0 \pm 6.4$ & $12.1 \pm 1.5$\\
11271382-3735076 & (L2.5) & TWA & $87.1$ & $1.4$ & $9.3 \pm 0.7$ & $62.2^{+8.8}_{-8.0}$ & $12.3 \pm 2.0$\\
11283294-2924353 & (M5.0) & TWA & $63.3$ & $3.5$ & $41.5^{+8.6}_{-6.8}$ & $40.6 \pm 4.8$ & $10.7 \pm 1.5$\\
11382538-3841525 & (M3.9) & TWA & $98.9$ & $0.9$ & $90.7^{+10.3}_{-10.5}$ & $63.0 \pm 7.6$ & $11.7 \pm 1.7$\\
11382693-3843138 & (M4.6) & TWA & $99.0$ & $0.7$ & $59.1^{+8.6}_{-8.4}$ & $60.2^{+7.2}_{-6.8}$ & $11.4 \pm 1.5$\\
11423628-3859108 & (M5.2) & TWA & $98.3$ & $0.5$ & $35.8^{+7.2}_{-6.8}$ & $55.0 \pm 6.4$ & $11.0 \pm 1.7$\\
11430143-3927002 & (M5.3) & TWA & $97.9$ & $0.7$ & $33.0^{+6.1}_{-7.8}$ & $62.6^{+7.6}_{-6.8}$ & $11.4 \pm 1.5$\\
11443034-3820341 & (M4.3) & TWA & $77.9$ & $1.5$ & $69.8^{+11.1}_{-9.6}$ & $64.2^{+7.6}_{-8.0}$ & $12.0 \pm 1.7$\\
11443970-3455026 & (M5.5) & TWA & $72.9$ & $1.7$ & $23.9^{+1.8}_{-2.5}$ & $49.8^{+5.6}_{-5.2}$ & $10.3 \pm 1.5$\\
11501755-3407074 & (M5.2) & TWA & $74.6$ & $2.9$ & $36.9^{+7.5}_{-6.6}$ & $31.3 \pm 3.6$ & $10.0 \pm 1.5$\\
11511119-4132064 & (M5.6) & TWA & $59.7$ & $1.8$ & $23.5^{+1.8}_{-2.5}$ & $68.6^{+8.0}_{-8.4}$ & $12.1 \pm 1.7$\\
11554920-4303109 & (M4.1) & TWA & $69.7$ & $3.0$ & $75.4^{+10.3}_{-10.2}$ & $75.0^{+8.8}_{-9.2}$ & $12.1 \pm 1.7$\\
11561415-3917217 & (M5.8) & TWA & $98.8$ & $0.6$ & $21.3^{+1.1}_{-1.5}$ & $54.2 \pm 6.0$ & $10.5 \pm 1.5$\\
11571557-4022292 & (M5.2) & TWA & $10.4$ & $12.9$ & $36.5^{+7.4}_{-6.7}$ & $74.2^{+8.8}_{-9.2}$ & $12.3 \pm 1.7$\\
12011772-3712329 & (M5.0) & TWA & $38.1$ & $13.0$ & $45.0^{+10.0}_{-7.8}$ & $72.6 \pm 8.0$ & $11.3 \pm 1.7$\\
12012242-4103432 & (M5.3) & TWA & $95.4$ & $1.6$ & $29.1^{+3.9}_{-9.5}$ & $73.8^{+8.4}_{-7.6}$ & $11.2 \pm 1.7$\\
12023799-3328402 & (M3.6) & TWA & $98.3$ & $1.2$ & $159.8^{+16.0}_{-16.9}$ & $57.4^{+6.4}_{-6.0}$ & $10.0 \pm 1.7$\\
12072486-3608359 & (M5.8) & TWA & $86.5$ & $1.8$ & $20.6^{+0.8}_{-1.3}$ & $65.0 \pm 6.8$ & $10.5 \pm 1.7$\\
12093096-3820290 & (M6.4) & TWA & $52.9$ & $8.4$ & $17.7^{+0.7}_{-0.6}$ & $75.8^{+8.0}_{-7.6}$ & $11.0 \pm 1.7$\\
12105770-3708100 & (M7.1) & TWA & $65.9$ & $1.8$ & $15.7 \pm 0.6$ & $61.4^{+6.0}_{-6.8}$ & $9.5 \pm 2.0$\\
12120009-3519434 & (M5.2) & TWA & $43.1$ & $9.0$ & $36.9^{+7.7}_{-6.4}$ & $70.2 \pm 7.6$ & $10.7 \pm 1.7$\\
12173617-2846082 & (M5.8) & TWA & $36.1$ & $7.8$ & $21.3^{+1.0}_{-1.4}$ & $49.0^{+4.8}_{-5.2}$ & $8.5 \pm 1.8$\\
12193723-3132237 & (M5.3) & TWA & $55.9$ & $3.7$ & $32.2^{+5.7}_{-8.2}$ & $56.2^{+6.0}_{-6.4}$ & $9.6 \pm 1.8$\\
12220574-4159572 & (M5.3) & TWA & $97.6$ & $1.2$ & $34.4^{+6.8}_{-7.2}$ & $72.2^{+8.0}_{-8.4}$ & $10.3 \pm 1.8$\\
12281366-4316388 & (M4.6) & ARG & $14.5$ & $3.0$ & $137.7^{+14.6}_{-14.9}$ & $49.0 \pm 5.2$ & $-0.6 \pm 1.7$\\
12333935-3040139 & (M7.7) & TWA & $14.5$ & $9.6$ & $14.6 \pm 0.4$ & $62.6^{+6.0}_{-5.6}$ & $8.8 \pm 1.8$\\
12384389-2705384 & (M5.8) & TWA & $20.1$ & $12.0$ & $20.6^{+0.8}_{-1.3}$ & $57.8^{+6.0}_{-5.6}$ & $8.3 \pm 1.8$\\
12414195-3625573 & (M4.3) & TWA & $94.8$ & $1.3$ & $70.2^{+11.0}_{-9.2}$ & $59.0^{+6.8}_{-6.4}$ & $8.5 \pm 1.8$\\
12471536-3252233 & (M5.6) & TWA & $43.5$ & $5.4$ & $23.0^{+1.5}_{-2.0}$ & $59.4^{+6.4}_{-6.0}$ & $8.1 \pm 2.0$\\
12522053-4515542 & (M5.1) & TWA & $47.3$ & $4.9$ & $41.8^{+8.6}_{-6.4}$ & $81.8^{+8.8}_{-8.4}$ & $9.2 \pm 1.7$\\
12574463-3635431 & (M7.2) & TWA & $23.0$ & $5.7$ & $15.6^{+0.4}_{-0.6}$ & $69.4^{+6.4}_{-7.6}$ & $8.9 \pm 2.1$\\
13075615-4159202 & (M5.4) & TWA & $15.2$ & $3.1$ & $25.7^{+2.4}_{-6.7}$ & $64.6^{+6.8}_{-7.6}$ & $8.1 \pm 2.1$\\
13110859-3725022 & (M5.8) & TWA & $25.8$ & $5.2$ & $20.2^{+0.8}_{-1.1}$ & $68.2^{+7.2}_{-7.6}$ & $8.3 \pm 2.1$\\
13153357-3425084 & (M5.8) & TWA & $24.8$ & $7.3$ & $19.9^{+0.7}_{-1.0}$ & $59.0 \pm 6.0$ & $6.8 \pm 2.0$\\
13191194-3600082 & (M5.7) & TWA & $15.7$ & $6.9$ & $21.6^{+1.1}_{-1.5}$ & $65.0^{+6.8}_{-7.2}$ & $7.8 \pm 2.2$\\
18323637-8500364 & (M3.9) & THA & $13.5$ & $< 0.1$ & $164.1^{+21.2}_{-19.1}$ & $56.2^{+4.8}_{-4.4}$ & $8.9 \pm 2.4$\\
19002383-6120156 & (M5.3) & BPMG & $96.0$ & $8.5$ & $77.2^{+4.6}_{-5.3}$ & $26.9 \pm 2.4$ & $0.9 \pm 2.2$\\
19472488-7055187 & (M4.7) & THA & $11.2$ & $< 0.1$ & $118.8^{+15.2}_{-13.0}$ & $50.6^{+3.6}_{-3.2}$ & $6.2 \pm 2.1$\\
19501998-4327025 & (M4.3) & ARG & $64.2$ & $12.8$ & $151.6^{+17.8}_{-19.5}$ & $26.5^{+4.0}_{-3.6}$ & $-16.8 \pm 1.7$\\
20154344-6354097 & (M5.3) & ABDMG & $76.7$ & $4.8$ & $137.8^{+13.0}_{-11.7}$ & $30.9 \pm 2.0$ & $13.0 \pm 1.7$\\
20172696-5843359 & (M5.7) & THA & $65.0$ & $< 0.1$ & $53.8^{+7.7}_{-6.1}$ & $53.0^{+3.6}_{-4.0}$ & $0.4 \pm 2.4$\\
21134380-7013153 & (M3.7) & THA & $87.0$ & $< 0.1$ & $176.8^{+22.0}_{-19.1}$ & $48.6 \pm 3.2$ & $5.7 \pm 2.4$\\
21144103-4339531 & (M6.1) & ABDMG & $74.5$ & $5.9$ & $75.5^{+6.8}_{-6.6}$ & $41.8 \pm 2.4$ & $2.7 \pm 0.3$\\
21272613-4215183 & M8 & BPMG & $82.5$ & $0.6$ & $21.6^{+4.3}_{-5.0}$ & $34.6 \pm 7.5$ & $-7.6 \pm 0.3$\\
21380269-5744583 & M3.7 & THA & $98.7$ & $< 0.1$ & $187.7^{+18.0}_{-14.9}$ & $48.6^{+2.8}_{-3.2}$ & $-0.5 \pm 1.3$\\
21414678-2704542 & M4.5 & ABDMG & $45.7$ & $2.1$ & $122.8^{+12.4}_{-11.0}$ & $21.3 \pm 1.2$ & $-1.1 \pm 1.8$\\
21503526-5818010 & (M5.8) & THA & $92.4$ & $< 0.1$ & $49.3^{+7.5}_{-5.9}$ & $49.4 \pm 3.2$ & $1.6 \pm 2.5$\\
21521075-6145371 & (M6.3) & THA & $64.1$ & $< 0.1$ & $36.8^{+8.9}_{-6.0}$ & $51.8 \pm 3.2$ & $1.8 \pm 2.2$\\
21522126-5209212 & (M5.7) & THA & $33.8$ & $< 0.1$ & $51.8^{+7.5}_{-5.6}$ & $39.4^{+2.4}_{-2.0}$ & $-0.5 \pm 2.2$\\
22021125-1109461 & M6.5 & ABDMG & $84.9$ & $1.3$ & $65.7^{+6.1}_{-5.7}$ & $28.1^{+1.6}_{-2.0}$ & $-9.4 \pm 1.0$\\
22062377-7627110 & (M5.8) & THA & $94.0$ & $< 0.1$ & $49.0^{+7.5}_{-5.9}$ & $50.6^{+3.2}_{-3.6}$ & $8.1 \pm 2.4$\\
22082542-5315305 & (M5.2) & THA & $19.8$ & $< 0.1$ & $88.6^{+11.4}_{-9.2}$ & $50.2 \pm 3.2$ & $0.4 \pm 2.4$\\
22191486-6828018 & (M7.0) & THA & $16.6$ & $< 0.1$ & $33.0^{+6.7}_{-4.5}$ & $56.2^{+3.6}_{-3.2}$ & $5.1 \pm 2.4$\\
22305171+0939510 & (M6.6) & ABDMG & $68.2$ & $5.1$ & $67.1^{+6.3}_{-5.9}$ & $34.2 \pm 2.4$ & $-12.7 \pm 2.0$\\
22345110+0145137 & (M5.3) & ABDMG & $88.1$ & $1.6$ & $129.7^{+12.5}_{-11.1}$ & $26.5 \pm 1.6$ & $-9.3 \pm 2.1$\\
22400704-7112205 & (M5.3) & THA & $99.0$ & $< 0.1$ & $70.3^{+10.2}_{-7.7}$ & $47.0^{+3.2}_{-2.8}$ & $6.7 \pm 2.5$\\
22422096-4103566 & (M4.6) & THA & $27.1$ & $< 0.1$ & $123.4^{+15.6}_{-13.0}$ & $45.4 \pm 2.8$ & $-2.7 \pm 2.2$\\
22541103+1606546 & M4 & ARG & $68.8$ & $0.8$ & $155.1^{+14.6}_{-12.8}$ & $30.2 \pm 1.3$ & $-7.1 \pm 1.3$\\
23005950-4013010 & (M5.1) & THA & $64.6$ & $< 0.1$ & $94.3^{+12.3}_{-10.0}$ & $39.4 \pm 2.4$ & $-1.6 \pm 2.2$\\
23014396-5935316 & (M5.7) & THA & $35.3$ & $< 0.1$ & $51.3^{+7.5}_{-5.9}$ & $51.4 \pm 3.2$ & $3.4 \pm 2.4$\\
23102196-0748531 & (M5.9) & BPMG & $57.7$ & $12.4$ & $42.8^{+2.6}_{-2.5}$ & $24.1 \pm 2.0$ & $-1.9 \pm 1.5$\\
23133055-5352079 & (M5.7) & THA & $63.7$ & $< 0.1$ & $61.7^{+8.8}_{-6.6}$ & $37.8 \pm 2.4$ & $2.7 \pm 2.4$\\
23143092-5405313 & (M4.7) & THA & $81.5$ & $< 0.1$ & $121.2^{+15.6}_{-13.4}$ & $46.6 \pm 2.8$ & $2.7 \pm 2.7$\\
23170894-3754485 & (M5.3) & ABDMG & $53.3$ & $2.0$ & $130.4^{+12.7}_{-11.3}$ & $22.5^{+1.2}_{-1.6}$ & $9.7 \pm 1.8$\\
23252516-6740080 & (M5.1) & ABDMG & $87.3$ & $1.6$ & $168.5^{+15.2}_{-13.9}$ & $18.9 \pm 1.2$ & $19.7 \pm 1.5$\\
23261182+1700082 & M4.5+M6 & BPMG & $66.8$ & $11.8$ & $206.5^{+4.3}_{-2.2}$ & $28.9 \pm 2.4$ & $-4.8 \pm 1.7$\\
23270960-8515209 & (M3.5) & THA & $77.3$ & $< 0.1$ & $199.5^{+10.2}_{-7.0}$ & $49.4^{+4.0}_{-3.6}$ & $8.9 \pm 2.9$\\
23271378-4815022 & (M5.7) & THA & $77.7$ & $< 0.1$ & $49.9^{+7.4}_{-5.7}$ & $37.8 \pm 2.0$ & $1.9 \pm 2.4$\\
23310161-0406193 & M8+L3 & ABDMG & $99.0$ & $0.1$ & $45.3^{+3.6}_{-3.2}$ & $26.1 \pm 0.4$ & $-2.0 \pm 2.1$\\
23361580-3916080 & (M5.3) & THA & $58.4$ & $12.4$ & $88.2^{+11.4}_{-9.1}$ & $36.2 \pm 2.0$ & $0.4 \pm 2.1$\\
23364060-1622292 & (M5.7) & ABDMG & $34.2$ & $7.6$ & $93.2^{+9.1}_{-8.5}$ & $36.6 \pm 2.4$ & $3.7 \pm 2.1$\\
23371616-6252226 & (M6.1) & THA & $59.4$ & $< 0.1$ & $40.2^{+8.9}_{-5.9}$ & $50.6 \pm 3.2$ & $5.7 \pm 2.5$\\
23372366-8004524 & (M5.6) & THA & $40.2$ & $< 0.1$ & $63.8^{+9.1}_{-7.0}$ & $51.0^{+3.2}_{-3.6}$ & $11.3 \pm 2.4$\\
23421895+1138362 & (M5.7) & ABDMG & $27.4$ & $11.7$ & $102.5^{+10.3}_{-9.8}$ & $39.0 \pm 2.8$ & $-6.8 \pm 2.2$\\
23450137-3108048 & (M5.3) & THA & $39.0$ & $< 0.1$ & $84.3^{+11.0}_{-8.5}$ & $39.4^{+2.4}_{-2.0}$ & $-2.5 \pm 2.1$\\
23461092-0519325 & (M5.7) & BPMG & $77.8$ & $10.0$ & $54.0^{+3.1}_{-3.5}$ & $24.5 \pm 2.0$ & $0.6 \pm 1.5$\\
23515597-6447345 & (M3.5) & THA & $99.6$ & $< 0.1$ & $191.2^{+15.6}_{-12.7}$ & $47.4^{+3.2}_{-2.8}$ & $6.2 \pm 2.4$\\
23524562-5229593 & M4.6 & THA & $99.9$ & $< 0.1$ & $104.1^{+13.7}_{-11.1}$ & $43.0 \pm 2.4$ & $3.1 \pm 0.7$\\
23532556-1844402 & (M5.2) & BPMG & $17.6$ & $< 0.1$ & $84.4^{+5.6}_{-5.9}$ & $33.3 \pm 3.2$ & $3.7 \pm 1.5$\\
23563848-6753300 & (M6.0) & THA & $13.9$ & $< 0.1$ & $43.7^{+7.4}_{-5.6}$ & $53.8 \pm 3.2$ & $7.9 \pm 2.5$\\
\cutinhead{Candidates with a Modest Probability}
00085614-2813211 & (L8.9) & BPMG & $21.5$ & $21.8$ & $6.1 \pm 0.1$ & $16.1 \pm 1.2$ & $5.8 \pm 1.5$\\
00102936-0746487 & (M6.2) & ABDMG & $18.2$ & $19.9$ & $74.3^{+7.0}_{-6.6}$ & $43.8^{+3.2}_{-2.8}$ & $3.3 \pm 2.1$\\
00192753-3620153 & M5.5 & THA & $11.5$ & $43.0$ & $60.3^{+8.6}_{-6.8}$ & $37.8^{+2.0}_{-2.4}$ & $0.9 \pm 2.2$\\
00193193-0554404 & (M5.0) & BPMG & $30.8$ & $44.2$ & $89.9^{+6.4}_{-6.1}$ & $33.8^{+3.6}_{-3.2}$ & $3.2 \pm 1.7$\\
00281434-3227556 & M5 & BPMG & $30.4$ & $45.7$ & $168.7^{+10.6}_{-11.1}$ & $32.1^{+2.8}_{-3.2}$ & $8.1 \pm 1.5$\\
00324451+2744454 & (M5.0) & BPMG & $17.4$ & $36.0$ & $93.9 \pm 5.6$ & $35.8 \pm 3.2$ & $-3.6 \pm 2.0$\\
00465095+3822416 & (M5.5) & ARG & $15.8$ & $28.2$ & $77.3^{+7.9}_{-8.2}$ & $33.8^{+3.2}_{-3.6}$ & $2.3 \pm 1.7$\\
00473149-1424425 & (M4.8) & BPMG & $54.3$ & $34.2$ & $100.0^{+5.7}_{-6.3}$ & $30.9 \pm 2.8$ & $6.9 \pm 1.5$\\
00584590+2430511 & (M5.8) & BPMG & $24.8$ & $27.3$ & $46.8 \pm 2.6$ & $31.3 \pm 2.8$ & $2.2 \pm 2.1$\\
01012488-2412472 & (M6.0) & BPMG & $12.1$ & $30.2$ & $41.5^{+2.8}_{-2.5}$ & $23.3 \pm 2.0$ & $9.3 \pm 1.5$\\
01044008+1129485 & (M5.3) & BPMG & $76.5$ & $26.1$ & $68.3 \pm 4.9$ & $32.9^{+3.2}_{-3.6}$ & $2.0 \pm 2.0$\\
01152518+4410518 & (M5.2) & ARG & $11.3$ & $20.0$ & $98.5 \pm 10.2$ & $31.7^{+3.2}_{-2.8}$ & $3.4 \pm 1.7$\\
01234181-3833496 & M4.5 & BPMG & $0.6$ & $54.4$ & $37.2 \pm 3.8$ & $14.5^{+1.6}_{-2.0}$ & $18.4 \pm 6.3$\\
01425614+3426237 & (M4.5) & ABDMG & $59.1$ & $17.7$ & $202.6^{+7.5}_{-4.9}$ & $43.0 \pm 2.8$ & $-6.7 \pm 1.8$\\
02020653+2006560 & (M5.6) & BPMG & $43.2$ & $47.4$ & $58.8^{+4.0}_{-4.3}$ & $38.6 \pm 3.6$ & $6.5 \pm 2.0$\\
02033222+0648588 & (M4.5) & BPMG & $64.5$ & $19.6$ & $115.4^{+7.9}_{-8.4}$ & $27.7 \pm 2.8$ & $7.2 \pm 1.8$\\
02050852-2101390 & (M5.3) & ABDMG & $24.5$ & $25.8$ & $126.5^{+13.0}_{-12.1}$ & $42.6 \pm 3.6$ & $17.6 \pm 2.1$\\
02143767+2435486 & (M5.3) & BPMG & $45.3$ & $28.3$ & $68.8 \pm 4.3$ & $32.9^{+2.8}_{-3.2}$ & $7.1 \pm 2.1$\\
02155737+0538072 & (M6.5) & ABDMG & $25.1$ & $20.6$ & $69.9^{+6.8}_{-6.7}$ & $42.2^{+4.4}_{-4.0}$ & $8.5 \pm 3.1$\\
02272166+2356559 & (L9.0) & ARG & $29.0$ & $15.5$ & $5.8^{+0.3}_{-0.1}$ & $14.9 \pm 1.2$ & $13.1 \pm 2.0$\\
02281391-6248045 & (M5.2) & ARG & $77.7$ & $28.6$ & $100.0 \pm 10.0$ & $22.5 \pm 2.0$ & $6.5 \pm 2.1$\\
02513113+2413154 & (M4.8) & ABDMG & $22.8$ & $15.8$ & $189.4^{+15.7}_{-13.1}$ & $41.4^{+4.0}_{-3.6}$ & $4.3 \pm 3.2$\\
02540607+0527119 & (M5.3) & BPMG & $63.2$ & $46.9$ & $72.9^{+5.3}_{-5.6}$ & $34.2^{+4.0}_{-3.6}$ & $12.3 \pm 2.1$\\
03090022-4924513 & M4.5 & ARG & $18.8$ & $58.8$ & $114.0^{+11.4}_{-11.6}$ & $25.3 \pm 2.4$ & $11.6 \pm 2.4$\\
03103597-1046072 & (M5.7) & BPMG & $37.4$ & $39.0$ & $56.3^{+4.3}_{-5.0}$ & $28.1 \pm 3.2$ & $14.5 \pm 1.8$\\
03170737-8126555 & (M5.6) & CAR & $12.5$ & $38.7$ & $61.6^{+8.9}_{-7.4}$ & $76.6^{+7.6}_{-6.8}$ & $16.9 \pm 1.3$\\
03182597-3708118 & (M5.8) & COL & $59.0$ & $41.0$ & $51.4^{+7.7}_{-7.0}$ & $59.0^{+6.4}_{-6.0}$ & $18.2 \pm 1.7$\\
03224269+7932066 & (M5.3) & ABDMG & $12.4$ & $37.5$ & $132.2^{+13.0}_{-12.0}$ & $26.9 \pm 2.0$ & $-20.4 \pm 1.4$\\
03264032+0513352 & (M5.3) & BPMG & $81.1$ & $16.4$ & $70.2 \pm 5.0$ & $26.1 \pm 2.8$ & $13.1 \pm 2.0$\\
03283911-1537333 & (M5.4) & ARG & $32.3$ & $48.4$ & $79.4 \pm 8.1$ & $16.9 \pm 1.6$ & $18.6 \pm 2.4$\\
03320901-3042409 & (M3.6) & ABDMG & $54.0$ & $45.8$ & $361.9^{+29.6}_{-26.8}$ & $39.8^{+4.0}_{-3.6}$ & $25.7 \pm 2.0$\\
03370359-1758079 & L4.5 & ARG & $11.6$ & $40.4$ & $10.3^{+0.7}_{-0.3}$ & $16.5 \pm 1.6$ & $16.9 \pm 2.4$\\
03401701-4149000 & (M4.4) & COL & $54.6$ & $28.5$ & $128.5^{+17.4}_{-17.1}$ & $60.2^{+7.6}_{-6.8}$ & $19.6 \pm 1.7$\\
03421667-7029176 & (M5.8) & CAR & $54.3$ & $33.9$ & $53.3^{+7.8}_{-6.8}$ & $60.2^{+5.6}_{-6.0}$ & $18.2 \pm 1.1$\\
03460432-2104472 & (M5.6) & ABDMG & $20.4$ & $23.7$ & $111.2^{+11.6}_{-10.9}$ & $34.2 \pm 2.8$ & $24.2 \pm 2.0$\\
03470321-2612598 & (M7.1) & COL & $28.2$ & $43.4$ & $30.6^{+6.4}_{-4.3}$ & $63.4^{+7.2}_{-6.0}$ & $19.3 \pm 2.0$\\
03505949+1414017 & (M4.4) & BPMG & $68.8$ & $24.1$ & $124.4^{+10.5}_{-11.1}$ & $27.3^{+3.6}_{-3.2}$ & $14.1 \pm 2.1$\\
04014383-3954451 & (M5.2) & COL & $73.2$ & $17.3$ & $82.9^{+11.7}_{-11.3}$ & $49.8^{+6.0}_{-6.8}$ & $20.8 \pm 1.8$\\
04051027-4319337 & (M7.4) & COL & $14.3$ & $48.6$ & $26.3^{+7.2}_{-4.5}$ & $69.8^{+7.6}_{-9.2}$ & $20.4 \pm 2.1$\\
04063659-4912526 & (M4.0) & COL & $60.0$ & $27.2$ & $156.1^{+21.3}_{-21.2}$ & $66.2^{+8.8}_{-8.0}$ & $20.3 \pm 1.7$\\
04084537-4747089 & (M4.1) & COL & $27.3$ & $47.2$ & $156.1^{+21.5}_{-21.3}$ & $75.8^{+10.0}_{-9.6}$ & $20.3 \pm 1.7$\\
04132960-4821508 & (M5.8) & COL & $15.5$ & $44.4$ & $56.3^{+8.2}_{-7.7}$ & $69.4^{+8.8}_{-8.0}$ & $20.7 \pm 1.7$\\
04163317-2535500 & (M5.4) & ABDMG & $51.1$ & $18.8$ & $120.8^{+12.8}_{-12.3}$ & $29.3 \pm 2.8$ & $26.4 \pm 2.0$\\
04222769-7321116 & (M6.4) & CAR & $11.8$ & $43.3$ & $38.4^{+9.3}_{-6.4}$ & $76.2^{+8.0}_{-9.2}$ & $18.4 \pm 1.3$\\
04231392+7144031 & (M4.8) & ABDMG & $18.0$ & $38.8$ & $192.3^{+14.5}_{-11.6}$ & $32.9 \pm 2.4$ & $-16.3 \pm 1.4$\\
04232280-3901212 & (M4.5) & COL & $89.6$ & $16.5$ & $123.3^{+16.9}_{-17.1}$ & $60.2^{+8.0}_{-7.6}$ & $21.4 \pm 1.5$\\
04254621-2153590 & (M5.1) & ABDMG & $47.6$ & $28.1$ & $164.1^{+15.5}_{-14.9}$ & $33.3 \pm 2.8$ & $26.0 \pm 2.0$\\
04312637-8042362 & (M3.6) & CAR & $12.4$ & $23.0$ & $206.2^{+5.0}_{-2.4}$ & $71.8^{+8.8}_{-10.4}$ & $17.9 \pm 1.4$\\
04331363-3717454 & (M5.6) & COL & $64.7$ & $22.9$ & $62.3^{+9.5}_{-9.3}$ & $62.2^{+8.8}_{-9.6}$ & $21.5 \pm 2.0$\\
04331474-1149505 & (M5.2) & COL & $24.0$ & $24.4$ & $83.3^{+11.1}_{-10.0}$ & $57.4^{+6.0}_{-5.2}$ & $20.0 \pm 1.8$\\
04332964-0059393 & (M4.0) & COL & $64.3$ & $17.2$ & $158.3^{+20.9}_{-19.5}$ & $49.8^{+5.2}_{-4.8}$ & $18.3 \pm 2.2$\\
04364599-0107487 & (M5.7) & COL & $22.4$ & $17.4$ & $60.3^{+8.8}_{-7.9}$ & $47.4^{+5.6}_{-5.2}$ & $19.3 \pm 2.7$\\
04382150-0512464 & (M5.8) & COL & $25.0$ & $31.2$ & $52.8^{+7.7}_{-6.6}$ & $55.8^{+5.2}_{-4.8}$ & $19.1 \pm 1.8$\\
04390494-0959012 & M6 & ABDMG & $15.4$ & $27.1$ & $74.8^{+7.0}_{-6.7}$ & $35.4^{+2.4}_{-2.8}$ & $22.9 \pm 2.1$\\
04424872+0457431 & (M8.0) & COL & $11.4$ & $37.9$ & $22.3^{+4.6}_{-3.2}$ & $53.4^{+4.4}_{-4.0}$ & $17.7 \pm 2.0$\\
04484076-0145269 & (M5.3) & COL & $62.4$ & $16.8$ & $78.2^{+11.0}_{-10.0}$ & $47.8^{+4.8}_{-5.6}$ & $19.6 \pm 2.2$\\
04493186-4044022 & (M6.3) & COL & $15.8$ & $23.3$ & $45.8^{+8.4}_{-7.4}$ & $52.2^{+6.8}_{-7.6}$ & $22.5 \pm 1.5$\\
04511750-5154282 & (M6.3) & COL & $40.5$ & $30.3$ & $42.1^{+8.9}_{-7.1}$ & $66.6^{+9.2}_{-10.4}$ & $21.5 \pm 1.8$\\
04545503-4755337 & (M5.1) & COL & $65.0$ & $17.2$ & $86.5^{+12.7}_{-13.2}$ & $57.0^{+8.4}_{-10.0}$ & $22.0 \pm 1.7$\\
05022823-5639575 & (M5.8) & ABDMG & $23.2$ & $33.4$ & $111.5^{+15.1}_{-16.7}$ & $35.0^{+6.8}_{-6.0}$ & $29.7 \pm 1.4$\\
05081734-2249218 & (M5.6) & COL & $66.6$ & $15.1$ & $62.3^{+9.2}_{-8.4}$ & $47.8^{+6.0}_{-5.6}$ & $22.5 \pm 1.4$\\
05104717-5303001 & (M5.7) & COL & $60.5$ & $18.3$ & $61.1^{+9.2}_{-8.8}$ & $59.4^{+8.8}_{-7.6}$ & $21.8 \pm 1.4$\\
05143708-0106240 & (M6.3) & COL & $26.1$ & $37.8$ & $38.9^{+9.5}_{-6.4}$ & $58.6^{+5.6}_{-5.2}$ & $19.8 \pm 2.0$\\
05193582-5045254 & (M8.4) & COL & $14.7$ & $37.9$ & $20.6^{+5.3}_{-2.8}$ & $70.6^{+7.2}_{-6.4}$ & $22.8 \pm 1.4$\\
05304407-4015022 & (M6.2) & COL & $54.6$ & $15.1$ & $49.6^{+8.8}_{-8.9}$ & $45.4^{+8.8}_{-7.2}$ & $23.2 \pm 1.4$\\
05410486-4250318 & (M5.6) & ARG & $30.7$ & $37.7$ & $71.0^{+7.4}_{-7.2}$ & $20.5 \pm 2.0$ & $16.6 \pm 2.5$\\
05431123-1914441 & (M4.9) & COL & $78.2$ & $19.9$ & $98.4^{+13.8}_{-14.1}$ & $55.8^{+8.0}_{-6.8}$ & $23.1 \pm 1.5$\\
05444541-4043541 & (M6.3) & COL & $49.4$ & $19.0$ & $47.4^{+8.8}_{-8.5}$ & $50.6^{+9.2}_{-8.0}$ & $23.4 \pm 1.4$\\
05520056-5711115 & (M5.7) & COL & $21.6$ & $35.7$ & $57.9^{+8.6}_{-8.4}$ & $66.6^{+9.6}_{-8.4}$ & $21.8 \pm 1.4$\\
05560733-6152431 & (M5.3) & ARG & $80.2$ & $34.4$ & $86.2^{+8.6}_{-8.4}$ & $30.5 \pm 2.8$ & $12.1 \pm 2.4$\\
05574516-1611279 & (M5.5) & COL & $61.0$ & $25.6$ & $65.7^{+9.8}_{-9.2}$ & $55.0^{+7.6}_{-6.8}$ & $23.2 \pm 1.5$\\
06124306-4503254 & (M5.1) & ARG & $85.4$ & $24.7$ & $106.6^{+11.1}_{-11.7}$ & $22.1 \pm 2.4$ & $17.3 \pm 2.4$\\
06142994-6318559 & (M4.3) & ARG & $89.0$ & $30.0$ & $159.3 \pm 16.2$ & $30.1 \pm 2.8$ & $11.0 \pm 2.2$\\
06375666-3711326 & (M4.8) & ARG & $64.9$ & $46.5$ & $120.1^{+13.7}_{-14.5}$ & $24.5 \pm 3.2$ & $21.0 \pm 2.1$\\
06422966-6338532 & (M5.3) & ARG & $23.7$ & $38.1$ & $87.5^{+8.8}_{-8.5}$ & $30.1 \pm 2.8$ & $8.6 \pm 2.1$\\
06443003+7206516 & (M7.2) & ARG & $24.0$ & $30.8$ & $34.1^{+4.3}_{-3.9}$ & $21.7^{+1.6}_{-2.0}$ & $6.5 \pm 1.7$\\
10033606-2717454 & (M5.6) & ARG & $52.0$ & $29.0$ & $70.5^{+7.4}_{-7.5}$ & $18.9 \pm 2.0$ & $11.3 \pm 1.3$\\
11131034-1504005 & (M5.8) & TWA & $24.5$ & $16.4$ & $20.9^{+1.0}_{-1.3}$ & $38.6^{+4.0}_{-3.6}$ & $9.7 \pm 1.4$\\
12094695-3213217 & (M5.0) & ARG & $33.5$ & $40.3$ & $111.9^{+11.3}_{-11.7}$ & $26.1^{+2.8}_{-2.4}$ & $-0.1 \pm 1.4$\\
12342562-3449134 & (M5.3) & ARG & $15.1$ & $49.2$ & $87.2^{+8.9}_{-8.6}$ & $26.9^{+2.8}_{-2.4}$ & $-2.5 \pm 1.4$\\
12471067-3632150 & (M5.1) & TWA & $12.4$ & $15.2$ & $41.1^{+8.5}_{-6.4}$ & $74.2 \pm 8.0$ & $9.6 \pm 1.8$\\
13325579-2916199 & (M5.4) & ARG & $16.6$ & $44.7$ & $77.7^{+7.9}_{-8.1}$ & $20.1 \pm 2.0$ & $-7.6 \pm 1.7$\\
15031325-2840134 & M5 & ABDMG & $4.3$ & $27.5$ & $113.4^{+11.3}_{-10.6}$ & $29.7 \pm 1.6$ & $-1.6 \pm 1.7$\\
17052735-8927393 & (M5.2) & ARG & $67.9$ & $42.6$ & $101.0^{+10.9}_{-11.6}$ & $39.8^{+4.8}_{-4.4}$ & $0.2 \pm 2.4$\\
19002957-6341281 & (M5.5) & BPMG & $44.9$ & $33.0$ & $61.7^{+3.9}_{-4.0}$ & $35.4^{+3.2}_{-2.8}$ & $3.6 \pm 2.4$\\
19574428-4548351 & (M5.6) & BPMG & $68.4$ & $31.6$ & $57.5^{+3.6}_{-3.9}$ & $37.8 \pm 3.2$ & $-4.7 \pm 2.0$\\
20042845-3356105 & M4.5 & BPMG & $93.8$ & $18.4$ & $202.3^{+8.2}_{-5.2}$ & $36.2^{+3.2}_{-3.6}$ & $-6.7 \pm 2.0$\\
20125357-8750136 & (M5.7) & ARG & $81.8$ & $37.0$ & $68.1^{+7.2}_{-7.1}$ & $40.6^{+4.0}_{-4.4}$ & $-0.1 \pm 2.2$\\
20134431-8027523 & (M4.9) & ABDMG & $12.9$ & $21.4$ & $182.7^{+16.4}_{-15.1}$ & $34.6 \pm 2.8$ & $19.3 \pm 1.7$\\
20300192+0023553 & (M4.5) & ARG & $54.5$ & $34.3$ & $141.3^{+16.7}_{-18.1}$ & $22.5 \pm 3.2$ & $-19.0 \pm 1.8$\\
20485716-0053473 & (M5.7) & BPMG & $25.3$ & $47.9$ & $56.4^{+4.2}_{-4.7}$ & $31.7^{+3.6}_{-3.2}$ & $-11.7 \pm 1.8$\\
20491839-3130422 & (M6.5) & BPMG & $60.5$ & $19.2$ & $34.5^{+2.9}_{-2.6}$ & $33.3 \pm 2.8$ & $-4.3 \pm 1.8$\\
20505221-3639552 & (M7.2) & ARG & $25.1$ & $39.4$ & $37.3^{+5.0}_{-4.7}$ & $35.0^{+4.0}_{-4.4}$ & $-14.7 \pm 1.8$\\
20542341-2947370 & (M5.4) & BPMG & $10.7$ & $37.9$ & $64.9 \pm 4.3$ & $35.0 \pm 3.2$ & $-3.6 \pm 1.7$\\
20544332-2745512 & (L3.6) & BPMG & $25.8$ & $43.0$ & $9.7 \pm 0.3$ & $38.6 \pm 3.6$ & $-5.3 \pm 2.0$\\
21332663-3023385 & (M5.3) & BPMG & $14.4$ & $44.3$ & $77.7^{+4.5}_{-5.3}$ & $36.6 \pm 3.2$ & $-2.0 \pm 1.7$\\
21350124-0308342 & (M5.3) & BPMG & $29.8$ & $44.6$ & $74.4^{+4.9}_{-5.6}$ & $35.4 \pm 3.6$ & $-8.9 \pm 1.8$\\
21421917+1041299 & (M3.8) & ABDMG & $10.7$ & $47.6$ & $207.8^{+2.6}_{-1.3}$ & $45.0^{+4.0}_{-3.6}$ & $-16.9 \pm 2.2$\\
21500933+0558102 & (M4.9) & ARG & $23.6$ & $47.2$ & $117.6^{+13.5}_{-14.6}$ & $27.7^{+4.0}_{-3.6}$ & $-14.0 \pm 2.2$\\
21501011+0558137 & (M4.9) & BPMG & $19.6$ & $33.9$ & $95.7^{+7.2}_{-7.7}$ & $28.9^{+3.6}_{-3.2}$ & $-9.0 \pm 2.2$\\
21571877-3520194 & (M5.5) & ARG & $52.1$ & $30.2$ & $74.8^{+8.1}_{-8.6}$ & $20.5 \pm 2.4$ & $-11.0 \pm 1.3$\\
22043859-1832204 & M4.5 & BPMG & $26.3$ & $29.1$ & $71.2^{+5.3}_{-5.4}$ & $36.6^{+4.0}_{-4.4}$ & $-7.2 \pm 3.8$\\
22071111+3116554 & (M4.9) & ARG & $16.6$ & $27.5$ & $121.1^{+13.0}_{-13.4}$ & $26.9^{+2.8}_{-3.2}$ & $-8.9 \pm 1.4$\\
22204161+2755040 & (M4.5) & ARG & $18.1$ & $32.3$ & $141.4^{+15.2}_{-15.6}$ & $32.5 \pm 3.6$ & $-11.2 \pm 1.5$\\
22254652-0606269 & (M5.4) & ABDMG & $17.2$ & $19.7$ & $120.2^{+12.3}_{-11.1}$ & $42.2^{+3.2}_{-2.8}$ & $-6.5 \pm 2.4$\\
22294830-4858285 & M4.5 & BPMG & $21.1$ & $44.4$ & $85.5^{+5.4}_{-5.6}$ & $33.8^{+2.8}_{-3.2}$ & $3.7 \pm 1.8$\\
22302626-0142063 & M4 & ABDMG & $14.6$ & $18.0$ & $190.5^{+15.1}_{-12.5}$ & $40.2 \pm 2.8$ & $-8.1 \pm 2.2$\\
23135156-4608234 & (M5.3) & ARG & $13.7$ & $45.0$ & $86.7^{+9.1}_{-9.2}$ & $36.6 \pm 4.0$ & $-3.6 \pm 1.7$\\
23241688-1522228 & (M5.5) & BPMG & $37.2$ & $17.1$ & $59.9^{+4.0}_{-4.2}$ & $24.9^{+2.0}_{-2.4}$ & $0.6 \pm 1.5$\\
23254385+3000061 & (L3.8) & ABDMG & $16.3$ & $33.6$ & $16.0^{+2.6}_{-3.1}$ & $41.0^{+4.4}_{-4.8}$ & $-14.7 \pm 3.4$\\
23301129-0237227 & M6 & BPMG & $42.8$ & $35.7$ & $137.0^{+8.9}_{-9.5}$ & $35.4^{+3.2}_{-3.6}$ & $-1.2 \pm 1.5$\\
23415196-0256296 & (M4.0) & BPMG & $34.1$ & $41.1$ & $147.3^{+9.6}_{-10.2}$ & $35.0^{+3.6}_{-3.2}$ & $-0.1 \pm 1.8$\\
23473986-0739414 & (M5.8) & BPMG & $28.1$ & $40.0$ & $49.3^{+2.6}_{-3.1}$ & $34.2^{+3.2}_{-2.8}$ & $1.1 \pm 1.5$\\
\enddata
\tablenotetext{a}{Spectral types in parentheses were estimated from \href{http://www.ipac.caltech.edu/2mass/}{\emph{2MASS}}--\href{http://wise2.ipac.caltech.edu/docs/release/allwise/}{\emph{AllWISE}} colors (see \hyperref[sec:filters]{Section~\ref*{sec:spt}}).}
\tablenotetext{b}{The binary hypothesis is more probable than the single hypothesis (see \hyperref[sec:filters]{Section~\ref*{sec:filters}}).}
\end{deluxetable*}
\twocolumngrid

==> hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump


